Efficient and High-Quality Seeded Graph Matching: Employing High Order Structural Information

Driven by many real applications, we study the problem of seeded graph matching. Given two graphs $G_1 = (V_1, E_1)$ and $G_2 = (V_2, E_2)$, and a small set $S$ of pre-matched node pairs $[u, v]$ where $u \in V_1$ and $v \in V_2$, the problem is to identify a matching between $V_1$ and $V_2$ growing from $S$, such that each pair in the matching corresponds to the same underlying entity. Recent studies on efficient and effective seeded graph matching have drawn a great deal of attention and many popular methods are largely based on exploring the similarity between local structures to identify matching pairs. While these recent techniques work well on random graphs, their accuracy is low over many real networks. Motivated by this, we propose to utilize high order neighboring information to improve the matching accuracy. As a result, a new framework of seeded graph matching is proposed, which employs Personalized PageRank (PPR) to quantify the matching score of each node pair. To further boost the matching accuracy, we propose a novel postponing strategy, which postpones the selection of pairs that have competitors with similar matching scores. We theoretically prove that the postpone strategy indeed significantly improves the matching accuracy. To improve the scalability of matching large graphs, we also propose efficient approximation techniques based on algorithms for computing PPR heavy hitters. Our comprehensive experimental studies on large-scale real datasets demonstrate that, compared with state of the art approaches, our framework not only increases the precision and recall both by a significant margin but also achieves speed-up up to more than one order of magnitude.

==> 0abstract.tex <==

\begin{abstract}
Driven by many real applications, in this paper we study the problem of seeded graph matching problem, a generalization of isomorphic mapping. Given two graphs $G_1 = (V_1, E_1)$ and $G_2 = (V_2, E_2)$ and a set $S$ of pairs of matched vertices $[u, v]$ where $u \in V_1$ and $v \in V_2$ , the problem of seeded graph matching is to identify the pairs of the the vertices from $V_1 \times V_2$ such that each pair $[u, v]$ is a matching between $u$ and $v$ extending $S$. This problem is a generalization of isomorphic mapping; it is harder
then the isomorphic mapping since $G_1$ and $G_2$ are generally not identical but similar regarding certain parts. The key issues are to develop effective matching scores and fast algorithms to conduct matching to maximize scores.
Recent studies on efficient and effective seeded graph matching have drawn a great deal of attentions and are largely based on local information. While these recent techniques work well on random graphs, their accuracy is low over many real graphs. Motivated by this, in this paper we propose to explore high order neighbouring structural information to increase the matching accuracy. As a result, a new framework of seeded graph matching is proposed by employing Personalized PageRank. To further boost the matching accuracy, we propose to postpone the selection of a matching pair among the pairs sharing one common vertex with similar matching scores. We can prove theoretically that the postpone strategy indeed significantly improves the matching accuracy. To speed up the computation, we also propose approximation techniques. Our comprehensive experimental studies on real datasets demonstrate that compared with the state of the art techniques, our techniques not only increase both precision and recall by a significant margin but also archive speed-up up to one order of magnitude.
%also more space- and time-efficient in most cases. %and has stronger robustness to the unaligned structures and incorrect seed matches.
$\tilde{O}(n)$
\end{abstract}


==> 0abstractNEW.tex <==

\begin{abstract}
%Driven by many real applications, in this paper we study the problem of seeded graph matching problem, a generalization of isomorphic mapping. Given two graphs $G_1 = (V_1, E_1)$ and $G_2 = (V_2, E_2)$ and a set $S$ of pairs of matched vertices $[u, v]$ where $u \in V_1$ and $v \in V_2$ , the problem of seeded graph matching is to identify the pairs of the the vertices from $V_1 \times V_2$ such that each pair $[u, v]$ is a matching between $u$ and $v$ extending $S$. This problem is a generalization of isomorphic mapping; it is is harder
%then the isomorphic mapping since $G_1$ and $G_2$ are generally not identical but similar regarding certain parts. The key issues are to develop effective matching scores and fast algorithms to conduct matching to maximize scores.
%Recent studies on efficient and effective seeded graph matching have drawn a great deal of attentions and are largely based on local information. While these recent techniques work well on random graphs, their accuracy is low over many real graphs. Motivated by this, in this paper we propose to explore high order neighbouring structural information to increase the matching accuracy. As a result, a new framework of seeded graph matching is proposed by employing Personalized PageRank. To further boost the matching accuracy, we propose to postpone the selection of a matching pair among the pairs sharing one common vertex with similar matching scores. We can prove theoretically that the postpone strategy indeed significantly improves the matching accuracy. To speed up the computation, we also propose approximation techniques. Our comprehensive experimental studies on real datasets demonstrate that compared with the state of the art techniques, our techniques not only increase both precision and recall by a significant margin but also archive speed-up up to one order of magnitude.

Driven by many real applications, in this paper we study the problem of seeded graph matching.
Given two graphs $G_1 = (V_1, E_1)$ and $G_2 = (V_2, E_2)$ and a set $S$ of pairs of matched vertices $[v, u]$ where $v \in V_1$ and $u \in V_2$,
the problem of seeded graph matching is to identify the vertex pairs from $V_1 \times V_2$ such that each pair $[v, u]$ is a matching between $v$ and $u$ extending $S$. This problem is a generalization of isomorphic mapping;
%it is harder than the isomorphic mapping since $G_1$ and $G_2$ are generally not identical but similar regarding certain parts.
it is more challenging than the isomorphic mapping due to the structural difference in two graphs.
The key issues are to design effective matching scores for each $[v, u]$ and develop efficient algorithms to conduct matching with the aim to maximize the overall matching scores.
Recent studies on seeded graph matching have drawn a great deal of attentions and are largely based on local information.
Though these techniques work well on random graphs, their accuracy is low over many real graphs.
Motivated by this, in this paper we propose to explore high order structural information to increase the matching accuracy.
%As a result, a new framework of seeded graph matching is proposed by employing personalized PageRank. To further boost the matching accuracy, we propose to postpone the selection of a matching pair among the pairs sharing one common vertex with similar matching scores. We can prove theoretically that the postpone strategy indeed significantly improves the matching accuracy. To speed up the computation, We also propose approximation techniques. Our comprehensive experimental studies on real datasets demonstrate that compared with the state-of-the-art techniques, our techniques not only increase both precision and recall by a significant margin but also achieve speed-up up to one order of magnitude.
%also more space- and time-efficient in most cases. %and has stronger robustness to the unaligned structures and incorrect seed matches.
%As a result, a new framework of seeded graph matching is proposed to quantify the connection between matched vertices and the vertices to be matched with personalized PageRank;
%afterwards, the algorithm has the early matched vertices to provide evidence for the matching of new pairs.
As a result, a new framework of seeded graph matching is proposed by quantifying the connection between matched vertices and the vertices to be matched 
with personalized PageRank and conducting matching iteratively. 
%To further boost the matching accuracy, we design certain criteria to allow only the very strong candidate pairs to be matched. 
%To further boost the matching accuracy, we propose to postpone the selection of a matching pair among the pairs sharing one common vertex with similar matching scores.
To further boost the matching accuracy, we propose to postpone the matching of a pair $[v,u]$ if there is another pair containing $v$ or $u$ holding a similar matching score as that of $[v,u]$.
%We can prove theoretically that our criteria significantly improves the matching precision.
We can prove theoretically that our postpone strategy significantly improves the matching precision.
%postpone the selection of a matching pair among the pairs sharing one common vertex with similar matching scores. We can prove theoretically that the postpone strategy indeed significantly improves the matching accuracy.
To speed up the computation, we raise effective optimization techniques by adopting Forward-Push to obtain PPR heavy hitters; the time complexity of our framework is also analysed.
Our comprehensive experimental studies on various large-scale graphs demonstrate that our new seeded graph matching algorithm outperforms the start-of-the-art algorithms w.r.t. quality, efficiency, and robustness.
 %demonstrate that compared with the state-of-the-art techniques, our techniques not only increase both precision and recall by a significant margin but also achieve speed-up up to one order of magnitude.
%also more space- and time-efficient in most cases. %and has stronger robustness to the unaligned structures and incorrect seed matches.

\end{abstract}


==> 1introductionNEW.tex <==
\section{Introduction}\label{sec1}

%In many applications such as social network de-anonymization, protein-network alignment,
%pattern recognition, etc., a key task is to match two graphs $G_1$ and $G_2$ from different domains by building an injective mapping from a subset of vertices in $G_1$ to the vertex set of $G_2$.
%Formally, we are given two graphs, $G_1=(V_1, E_1)$ and $G_2=(V_2, E_2)$ with certain part of the two vertex sets $V_1$ and $V_2$ being the same; that is, in general, $V_1$ and $V_2$ may only have a partial overlapping.
%For example, $G_1$ and $G_2$ could be the user networks of Facebook and Twitter,  respectively, where part of the users in the two networks are the same.
%The graph matching problem aims to identify all pairs of vertices $[v_i, u_j]\in V_1 \times V_2$ such that $v_i$ and $u_j$ correspond to the same entity.


In many applications such as social network de-anonymization, protein-network alignment,
pattern recognition, etc., a key task is to match two graphs $G_1$ and $G_2$ from different domains by building an injective mapping from a subset of vertices in $G_1$ to the vertex set of $G_2$.
Formally, we are given two graphs, $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$, with certain part of the two vertex sets $V_1$ and $V_2$ being the same;
%where $V_1$ and $V_2$ may only have a partial overlapping.
for example, $G_1$ and $G_2$ could be the user networks of Facebook and Twitter respectively, and only a part of users in one network also have accounts on the other network.
%part of the users in the two networks are the same.
The graph matching problem aims to identify all pairs of vertices $[v, u]\in V_1 \times V_2$ such that $v$ and $u$ correspond to the same entity.


%
%Graph matching is often conducted by exploiting both structural information and semantic features \cite{malhotra2012studying, nunes2012resolving, zhang2015cosnet}. In this paper, we focus on the structure-based graph matching for the following reasons:
%1) the semantic features are often unavailable in the matching of networks \cite{singh2008global, mohammadi2017triangular}, 2) it has been shown structural information is the most important to identify a node in network \cite{henderson2011s},
%and 3) the techniques based on semantic features may be fragile against malicious users with fake profiles. Consider the input graphs (e.g., $G_1$ and $G_2$) to be matched are often not based on label information. Consequently,  the algorithm needs to construct the matching relying solely on the graph structural information. Moreover, two graphs to be matched are usually similar in some part but the similar part are often not identical. This makes the problem of graph matching much more challenging than the classic graph isomorphism detection problem since it is even hard to identify the exact matching. Therefore, the graph match is often conducted with the aim to maximize the matching scores. (no definition for matching score.)

%
Graph matching is often conducted by exploiting both structural information and semantic features \cite{malhotra2012studying, nunes2012resolving, zhang2015cosnet}.
%Two kinds of information are often exploited in graph matching, i.e., the graph structure and the semantic features \cite{malhotra2012studying, nunes2012resolving, zhang2015cosnet}.
In this paper, we focus on the structure-based graph matching for the following reasons:
1) the semantic features are often unavailable %in the matching of networks
\cite{singh2008global, mohammadi2017triangular};
2) it has been shown structural information is the most important feature to identify a vertex in network \cite{henderson2011s};
and 3) the techniques based on semantic features may be fragile against malicious users with fake profiles.
Consequently, effective algorithms need to be developed to construct the matching relying solely on the graph structural information.

The structural difference in two graphs to be matched makes the graph matching much more challenging than the classic graph isomorphism problem; identifying the exact matching between two isomorphic graphs is widely believed to be intractable in general. Therefore, the graph matching is often conducted with the aim to maximize the overall matching scores,
where one matching score, corresponding to the match of a pair $[v,u]$, is often differently defined in the literature.

%In this paper, we study the problem of {\em seeded graph matching}; that is, given two graphs $G_1 (V_1, E_1)$ and $G_2 (V_2, E_2)$ and a set $S$ of pairs of vertices $[u, v]$ ($u \in V_1$ and $v \in V_2$) denoting the matching of $u$ and $v$, the problem of seeded graph matching is to identify vertex pairs $[u', v']$ ($u' \in V_1$ and $v' \in V_2$) in $V_1 \times V_2$  extending $S$
%such that $u'$ is injective mapped to $v'$, corresponding to a unique identity (e.g., a person).

%In this paper, we further assume that the algorithm is provided with a small set of ``pre-matched" node pairs in the beginning; this assumption is also adopted in a line of work~\cite{yartseva2013performance, korula2014efficient, kazemi2015growing, zhou2016cross, shirani2017seeded}. We call this the \emph{seeded graph matching} problem.

Motivated by real applications, in this paper, we study the problem of {\em seeded graph matching}: given two graphs $G_1 (V_1, E_1)$ and $G_2 (V_2, E_2)$ and a \emph{seed} set $S$ of pairs of vertices $[v, u]$ ($v \in V_1$ and $u \in V_2$) denoting the matching of $v$ and $u$, the problem of seeded graph matching is to identify vertex pairs $[v', u']$ in $V_1 \times V_2$  extending $S$
such that $v'$ is injective mapped to $u'$, corresponding to a unique identity (e.g., a person).


\vspace{0.1cm}
\noindent
\textbf{Applications.}
%The seeded graph matching has many real applications. For example, in social networks such as Instagram and Facebook, each vertex represents a user, and a network contains an edge $(v_i, v_j)$ if a user $v_i$ is followed by another user $v_j$. Given that many users on Instagram may connect to their Facebook accounts, such linking information may be used as the seeded matching to identify pairs of accounts on two networks that belong to the same individual. Consequently, we can recommend friends and social communities, and label users from one social network to another social network.
The seeded graph matching has many applications. For example, in social networks such as Instagram and Facebook, each vertex represents a user, and a network contains an edge $(v, u)$ if a user $v$ is followed by another user $u$. Given that many users on Instagram may connect to their Facebook accounts, such linking information may be used as the seeded matching to identify pairs of accounts on two networks that belong to the same individual. Consequently, we can recommend friends and social communities, and label users from one social network to another social network.

%Another application is that seeded graph matching is a key step in a general graph matching without seeds.  Many existing techniques \cite{zhu2013high, wang2018deepmatching, zhou2018structure} to conduct a general graph matching often involve two steps: 1) Seed Detection: detect the two small set $S_1$ and $S_2$ of vertices from $G_1$ and $G_2$, respectively, together with one-to-one mapping from $S_1$ to $S_2$, and 2) Seed Propagation: expand the mapping between $S_1$ and $S_2$ to generate graph matching between $G_1$ and $G_2$; that is, seeded graph matching.
%Another application is that seeded graph matching is a key step in a general graph matching without seeds.  Many existing techniques \cite{zhu2013high, wang2018deepmatching, zhou2018structure} of general graph matching often involve two steps: 1) Seed Detection: detect the two small set $S_1$ and $S_2$ of vertices from $V_1$ and $V_2$, respectively, together with a one-to-one mapping from $S_1$ to $S_2$, and 2) Seed Propagation: expand the mapping between $S_1$ and $S_2$ to generate a graph matching between $V_1$ and $V_2$; that is, seeded graph matching.
The seeded graph matching is also a key step in the general graph matching without seeds.
Many existing techniques \cite{zhu2013high, wang2018deepmatching, zhou2018structure} in general graph matching often involve two steps: 1) Seed Detection: detect a small set $S$ of matches from $V_1\times V_2$; and 2) Seed Propagation: expand the mapping from $S$ to generate a graph matching between $V_1$ and $V_2$; that is, seeded graph matching.

\vspace{0.1cm}
\noindent
\textbf{Percolation Graph Matching and its Limit.}
%Recently, the problem of seeded graph matching has drawn a reasonable deal of attention
%\cite{yartseva2013performance, korula2014efficient, kazemi2015growing, zhou2016cross, shirani2017seeded,yacsar2018iterative}. The existing techniques is largely based on effectively using local information to identify matching pairs.  For example, if a vertex $v \in V_1$ has a neighbor $v'$ which is already matched to a neighbor $u'$ of $u \in V_2$, then $[v,u]$ gets a vote from $[v', u']$ to be a valid matching pair. This is the central idea of the state-of-the-art paradigm, {\em percolation} graph matching (PGM).
Recently, the problem of seeded graph matching has drawn a reasonable deal of attention
\cite{yartseva2013performance, korula2014efficient, kazemi2015growing, zhou2016cross, shirani2017seeded,yacsar2018iterative}. The existing techniques are largely based on effectively using local information to identify matches.  For example, if vertex $v \in V_1$ has a neighbor $v'$ which is already matched to $u'$, a neighbor of $u \in V_2$, then $[v,u]$ gets a vote from $[v', u']$ to be a valid match. This is the central idea of the state-of-the-art paradigm, \emph{percolation} graph matching (PGM).

%
%The seed matches provide valuable information for identifying other matching pairs.  For example, if $i\in V_1$ has a neighbor which is already matched to a neighbor of $j\in V_2$, then $[i,j]$ is more likely to be a valid pair. This simple idea lies at the heart of a popular class of algorithms, namely percolation graph matching.

%
%(PGM) as a framework is firstly referred in
%. For a pair $[u_i, v_j]$ of vertices, where $u_i\in V_1,v_j\in V_2$,  we say $[u_{i'},v_{j'}]$ is its neighboring pair if $(u_i, u_{i'})\in E_1$ and $(v_j,v_{j'})\in E_2$.
% the case has not helped?
%So one can imagine there is large graph consists of $|V_1|\cdot|V_2|$ nodes corresponding to all possible pairs; two nodes are adjacent if they are neighboring pairs.
%

%PGM was first proposed in \cite{narayanan2009anonymizing}; it iteratively maintains a set of matched pairs starting from the set $S$ of seed pairs: (1) in each round, each \emph{unused} (initially all seed pairs are unused) matched pair (e.g., the above $[v', u']$) percolates to \emph{neighboring pairs}  (e.g., the above $[v, u]$) by adding one score to each of them and then becomes {\em used} pair;
%and (2) the pairs that received marks, namely \emph{candidate pairs}, are then examined by certain criteria and matched if they are qualified (new qualified pairs are then marked with \emph{unused}); for example if the score $r$ received is above a given threshold $T$ \cite{yartseva2013performance}. The iteration (algorithm) terminates when all matched pairs are used (i.e., have percolated) and no new candidate pair qualifies.

PGM was first proposed in \cite{narayanan2009anonymizing}; it iteratively maintains a set of matched pairs starting from the set $S$ of seed pairs:
(1) in each round, each \emph{unused} matched pair or seed pair (e.g., the above $[v', u']$) percolates $1$ mark to each of its \emph{neighboring pairs} (e.g., the above $[v, u]$);
(2) the pairs that received marks, namely \emph{candidate pairs}, are then examined by certain criteria, e.g., whether the number of marks $r$ received is above a given threshold $T$ \cite{yartseva2013performance}, and are matched if they are qualified (the matched pairs will percolate in the next round). The algorithm terminates when all matched pairs have percolated and no new candidate pair is eligible for the criteria.

%There are several variations towards recent PGM based algorithms to specify their matching scores and/or matching criteria. The authors in \cite{korula2014efficient} (also used in \cite{wang2018deepmatching}) propose to firstly consider pairs with high vertex degrees and then among such pairs select the candidate pair with the highest score $r$ (and also above a threshold $T$) to match, while the authors in ~\cite{kazemi2015growing} puts the first preference on selecting pairs with the highest matching score $r$ (and also above a threshold $T$) and the second preference on minimum degree difference between a pair of vertices.
%The authors in ~\cite{zhou2016cross} proposes to simply choose the pairs of vertices with the maximal matching score by ignoring threshold $T$. %(It includes some other techniques like tie strategy.)
%A very recent work \cite{yacsar2018iterative} proposes to use the seeds as anchors to allocate each vertex $v$ based on the lengths of shortest paths from $v$ to each
%anchors. Then, the algorithm matches vertices in the same regions by greedily choosing pairs with the maximum similarity scores which are based on a combination of the number of neighbouring matched pairs and the degree difference.
%The larger portion of the neighbouring pairs are matched pairs and the smaller degree differences, the larger similarity of $[v, u]$.
%There are several variations towards recent PGM based algorithms to specify their matching scores and/or matching criteria.
%The authors in \cite{korula2014efficient} (also used in \cite{wang2018deepmatching}) propose to firstly consider pairs with high vertex degrees and among such pairs select the pair with the highest score $r$ (and also above a threshold $T$) to match,
%while the authors in ~\cite{kazemi2015growing} put the first preference on selecting pairs with the highest matching score $r$ (and also above a threshold $T$) and the second preference on minimum degree difference between the pair of vertices.
%The authors in ~\cite{zhou2016cross} choose the vertex pairs with the maximal matching score ignoring the threshold $T$. %(It includes some other techniques like tie strategy.)
%A very recent work \cite{yacsar2018iterative} proposes to locate each vertex $v$ based on the lengths of shortest paths from $v$ to the seeds (anchors).
%Then, the algorithm measures vertices in the same regions and prefers pairs with smaller degree difference and larger portion of matched pairs among the neighbouring pairs.

There are several variations towards PGM algorithms to specify their matching scores and/or matching criteria.
\cite{korula2014efficient} (also used in \cite{wang2018deepmatching}) matches the pair with the highest score $r$ among a set of candidate pairs with high vertex degrees;
%firstly consider the pairs with high vertex degrees and among such pairs match the one with the highest score $r$ (and also above a threshold $T$).
\cite{zhou2016cross} chooses the vertex pairs with the maximal matching score ignoring the threshold $T$;
\cite{kazemi2015growing} puts the first preference on selecting pairs with the highest matching score $r$ (and $r\ge T$) and the second preference on minimum degree difference between the two end vertices of a pair.
%A very recent work \cite{yacsar2018iterative} proposes to use the seeds as anchors to allocate each vertex $u$ based on the lengths of shortest paths from $u$ to each
%anchors. Then, we match vertices in the same regions by greedily choosing pairs with the maximum similarity scores which are based on a combination of the number of neighbouring matched pairs and the degree difference.
%The larger portion of the neighbouring pairs are matched pairs and the smaller degree differences, the larger similarity of $[u, v]$.
A very recent work \cite{yacsar2018iterative} proposes to locate each vertex $v$ based on the lengths of shortest paths from $v$ to the seeds (anchors).
Then, the algorithm measures vertices in the same regions and prefers pairs with smaller degree difference and larger portion of matched pairs among the neighbouring pairs.


%
%The performance of the PGM framework is highly sensitive to the size of seed set and the threshold $T$. Insufficient number of seeds often leads to early termination of percolation.
%One can reduce the threshold $k$ to make the algorithm percolate easily, but this tends to match wrong pairs.
%To prevent early stopping, a new strategy, namely ExpandWhenStuck (EWS), is proposed in~\cite{kazemi2015growing}. When the percolation stops, EWS then collects all candidate pairs, which are pairs that receive at least $1$ mark but haven't meet the matching criteria, to form a \emph{noisy seed set}, and allows this set of pairs to percolate. After this noisy expansion, the algorithm continues the normal PGM process.
%Once the candidate pairs is added to noisy seed set, they will not be used for percolation again.
%This approach effectively prevents early-stop, and EWS significantly outperforms previous PGM algorithms when the number of seeds is very small.

\begin{figure}[h]
\begin{centering}
\includegraphics [width=3.0in]{fig/fig11.eps}
%\includegraphics[trim=2 0 38 0,clip,width=\figsize]{fig/fig1.eps}
%\label{fig:fig1}
\vspace*{-1mm}
\caption{Left Graph $G_L$ and Right Graph $G_R$. }
\label{MatchingExample}
\vspace*{-2mm}
\end{centering}
\end{figure}

%A major limit of the existing PGM algorithms is that local information can easily lead to wrong matching.
%Regarding the example in  Figure \ref{MatchingExample}, suppose that seeds $s_i$ matches $s'_i$ for $1 \leq i \leq 3$, respectively. Intuitively, in this case $v_i$ should be matched with $u_i$ for $1 \leq i \leq 8$ though $G_L$ and $G_R$ are not the same.
%Nevertheless, the state of the art PGM algorithms \cite{korula2014efficient, zhou2016cross, kazemi2015growing} will lead to
%the focus of the local information as shown in Figure \ref{local}. In particular, the algorithms \cite{korula2014efficient, kazemi2015growing} conclude that $u_1$ matches $v_2$ and $u_2$ matches $v_1$ if the threshold $T = 2$, while the algorithms in  \cite{zhou2016cross, yacsar2018iterative} also leads to the same result by the greedy heuristic.
%Moreover, the algorithms in \cite{korula2014efficient, kazemi2015growing} stops matching further, while the algorithms in \cite{yacsar2018iterative,zhou2016cross} may continue the wrong matching since no threshold constraints.

%\cite{yacsar2018iterative} is based on mapping rather than percolation. Not sure if good to put it in the following paragraph.
A major limit of existing PGM algorithms is that they mainly rely on neighboring information in each iteration, which can easily lead to wrong matches.
Regarding the example in  Figure \ref{MatchingExample}, suppose $[s_i,s'_i]$ for $1 \leq i \leq 3$ are the seed pairs. Intuitively, in this case $v_i$ should be matched with $u_i$ for $1 \leq i \leq 8$ though $G_L$ and $G_R$ are not the same.
Nevertheless, the state-of-the-art PGM algorithms will lead to the focus of the neighboring information as shown in Figure \ref{local}. In particular, the algorithms \cite{korula2014efficient, kazemi2015growing} match pairs $[v_1, u_2]$ and $[v_2, u_2]$ if the threshold $T = 2$; the algorithms in \cite{zhou2016cross, yacsar2018iterative} also lead to the same result by the greedy heuristic, while they continue the wrong matching since no threshold constraints. 
%Moreover, the algorithms in \cite{korula2014efficient, kazemi2015growing} stops matching further, while the algorithms in \cite{yacsar2018iterative,zhou2016cross} may continue the wrong matching since no threshold constraints.

\begin{figure}[h]
\begin{centering}
\includegraphics [width=3.2in]{fig/fig21.eps}
%\includegraphics[trim=2 0 38 0,clip,width=\figsize]{fig/fig1.eps}
%\label{fig:fig1}
\vspace*{-1mm}
\caption{Misled by Local Information}
\label{local}
\vspace*{-2mm}
\end{centering}
\end{figure}




%
%
%
%One major limitation of existing PGM algorithms is that they fail to break \emph{Local Symmetry}.
%It is easy to check all PGM algorithms mentioned above~\cite{yartseva2013performance, korula2014efficient, zhou2016cross, kazemi2015growing} fail to match the two graphs in Figure~\ref{fig:fig1} with probability $1/2$.
%We take EWS~\cite{kazemi2015growing} as an example, which matches node pairs with at least $2$ matched neighboring pairs ($r\ge 2$).
%%and utilizes the degree centrality by matching the node pair with minimal degree difference ($||N(i)|-|N(j)||$) first. %, i.e., the pair $[i,j]$ with the minimal $||N(i)|-|N(j)||$.
%%In Figure~\ref{fig:fig1}, we are matching two graphs (separated by the dashed line) designed to be isomorphic, thus the ground truth is clear: with seed pairs $[s_1, s_3]$ and $[s_2, s_4]$ provided, $[u_1,v_1]$ and $[u_2,v_2]$ are the correct matches because $\triangle_{u_1i_1i_2}$ and $\triangle_{v_1j_1j_2}$ are aligned, and $\wedge_{i_3u_2i_4}$ and $\wedge_{j_3v_2j_4}$ are aligned.
%The EWS algorithm first percolates from two seed pairs and obtains $4$ candidate pairs $[u_1,v_1]$, $[u_1,v_2]$, $[u_2,v_1]$ and $[u_2,v_2]$. Each candidate pair has a score $r=2$ satisfying the matching criteria. Meanwhile, all $4$ candidate pairs have the same degree difference $0$. In this case, the EWS randomly chooses a pair to be matched first, and thus will fail to find the correct hidden matching with probability $1/2$.
%
%
%Moreover, an early mistake may propagate and lead to cascade of errors.
%%Another concern for the PGM algorithms is the cascading mismatching. The percolation mechanism determines the high dependency of matching results, since whether a pair can be correctly matched relies on the matching results of its neighboring pairs directly. Note that the effect of early matches can be regarded as a strong bias on the later matching w.r.t. the effect of initial seed pairs.
%In the example of Figure~\ref{fig:fig1}, once EWS matches $[u_1,v_2]$ and $[u_2,v_1]$, the upper left part will more likely be matched to the lower right part. Intuitively, we should postpone this decision making and explore further to seek a symmetry breaker. %but,
%in our example, this leads to early stopping, as no other pair is qualified for percolation.

% The key is, even if the EWS allows repeated percolation whenever symmetry exists, it suffers from the dilemma of 1-order Weisfeiler Lehman coloring, i.e., the similarity is always decided by the first structure difference the percolation meets.
%
%\begin{figure}[!t]
%\begin{centering}
%\includegraphics [width=3.2in]{fig/fig1.eps}
%%\includegraphics[trim=2 0 38 0,clip,width=\figsize]{fig/fig1.eps}
%%\label{fig:fig1}
%\vspace*{-1mm}
%\caption{Graph matching on two isomorphic graphs.}
%\label{fig:fig1}
%\vspace*{-5mm}
%\end{centering}
%\end{figure}


%they may argue on the following method. But if we provide the this part, they may ask for a comparison in the experiments

%It is worth mentioning that an additional strategy of postponing the matching of \emph{close adversary pairs}, which has never been proposed though, can help the EWS algorithms match correctly in the case of Figure~\ref{fig:fig1}, i.e., after the first-round percolation, $[u_1,v_1]$ and $[u_1,v_2]$ are two adversary pairs relevant to node $u_1$ with the same scores $r=2$, and the algorithm should postpone the matching of $u_1$ until the tie is broken (in the third-round percolation).
%% corresponding to a weisfeiler-lehman graph labelling method? It does iterative percolation until it firstly finds the asymmetric structure.
%However, this strategy is still sensitive to the structure difference and fails some cases.
%% simple and direct case?
%For example, in Figure~\ref{fig:fig2}, we assume $[u_1,v_1]$ and $[u_2,v_2]$ are two correct matches considering the minimal graph edit distance. But the EWS algorithm with the postponing strategy wrongly matches $[u_1,v_2]$ by the effect of edges $(i_1,i_2)$ and $(j_1,j_2)$. This is because this approach does iterative percolation and is strongly affected by the first asymmetric structure detected. This approach doesn't solve the cascading mismatching either. Moreover, the additional matching criteria leads to a even larger candidate pair set than that of EWS algorithm.% though the latter is already infeasible on large graphs.

%\begin{table}[t]
%\small
%\renewcommand{\arraystretch}{1.4}
%\begin{center}
%\vspace*{-2mm}\caption{\label{table:rp}Reaching probability of decaying random walks. For example in Figure~\ref{MatchingExample}.}
%\resizebox{\columnwidth+0.1in}{!}{%
%\begin{tabular}{c|ccc|ccc}
%    \noalign{\hrule height 0.6pt}
%    \multirow{2}{*}{Target} & \multicolumn{3}{c|}{\textbf{1-step random walk}} & \multicolumn{3}{c}{\textbf{1 \& 2-step random walk}} \\
%    \cline{2-7}
%    & $s_1$($s'_1$) & $s_2$($s'_2$) & $s_3$($s'_3$) & $s_1$($s'_1$) & $s_2$($s'_2$) & $s_3$($s'_3$) \\
%    \hline
%    %\multicolumn{5}{l}{\textbf{1-step random walk}}\\
%    \hline
%    $v_1$ & $\PP/3$  & $0$                 & $\PP/3$  &  $\PP/3+\PP^2/6$  &  $\PP^2/4$  & $\PP/3+\PP^2/6$  \\
%    \hline
%    $v_2$ & $\PP/3$  & $\PP/2$  & $\PP/3$  &  $\PP/3$                     &  $\PP/2$   & $\PP/3$  \\
%    \hline\hline
%    $u_1$ & $\PP/3$  & $\PP/2$  & $\PP/3$  &  $\PP/3+\PP^2/6$  &  $\PP/2+\PP^2/4$ & $\PP/3+\PP^2/6$ \\
%    \hline
%    $u_2$ & $\PP/3$  & $0$                 & $\PP/3$  &  $\PP/3$                     &  $0$ & $\PP/3$ \\
%    \hline
%    \noalign{\hrule height  0.6pt}
%\end{tabular}
%}
%\end{center}
%\end{table}

%\noindent
%\textbf{Our approach.} To resolve this, we propose to combine local information with
%high order structural information to generate matching scores. In particular, for each seed $s_i$,
%we propose to use a random walk to reflect the graph structure as follows.
\noindent
\textbf{Our approach.} To resolve this, we propose to combine neighbouring information with  %combine neighbouring information ??
high order structural information to generate matching scores.
In particular, %for each seed $s_i$,
%we propose to use a random walk to reflect the graph structure as follows.
a random walk is used to reflect the connection between a seed vertex and a vertex to be matched: % as follows.
%
%Assume that one-step random walk from $v$ to $v'$ takes probability $\frac{1}{d_v}$ ($d_v$ is the degree of $v$) if there is an edge $(v, v')$, otherwise $0$. %Moreover, we also assume that a vertex has $\PP$ probability to grant a random walk at a vertex and $\SP$ to terminate a random walk at a vertex.
%Moreover, we also assume that a random walk at each step either moves to a neighboring vertex with probability $\PP$, or terminates at the current vertex (with probability $\SP$).
%Starting from $s_1$, $s_2$, and $s_3$ respectively, a $1$-step random walk has the following probabilities $p^1 (s_i, v_j)$ (for $1 \leq i \leq 3$ and $1 \leq j \leq 2$) to reach $v_1$ and $v_2$, respectively:
%\begin{itemize}
%\item   $p^1 (s_1, v_1) = \frac{1}{3} \PP$,
%        $p^1 (s_2, v_1) = 0$,
%        $p^1 (s_3, v_1) = \frac{1}{3} \PP$,
%        $p^1 (s_1, v_2) = \frac{1}{3} \PP$,
%        $p^1 (s_2, v_2) = \frac{1}{2} \PP$,
%        $p^1 (s_3, v_2) = \frac{1}{3} \PP$.
%        Similarly,
%\item   $p^1 (s'_1, u_1) = \frac{1}{3} \PP$,
%        $p^1 (s'_2, u_1) = \frac{1}{2} \PP$,
%        $p^1 (s'_3, u_1) = \frac{1}{3} \PP$,
%        $p^1 (s'_1, u_2) = \frac{1}{3} \PP$,
%        $p^1 (s'_2, u_2) = 0$,
%        $p^1 (s'_3, u_2) = \frac{1}{3} \PP$.
%\end{itemize}
%
%At each step of the random walk, we assume that the probability going from $v$  to $v'$ is $\frac{1}{|N(v)|}$ if there is an edge $(v, v')$, otherwise $0$. %Moreover, we also assume that a vertex has $\PP$ probability to grant a random walk at a vertex and $\SP$ to terminate a random walk at a vertex.
%Moreover, we also assume that, with probability $\SP$ , the random walk terminates at the current vertex.
%Given a proceeding probability $\PP$,
%For a random walk starting from $v$, we assume it, at each step, either proceeds to a randomly selected neighbor of the current vertex with probability $\PP$, or terminates at the current vertex (decaying) with probability $\SP$.
%, we assume that it at each step moves to a random neighbor of the probability going from $v$  to $v'$ is $\frac{1}{|N(v)|}$ if there is an edge $(v, v')$, otherwise $0$. %Moreover, we also assume that a vertex has $\PP$ probability to grant a random walk at a vertex and $\SP$ to terminate a random walk at a vertex.
%Moreover, we also assume that, with probability $\SP$, the random walk terminates at the current vertex.
%Starting from $s_i$ for $1 \leq i \leq 3$ respectively, a $1$-step random walk has the following probabilities $p^1 (s_i, v_j)$
%to reach $v_j$, for $1 \leq j \leq 2$ respectively:
%\begin{itemize}
%\item   $p^1 (s_1, v_1) = \PP/3$,
 %       $p^1 (s_2, v_1) = 0$,
   %     $p^1 (s_3, v_1) = \PP/3$,
     %   $p^1 (s_1, v_2) = \PP/3$,
       % $p^1 (s_2, v_2) = \PP/2$,
        %$p^1 (s_3, v_2) = \PP/3$.
        %Similarly,
%\item   $p^1 (s'_1, u_1) = \PP/3$,
  %      $p^1 (s'_2, u_1) = \PP/2$,
    %    $p^1 (s'_3, u_1) = \PP/3$,
     %   $p^1 (s'_1, u_2) = \PP/3$,
    %    $p^1 (s'_2, u_2) = 0$,
    %    $p^1 (s'_3, u_2) = \PP/3$.
%\end{itemize}
%In general, we use $p^t (s_i, v_j)$ ($p^t (s'_i, u_j)$) to denote the probability of a random walk
%from $s_i$ ($s'_i$) reaching $v_j$ ($u_j$) by $t$ steps. To measure the structural similarity of a vertex $u$ in $G_1$ and a vertex $v$ in $G_2$ regarding $t$ steps random walk, we simply use min/max to compare the accumulated probabilities from $s_i$ to $v$ and from $s'_i$ to $u$, respectively; that is,
%For a random walk starting from $v$, we assume it, at each step, either proceeds to a randomly selected neighbor of the current vertex with probability $\PP$, or terminates at the current vertex (decaying) with probability $\SP$.
%In general, we use $p^t (s_i, v_j)$ ($p^t (s'_i, u_j)$) to denote the probability that a decaying random walk starting
%from $s_i$ ($s'_i$) reaches $v_j$ ($u_j$) by $t$ steps. To measure the structural similarity of a vertex $u$ in $G_1$ and a vertex $v$ in $G_2$ regarding $t$-step random walks, we compare the accumulated probabilities from $s_i$ to $v$ and from $s'_i$ to $u$, respectively; more specifically, we use the following similarity function,
%We define the region that can be reached by a $t$-step random walk starting from $s$ as the \emph{Order-$t$} information w.r.t. source $s$.
%In our framework, order-$t$ information w.r.t. $s$ is compactly encoded by the probability distribution $q_s^{(t)}$,
%where $q_{s}^{(t)}(v)$ is the probability that random walk starting from $s$ reaches $v$ after $t$ steps.
we denote $q_{s}^{(t)}(v)$ the probability that a random walk starting from $s$ reaches $v$ after $t$ steps;
the \emph{Order-$t$} structural information w.r.t. $s$ is compactly encoded by the probability distribution $q_s^{(t)}$.
Intuitively, lower-order information is more important in deciding whether to match a pair, and thus will be assigned a higher
priority. Therefore, we encode the structural information of a vertex $v$ (w.r.t. some seed $s$) by
an accumulated probability $\pi^{(t)}(s,v)=\sum_{k=1}^{t}{\lambda^kq_s^{(k)}}$, where $0<\lambda<1$ is some weighing parameter.
It can be show that $\pi^{(\infty)}(s,v)$ is exactly the well-known \emph{Personalized PageRank} (PPR) of $v$ w.r.t. source $s$.

To measure the order-$t$ structural similarity of a vertex $v$ in $G_1$ and a vertex $u$ in $G_2$ w.r.t. a seed pair $[s_k,s'_k]$, we use the following similarity function,
\begin{equation}
\label{similarity}
sim^{(t)} (s_k, v, u) = \frac{\min\{ \pi^{(t)}(s_k,v), \pi^{(t)}(s'_k,u) \}}{\max \{ \pi^{(t)}(s_k,v), \pi^{(t)}(s'_k,u) \}}
\end{equation}
Here, we will define $sim^{(t)} (s_k, v, u) = 0$ if both $\pi^{(t)}(s_k,v)$ and $\pi^{(t)}(s'_k,u)$ are zero.
We use the sum of
$sim^{(t)} (s_k, v, u)$ over all seeds (i.e., $\sum_{[s_k,s'_k] \in S} sim^t (s_k, v, u)$) as the {\em matching score} of $[v,u]$.
Then we iteratively match the pair with the highest score.
Regarding the example above where $S = \{ s_1, s_2, s_3 \}$,
if the order-1 structural information is considered only, then
%$sim^{(1)} (S, v_2, u_1) = 3 $, $sim^{(1)} (S, v_2, u_2) = 2 $, $sim^{(1)} (S, v_1, u_1) = 2 $, $sim^{(1)} (S, v_1, u_2) = 2 $.
%Thus, we will choose intuitively wrong pairs to match:
%$v_2$ matches $u_1$ and then $v_1$ matches $u_2$.
we will choose intuitively wrong pairs to match: $v_2$ matches $u_1$ (with the highest score $sim^{(1)}(S, v_2, u_1)=3$) and then $v_1$ matches $u_2$.
However, if we continue to consider order-2 information w.r.t. all seeds, the order of matching scores in Step 1 may be reversed.
After calculating $sim^{(2)}(S, v_i, u_j)$  for $1\le i \le 2$ and $1 \le j \le 2$\footnote{We get $sim^{(2)}(S, v_1, u_1) = 3 - \frac{2}{2 + \lambda}$, $sim^{(2)}(S, v_2, u_1) = 3 - \frac{3 \lambda}{2 + \lambda}$, $sim^{(2)}(S, v_1, u_2) = 2 - \frac{2}{2 + \lambda}$, and $sim^{(2)}(S, v_2, u_2) = 2$.},
%$\pi^{(2)}(s_k,v)$ and $\pi^{(2)}(s'_k,u)$ for $1\le k \le 3$,
%it can be immediately verified that $sim^{(2)}(S, v_1, u_1) = 3 - \frac{2}{2 + \lambda}$, $sim^{(2)}(S, v_2, u_1) = 3 - \frac{3 \lambda}{2 + \lambda}$,
%$sim^{(2)}(S, v_1, u_2) = 2 - \frac{2}{2 + \lambda}$, and $sim^{(2)}(S, v_2, u_2) = 2$.
%Clearly, the largest value will be $sim^{(2)}(S, v_1, u_1)$ or $sim^{(2)}(S, v_2, u_1)$.
it is immediate, when $\lambda > \frac{2}{3}$, $sim^2 (S, v_1, u_1)$ is the highest score; that is, $v_1$ matches $u_1$ and $v_2$ matches $u_2$. This meets the intuition.
%that is, we match $[v_1,u_1]$ and then $[v_2,u_2]$. This meets the intuition.
%In fact, regarding the above example, our experiment also demonstrates that $sim^t(S, v_1, u_1)$ is greater than $sim^t(S, v_2, u_1)$ where $t\to \infty$ (i.e., the convergence values).

% Several paragraphs of advantages.

\noindent
\textbf{Contributions.}
%The above is the basic idea of our algorithm and the principal contribution of our paper. We employ the \emph{Personalized PageRank} (PPR) \cite{page1999pagerank} to quantify the connection between matched vertices and the vertices to be matched, etc. The main contributions of the paper can be summarized as follows.
%\begin{itemize}
%\item We propose to use PPR to generate matching scores to conduct seeded graph matching.
%The new paradigm employs high order structural information and our extensive experiment results
%demonstrate the new paradigm significantly improves the accuracy of the state-of-the-art techniques.
%\item We further propose an optimization policy to decide whether a candidate pair should be matched. Our policy is to only select a very strong pair to match;
%    that is, we choose the pair $[v,u]$ if the matching score of $[v,u]$ is greater than any of its adversary (candidate) pairs (i.e., $\{v\}\times V_2$ and $V_1 \times \{u\}$) by a factor of $(1+\beta)$ where $\beta > 0$ and the matching score of $[v,u]$ is greater than a given threshold $\gamma$.
%    While our experiment shows it can bring significant boost in precision and recall, we can also prove theoretically that this improves the precision significantly in random graph model.
%\item We develop efficient and effective approximate algorithms that retain the significant accuracy boost while speed-up the computation by up to one order of magnitude compared with the state-of-the-art algorithm with the best overall accuracy and efficiency \cite{kazemi2015growing}.
%\end{itemize}
The main contributions of the paper can be summarized as follows.
\begin{itemize}
\item We propose to quantify the connections between the seeds and the vertices to be matched with \emph{Personalized PageRank} (PPR) \cite{page1999pagerank}, which directly employs high order structural information. Based on that, we also design a new function to measure the matching score of each pair. 
%We propose to use PPR to generate matching scores to conduct seeded graph matching.
%The new paradigm employs high order structural information and our extensive experiment results
%demonstrate the new paradigm significantly improves the accuracy of the state-of-the-art techniques.
\item We raise the PPRGM framework which exploits the information of both initial seeds and the early matches to match new pairs. PPRGM uses the similar ideas as PGM to efficiently generate a set of candidate pairs. Further optimizations are proposed to conduct impact expansion efficiently by adopting Forward-Push to obtain PPR heavy hitters.
\item We also design effect matching criteria for PPRGM to select the very strong pairs to match;
    that is, we choose the pair $[v,u]$ if it satisfies $\mathtt{Score}(v,u)>(1+\beta)\mathtt{Score}(v',u')$ for any of adversary (candidate) pairs $[v',u']$ of $[v,u]$ (i.e., $\{v\}\times V_2$ and $V_1 \times \{u\}$ excluding $[v,u]$) where $\beta > 0$, and $\mathtt{Score}(v,u)>\gamma$ where $\gamma>1$ is a predefined threshold.
    While our experiment shows it can bring significant boost in precision and recall, we can also prove theoretically that this improves the precision significantly in random graph model.
\end{itemize}

%We conduct extensive experiments on various large-scale real-world graphs, which demonstrates that our new algorithm outperforms the start-of-the-art algorithm regarding the accuracy, robustness and efficiency.

\noindent
\textbf{Outline.} The related work immediately follows. Section \uppercase\expandafter{\romannumeral2} introduces notations and PPR.
Section \uppercase\expandafter{\romannumeral3} proposes a new matching score function and a basic graph matching algorithm.
Section\uppercase\expandafter{\romannumeral4} presents our PPRGM framework with unmatched advantages over the start-of-the-art methods, as well as effective optimization techniques to speed-up the computation.
It also presents the analysis of time complexity and effectiveness of our algorithm.
Section \uppercase\expandafter{\romannumeral5} evaluates all introduced algorithms using extensive experiments.
Finally we conclude the paper in Section \uppercase\expandafter{\romannumeral6}.

% Time complexity analysis:
%Besides, as PPRGM efficiently encodes the higher-order information of nodes (in each graph) and then compares the nodes across the graphs, the overall time complexity of Forward-Push is $O(|V_1||E_1|+|V_2||E_2|)$ in the worst case (or $c(|E_1|+|E_2|)$ for a const $c$ in practice), which overwhelms the $|E_1||E_2|$, the worst-case time complexity of Percolation in EWS.




==> 1relatedwork.tex <==
% high order may be not good.
% abstract local information -> higher-order

%\section{Related Work}

\noindent
\textbf{Related Work.}
%(1) matching based on isomorphic. (2) matching with ground truth.
%measurement of quality.
%isomorphic matching: (1) number of conserved edges \cite{singh2008global, zhu2013high} (2) number of conserved triangles \cite{mohammadi2017triangular} (no seed, 3-tensor, Maximum-weight-matching)
%ground truth matching: PGM algorithm. \cite{wang2018deepmatching}
%
%Given two graphs $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$, the graph matching aims to build a
%bijection $M$ between $V_1\rightarrow V_2$ s.t. each pair of vertices $[u,v]$ where $u\in V_1$
%and $v\in V_2$ corresponds to the same entity.
The graph matching problem is a generalization of the classic isomorphic mapping problem that is intractable in general \cite{lewis1983computers}. It has been widely used as a building block in various applications.
These include the alignment of protein-protein interaction networks in systems biology \cite{singh2008global, klau2009new, mohammadi2017triangular}, an identification of users (e.g., username, description, location and profile image) across different communities \cite{zafarani2009connecting, yartseva2013performance, korula2014efficient} in social networks, and de-anonymization which breaks the privacy of social networks \cite{backstrom2007wherefore, narayanan2009anonymizing, mislove2010you, wondracek2010practical, pedarsani2011privacy, ji2016seed}.

With the assumption of non-priori knowledge of the alignment, conventional graph matching algorithms firstly compute the similarity of each pair (all similarities are represented by a $|V_1|\times |V_2|$ matrix) and then identify the alignments with high scores.
\cite{singh2008global} builds the similarity matrix by iterative weighted propagation.
\cite{zhu2013high} consider both global vertex similarity $S_g$, defined by the similarity of corresponding eigenvectors from the spectral clustering, and local vertex similarity $S_{\ell}$, defined by the similarity of degree sequences of 2-neighborhood subgraphs.
Recent works \cite{wang2018deepmatching, zhou2018structure} propose to use deep-walk based graph embedding to compute the low-rank representation of each vertex. Then \cite{zhou2018structure} builds the node-to-node similarity matrix by defining a normalized Euclidean distance, while \cite{wang2018deepmatching} adopts Coherent Point Drift (CPD) method \cite{myronenko2007non} to identify the seeds and use \cite{korula2014efficient} to conduct seeded graph matching.

The seeded graph matching problem studied in this paper, however, assumes a small set of ``pre-matched'' pairs exists at the beginning. As discussed earlier,
the seed matches can be obtained by public link information \cite{zhang2015cosnet},
or by existing seed identification methods \cite{singh2008global, zhu2013high, wang2018deepmatching}.
A popular class of works are Percolation Graph Matching (PGM) \cite{korula2014efficient,yartseva2013performance,zhou2016cross}. %The PGM always matches the neighbors of seed matches and thus achieves great efficiency.
% If neighboring pair is defined in the introduction. Then omit the following definition.
%For a pair $[i,j]$, where $i\in V_1,j\in V_2$,  we say $[i',j']$ is its neighboring pair if $(i,i')\in E_1$ and $(j,j')\in E_2$.
While PGM is scalable and has a reasonable precision, traditional PGM methods may suffer from early-stop (low recall), especially when only a very small number of seeds are provided.
To prevent early termination, recently, ~\cite{kazemi2015growing} proposes a new strategy, namely ExpandWhenStuck (EWS).
Deviating from PGM, more recently, \cite{yacsar2018iterative} proposes to use seeds as anchor points to locate other vertices in a $2$-D space and then conduct mapping for the vertices in a same region. As we showed in
the introduction, the recent techniques in \cite{korula2014efficient,kazemi2015growing,yacsar2018iterative,zhou2016cross}
are all limited by solely looking at local information.

In approximate isomorphic mapping, it has been focused on maximizing the number of matched edges
\cite{singh2008global, klau2009new, zhu2013high}; and  \cite{mohammadi2017triangular} considers to maximize the number of matched triangles. A more related work \cite{zhu2013high} to ours is to first generate anchors and then extend the anchors to identify an approximate mapping.
It is quite slow as is demonstrated by our experiments. %Here,  \cite{zhu2013high} is closely related to our work.

In our experiments, we compare our techniques with the state-of-the-art techniques \cite{kazemi2015growing,yacsar2018iterative,zhou2016cross,zhu2013high}. 
The extensive experiments demonstrate that our algorithms significantly outperform these techniques. We did not compare \cite{korula2014efficient} since the authors in
 \cite{kazemi2015growing} already showed the advantage of EWS against \cite{korula2014efficient}.


%ou
%
%extend The anchor expansion algorithm in is similar to PGM. It measures the similarity of a pair of vertices by comparing the degree sequences of their 2-neighborhood subgraphs.
%However, this method is inefficient, as generating the 2-neighborhood subgraphs of all vertices takes $O(|V||E^{(3)}|)$ time where $|E^{(3)}|$ is the number of non-zero entries in $\sum_{i=1}^3{A^i}$ ($A$ is the adjacent matrix of the graph), and is ineffective, because the degree sequence of a subgraph cannot fully reflect the local structural information.
%It is found that \cite{zhu2013high} can be transferred into a PGM framework when a set of seed matches are provided ahead. To measure the similarity of a pair of vertices, it exploits high order structural information by comparing the degree sequences of their 2-neighborhood subgraphs. However, such a method is inefficient, as generating the 2-neighborhood subgraphs all vertices takes $O(|V||E^{(3)}|)$ time where $|E^{(3)}|$ is the number of non-zero entries in $\sum_{i=1}^3{A^i}$ ($A$ is the adjacent matrix of the graph), and is ineffective, as the degree sequence cannot fully reflect the local structural information.


==> 2relatedwork.tex <==
% high order may be not good.
% abstract local information -> higher-order
\section{Related Work}


%(1) matching based on isomorphic. (2) matching with ground truth.
%measurement of quality.
%isomorphic matching: (1) number of conserved edges \cite{singh2008global, zhu2013high} (2) number of conserved triangles \cite{mohammadi2017triangular} (no seed, 3-tensor, Maximum-weight-matching)
%ground truth matching: PGM algorithm. \cite{wang2018deepmatching}

Given two graphs $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$, the graph matching aims to build a bijection $M$ between $V_1\rightarrow V_2$ s.t. each pair of vertices $[u,v]$ where $u\in V_1$ and $v\in V_2$ corresponds to the same entity.
The graph matching problem is a generalization of the classic isomorphic mapping problem, the exact solution to which is NP-hard in general \cite{lewis1983computers}.
In approximate graph matching, some works aim to maximize the number of conserved edges
\footnote{For a matching $M$ on two graphs $G_1(V_1,E_1)$ and $G_2(V_2, E_2)$, the number of conversed edges is defined by $\sum_{[u_1,v_1],[u_2,v_2]\in M}{I((u_1,u_2)\in E_1)\times I((v_1,v_2)\in E_2)}$.} 
\cite{singh2008global, klau2009new, zhu2013high}, or further concerns the number of conserved triangles \cite{mohammadi2017triangular}.
While another series of works concern how matching result corresponds to the ground-truth \cite{kazemi2015growing, zhang2015cosnet, zhou2016cross, wang2018deepmatching}.


%(2) application

%From \cite{kazemi2015growing}
%social network, de-anonymization: \cite{backstrom2007wherefore, mislove2010you, narayanan2009anonymizing, pedarsani2011privacy, wondracek2010practical}
%    \cite{ji2016seed} provides quantification of prefect de-anonymizability, which requires $\Omega{\frac{1}{p p^3_e}}$ seeds (like $0.2n$).
%reconciliation of networks from different domains: \cite{korula2014efficient, yartseva2013performance} link-prediction: \cite{zhang2017link}
%biology, alignment of protein interaction networks:  \cite{klau2009new, singh2008global, mohammadi2017triangular}
%?compute vision, find similar images??: \cite{egozi2013probabilistic, torresani2008feature, wiskott1997face}

% In systems biology, complex biological systems are often modeled as networks. Examples include protein-protein interaction (PPI), metabolic, gene-regulatory, and signal transduction networks. The increasing quality and quantity of available data creates the need for automated analysis methods to better understand cellular processes, network organization, evolutionary changes, and disease mechanisms [1, 2]. Based on the assumption that evolutionary conservation implies functional significance, comparative approaches may help improve the accuracy of data, elucidate protein pathways and complexes, generate, investigate, and validate hypotheses about the underlying networks, and transfer functional annotations.

Graph matching has been widely used as a building block in various applications.
In systems biology, the alignment of protein-protein interaction networks can reveal the functional equivalences of proteins in different species \cite{singh2008global, klau2009new, mohammadi2017triangular}.
In social network, in order to support the cross-community analysis, the network reconciliation is often required which aims to identify users across different communities \cite{zafarani2009connecting, yartseva2013performance, korula2014efficient};
an emerging structure-based de-anonymization attacks have also been experimentally demonstrated to break the privacy of social networks \cite{backstrom2007wherefore, narayanan2009anonymizing, mislove2010you, wondracek2010practical, pedarsani2011privacy, ji2016seed}.




%(3) labelled graph matching

% why we study unlabelled graph matching:
% users¡¯ information in different networks is very unbalanced
% the label information is often unavailable
% the structural information is more reliable (ref. EWS)
% the structure-based method can be extended to solve labelled graph matching.


In the context of network de-anonymization or network reconciliation, a set of works extract information about user identities (e.g., username, description, location and profile image), and match graph by exploiting both structural information and semantic features \cite{malhotra2012studying, nunes2012resolving, zhang2015cosnet}. We study the structure-based graph matching for the following reasons:
the semantic features are often unavailable in the matching of networks \cite{singh2008global, mohammadi2017triangular};
%the semantic information across different networks can be very unbalanced \cite{zhang2015cosnet};
it has been shown structural information is the most important feature to identify a node in network \cite{henderson2011s};
the techniques based on semantic features may be fragile w.r.t. malicious users with fake profiles. 
Nevertheless, the content-based techniques can be combined with the structure-based matching algorithms to improve the matching performance.


%(4) Seed selection or graph matching without seeds.

% From \cite{zhu2013high}, the propagation-based works former to \cite{singh2008global}:
% Similarity flooding: a versatile graph matching algorithm and its application to schema matching.
% Authoritative sources in a hyperlinked environment.
% A measure of similarity between graph vertices: Applications to synonym extraction and web searching
A class of graph matching algorithms, assuming no apriori knowledge of the alignment, firstly compute the similarity of each pair (all similarities are often represented by a $|V_1|\times |V_2|$ similarity matrix) and then identify the alignments with high scores.
\cite{singh2008global} builds the similarity matrix by iterative weighted propagation.
%\cite{singh2008global} builds a similarity matrix by iterative weighted propagation, which can be solved by eigen decomposition. The iteration process can also incorporate other kind of similarity definition, like BLAST similarity score.
\cite{zhu2013high} concerns both global vertex similarity $S_g$, defined by the similarity of corresponding eigenvectors from the spectral clustering, and local vertex similarity $S_{\ell}$, defined by the similarity of degree sequences of 2-neighborhood subgraphs.
%where $S_g$ is defined by the similarity of corresponding eigenvectors w.r.t. normalized Laplacian matrices of two graphs and $S_l$ is defined by the similarity of degree sequences of the corresponding 2-neighborhood subgraphs.
%\cite{zhu2013high} Define global vertex similarity $S_g$ by the dot product of eigen vectors, and local vertex similarity $S_l$ by the similarity of degree sequences for 2-neighborhood subgraphs. Then vertex similarity $S=S_g\cdot S_l$. Greedily find the initial seeds, and propagate neighboring pairs as matches based on $S_l$.
\cite{wang2018deepmatching} instead uses deep-walk graph embedding to compute the low-rank representation of each vertex and then adopts Coherent Point Drift (CPD) method to build the similarity matrix. %It also considers local edge consistency in identifying matches.

%(5) Seed graph matching. percolation
The seeded graph matching problem studied in this paper, however, assumes a small set of ``pre-matched'' vertex pairs (seed matches) are provided at the beginning.
The seed matches can be obtained either by public link information, e.g., users may connect their accounts of different social networks \cite{zhang2015cosnet},
or by existing seed identification methods \cite{singh2008global, zhu2013high, wang2018deepmatching}.
A popular class of works, which are most related to ours, are referred as to Percolation Graph Matching (PGM). %The PGM always matches the neighbors of seed matches and thus achieves great efficiency.
% If neighboring pair is defined in the introduction. Then omit the following definition.
%For a pair $[i,j]$, where $i\in V_1,j\in V_2$,  we say $[i',j']$ is its neighboring pair if $(i,i')\in E_1$ and $(j,j')\in E_2$.
PGM maintains a set of matched pairs which consists of the seed pairs in the beginning, then adds new matches iteratively.
The neighboring pairs of matched pairs are examined by certain criteria and matched if they are qualified.
Whether to match a pair $[i,j]$, the PGM algorithms mainly concern the number (denoted as $r$) of its neighboring pairs that have already been matched. If the $r$ is above a given threshold $k$, the pair is added to the matched set~\cite{yartseva2013performance}. When there are multiple qualified candidates, additional rules are used for tie breaking, e.g.,~\cite{korula2014efficient} prefers the vertices of high degrees,~\cite{zhou2016cross} matches the vertex pairs with the maximal $r$. %and~\cite{kazemi2015growing} always selects the vertex pair with minimal degree difference.
Despite of the guaranteed high precision as a result of strict matching criteria, 
the traditional PGM methods often suffer from early-stop (low recall), especially when only a small number of seeds are provided.
To prevent to early termination, recently, ~\cite{kazemi2015growing} proposes a new strategy, namely ExpandWhenStuck (EWS), which collects the vertex pairs that haven't meet the matching criteria into a \emph{noisy set}, and allows this set of pairs to percolate. 
The PGM algorithms only concern the order-1 structural information (or order-2 structural information by EWS) of candidate pairs, thus cannot capture and measure the higher-order structural difference.
Different from PGM, more recently, \cite{yacsar2018iterative} proposes to map vertices of two graphs into the same 2-D space by using their shortest path distances to seeds, and considers cross-graph vertex pairs located in the same region. Besides, \cite{yacsar2018iterative} measures the similarity of each vertex pair by combining \emph{matched neighbor similarity}, defined by the ratio of $r$ to the number of matched vertices in $N(i)\cup N(j)$, with \emph{relative degree distance} \cite{koutra2013big}, and greedily matches vertex pair with the highest similarity each time. 
Note that \cite{yacsar2018iterative} uses the global structure-assist (i.e.) to reduce the number of vertex pairs that should be measured while still considers order-1 structural information only in measuring each pair.
It is found that \cite{zhu2013high} can be transferred into a PGM framework when a set of seed matches are provided ahead. To measure the similarity of a pair of vertices, it exploits high order structural information by comparing the degree sequences of their 2-neighborhood subgraphs. However, such a method is inefficient, as generating the 2-neighborhood subgraphs all vertices takes $O(|V||E^{(3)}|)$ time where $|E^{(3)}|$ is the number of non-zero entries in $\sum_{i=1}^3{A^i}$ ($A$ is the adjacent matrix of the graph), and is ineffective, as the degree sequence cannot fully reflect the local structural information.
Thus, this paper exploits the high order structure information in graphs and proposes an efficient and effective seeded graph matching algorithm. 
%\cite{zhu2013high}
%fully match in each iteration based on local vertex similarity
%\cite{yartseva2013performance}
%If the $r$ is above a given threshold $k$, the pair is added to the matched set.
%\cite{korula2014efficient}
%additional rules: prefer the vertices of high degrees
%\cite{zhou2016cross}
%additional rules: matches the vertex pairs with the maximal $r$
%\cite{kazemi2015growing}
%noisy percolation.
%additional rules: always selects the vertex pair with minimal degree difference.



==> 3labelling.tex <==
% stressing on PPR labelling may not be good, as we cannot prove its power.
% the model based on random walk is simpler. Turn to PPR for efficiency.

\section{Personalized PageRank in Graph Labelling} \label{3PPR}

Personalized PageRank has been extensively adopted in graph structure analysis, such as community detection~\cite{avron2015community}, graph ordering~\cite{benson2016higher, yin2017local}, and other applications~\cite{gleich2015pagerank}. The Personalized PageRank value plays different roles in various phenomena, such as denoting the local range or measuring the importance of nodes. In this paper, we exploit the power of personalized PageRank in graph labelling.

Given a set of seeds $S$ on graph $G$, we conduct a personalized PageRank approximation on each seed $s_k$ (as the source) by using the Forward-Push with the same stopping probability $\alpha$ and the same residue threshold $r_{max}$. The PPR value of node $i\in V$ w.r.t. $s_k$ is $\pi(s_k, i)$, and the PPR vector of node $i$ is $R(i) = \{\pi(s_1, i), \pi(s_2, i), \cdots, \pi(s_{|S|}, i) \}$. We take the PPR vector as the global label for each node. It can be shown the PPR vector of each node illustrates both its region information and local structure information in Appendix~\ref{7ppr}.

\subsection{PPR labelling} \label{3labelling}

\subsection{Properties of PPR labelling} \label{3property}
Then we will show the PPR vector of each node illustrates its region information and local structure information.
The PPR value $\pi(s_k, i)$ of node $i$ can be decomposed into two parts:
(i) the probability that a decaying random walk terminates at node $i$ the first time it arrives at $i$, denoted by \textbf{$\pi_1(s_k, i)$};
(ii) and the probability that a decaying random walk terminates at node $i$ after its arriving node $i$ for the first time, denoted by \textbf{$\pi_2(s_k, i)$}.

Following the analysis in Section~\ref{2PPR}, we denote $LS(i) = [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i$ the probability that a decaying random walk which starts from $i$ returns node $i$ after step $1,2,3 \cdots$, then
\begin{equation}\label{LS}
\pi_2(s_k, i) = \pi_1(s_k, i) \times LS(i).
\end{equation}
Thus the PPR value $\pi(s_k, i)$ can be presented by
\begin{equation}\label{PPR3-math}
\begin{split}
\pi(s_k, i) = \pi_1(s_k, i) +\pi_2(s_k, i) & = \pi_1(s_k, i) + \pi_1(s_k, i)\cdot LS(i) \\
                                            & = \pi_1(s_k, i) \cdot(1+LS(i)).
\end{split}
\end{equation}


Note that  $\frac{\pi_1(s_k, i)}{\alpha}$ represents the summed probability that a decaying random walk from $s_k$ hits node $i$ for the first time at iteration $0, 1, 2\cdots$. With a sufficient number of source nodes, apparently, the region information of node $i$ can be represented in a way by all hitting probabilities.
To be more specific, given a number of correct seed matches as the source nodes on two aligned graphs, with high probability $i\in V_1$ and $j\in V_2$ are on the aligned region over two graphs if and only if they have similar hitting probability vector, i.e., $\frac{\pi^1_1(s^1_k, i)}{\alpha}$ and $\frac{\pi^2_1(s^2_k, j)}{\alpha}$ should be relatively close w.r.t. a certain number of seed pair $[s^1_k, s^2_k]$.

Recall that $LS(i) = [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i$ is independent of the source node, but relevant to node $i$ and graph $G$.
$LS(i)$ demonstrates the local structure information of each node, and the nodes of similar local structures tends to have close $LS(i)$ value.
For instance, consider the probability that a random walk arrives at $i$ at the first two iterations, we denote it by $LS^{(2)}(i)$. Since there is no self loop in graph, a random walk from $i$ cannot return to $i$ at the $1^{st}$ iteration, then we have
\begin{equation}
\begin{split}
LS^{(2)}(i) & = [(1-\alpha)^{2}\cdot P^{2}\cdot e_i]_i  \\
            & = (1-\alpha)^{2}\cdot \frac{1}{|N(i)|} \sum_{(i,j)\in E}\frac{1}{|N(j)|}
\end{split}
\end{equation}
where $|N(j)|$ is the degree of node $j$. Thus $LS^{(2)}(i)$ represents the average reciprocal of degree of all neighbors of node $i$, containing the second-order local structure information.
Accordingly, the arriving probability of further iterations $LS^{(k)}(i)$ contains the higher-order local structure information of node $i$, the impact of which, however, is decayed by the factor $1-\alpha$ over iterations.



\subsection{Stopping Probability $\alpha$ in PPR}  \label{3alpha}

The stopping probability of random walk in PageRank often varies in different cases. A discussion has been presented in~\cite{gleich2010inner}.
Most works on web search~\cite{kamvar2003extrapolation, najork2007hits} adopt the high stopping probability ($\alpha=0.95$ or $0.9$) thus the power method can converge fast.
\cite{avrachenkov2007distribution} selects small stopping probability ($\alpha = 0.5$), as it prevents the Pure-Out nodes (which have links from the strongly connect components but not back) from having very large PageRank values.
We also set a small $\alpha$ (empirically $1-\frac{\sqrt{2}}{2}\approx 0.3$) in this paper, but for a different reason.

In graph labelling, the choice of $\alpha$ corresponds to the biases on either the region information ($\pi_1(s_k, i)$) or the local structure information ($LS(i)$).
With a very high value of $\alpha$, the PPR values of nodes are highly distinguished on the hitting probability of the random walk, i.e., the nodes near to the source node tend to have large PPR values; and the algorithm conducts much more forward-push iterations on these nodes with high PPR values. But in this case, the algorithm is sensitive to the unaligned structures in two network graphs.
While the low value of $\alpha$ shows a bias on the nodes' local structure information. Thus we empirically use $\alpha=0.3$ to balance the two kinds of biases and make labelling be robust to the cross-network unaligned structures.

%\textbf{Puzzle:} The setting of Residue threshold with respect to different stopping probability is still a mystery$\cdots$ May relevant to the size of datasets, the property of dataset graph, the number of seeds, and so on. Waiting the results of experiments on data sets.
%
%Results of exp: set all $\alpha=0.3$. For social network with a large number of triangles (facebook and twitter), $r_{max}=1e-6$; for others (Email and sx-mathflow) with fewer triangles, $r_{max}=1e-5$.
%Likely for graphs with more triangle, the PPR residue decays fast with respect to distance, thus use smaller $r_{max}$.
%Now we think twitter with more triangles should use larger $r_{max}$ (1e-5~1e-6) than amazon with fewer triangles (1e-7+).



==> 3preliminaries.tex <==
\section{Preliminaries} \label{sec2}


\subsection{Graph notation} \label{2Graphs}
Consider two undirected graphs $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$ to be matched.
%let $V_0 = V_1 \cap V_2$. Let $n_1 = |V_1|$, $n_2 = |V_2|$ and $n_0 = |V_1 \cap V_2|$.
We use $(i,j)\in E_{1} (E_2)$ to denote an edge between two $i,j$, and $[i,j]$ to represent a pair of nodes where $i \in V_1$ and $j\in V_2$. Let $N(i)$ be the neighbors of node $i$. The neighboring pairs of a pair $[i,j]$ is the set of all pairs $[i', j']\in V_1 \times V_2$ such that $(i, i')\in E_1$ and $(j, j') \in E_2$, which is exactly $N(i)\times N(j)$. We use $N(i,j)$ to denote the set of neighboring pairs of $[i,j]$.  The initial seed set is $S=\{[s^1_1, s^2_1], [s^1_2, s^2_2], ..., [s^1_{|S|}, s^2_{|S|}]\}$, where $s^1_k \in V_1$ and $s^2_k \in V_2$ for all $k$.

An undirected graph $G$ can be represented by an adjacency matrix $A$, where $A_{ij} =1$ if $(i,j)\in E$ and $A_{ij}=0$ otherwise. Note that $A$ is symmetric matrix since $G$ is undirected.
%Let $|N(i)|=\sum_{j\in V}{I((i,j)\in E)}$ be the number of neighbors of node $i$.
The probability transition matrix $P$ defined on $G$ is given by
\[
    P_{ji}=
\begin{cases}
    \frac{1}{|N(i)|} & \text{if } (i,j)\in E,\\
    0              & \text{otherwise.}
\end{cases}
\]
We use $[\boldsymbol{x}]_i$ to denote the $i^{th}$ value of the vector $\boldsymbol{x}$.



\subsection{Personalized PageRank} \label{2PPR}

Personalized PageRank has been extensively adopted in graph structure analysis, such as community detection~\cite{avron2015community}, graph ordering~\cite{benson2016higher, yin2017local}, and other applications~\cite{gleich2015pagerank}.

Given a source node $s\in V$ and a stopping probability $\alpha$ (also referred to as decaying factor in the literature), a random walk with restart from $s$ is a traversal of $G$ that starts from $s$ and, at each step, either (1) terminates at the current node with probability $\alpha$, or (2) proceeds to a randomly selected neighbor of the current node. For any node $i\in V$, its personalized PageRank value $\pi(s,i)$ with respect to source $s$ is the probability that a random walk from $s$ terminates at $i$.
%In this paper, we always use the same stoping probability $\alpha$ for all PPR computations.
%Given a seed pair $[s^1_k, s^2_k]\in S$ on $G_1$ and $G_2$, we let $\pi(s^1_k, i)$ represent the PPR value of node $i\in V_1$ w.r.t. source node $s^1_k$,
%and $\pi(s^2_k, j)$ represent the PPR value of node $j\in V_2$ w.r.t. source node $s^2_k$.
For a pair $[i,j]$, let $R^1(i) = \{\pi(s^1_1, i), \pi(s^1_2, i), ..., \pi(s^1_{|S|}, i) \}$ 
and $R^2(j) = \{\pi(s^2_1, j), \pi(s^2_2, j), ..., \pi(s^2_{|S|}, j) \}$ be the PPR vectors of $i\in V_1$ and $j \in V_2$ respectively.

Starting from $s_k$, let $p_i^{(t)}$ be the probability that the (non-decaying) random walk reaches node $i$ after $t$ steps. Since probability that the random walk doesn't stop before step $t$ is $(1-\alpha)^t$, the probability that the decaying random walk reaches node $i$ in the $t^{th}$ step is
$$r_i^{(t)} = (1-\alpha)^t p_i^{(t)}.$$
Such probabilities can be represented in matrix forms. Let $e_{s_k}\in \real^{|V|\times1}$ be the  $s_k^{th}$ standard basis vector, i.e. with $1$ at $s_k^{th}$ position and $0$'s everywhere else. %representing the initial state.
Let $P$ be the transition matrix defined in Section~\ref{2Graphs}, then
\begin{equation}\label{rit}
r^{(t)}_i = [(1-\alpha)^{t}\cdot P^{t}\cdot e_{s_k}]_i.
\end{equation}
Hence, the PPR value of node $i$ w.r.t. source node $s_k$ is
\begin{equation}\label{PPR-math}
\begin{split}
\pi(s_k, i) = \alpha\cdot\sum_{t=0}^{\infty}r^{(t)}_i &=\alpha\sum_{t=0}^{\infty}(1-\alpha)^t p_i^{(t)}\\
														&= \alpha \sum_{t=0}^{\infty}[(1-\alpha)^{t}\cdot P^{t}\cdot e_{s_k}]_i\\
                                                      %&= [\sum_{t=0}^{\infty}(1-\alpha)^{t}\cdot P^{t}\cdot \alpha e_{s_k}]_i\\
                                                      &=[(I-(1-\alpha)P)^{-1}\cdot (\alpha e_{s_k})]_i,
\end{split}
\end{equation}
where $I\in \real^{|V|\times |V|}$ is the identity matrix.
%Computing the exact PPR value takes $O(n^3)$ time, dominated by the time complexity of doing matrix inversion.

There are two classes of algorithms for approximating personalized PageRank, based on Forward-Push and Monte-Carlos sampling respectively.
%Recently,~\cite{wang2017fora} proposed a two-stage method FORA that runs Monte-Carlos sampling after doing Forward-Push, and approximates the PPR value with guaranteed relative error efficiently.
In PPRGM, we adopt the Forward-Push algorithm (see Algorithm~\ref{alg:FP}), for the following reasons: (1) It is simple and efficient; (2) It is deterministic; (3) The accuracy of Forward-Push is controlled by the residue threshold, which is more suitable for our purpose.
% it is unnecessary to pursue the PPR approximation of high quality due to the natural robustness of graph matching problem.


\begin{algorithm}[!tb]
\caption{Forward-Push method}\label{alg:FP}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input {$G(V, E)$, source node $s$, stopping probability $\alpha$, residue threshold $r_{max}$}
    \Output {$\pi(s, i)$ for all nodes $i\in V$}

    set $r(s, s)=1$, and $r(s,i)=0$ for all nodes $i\ne s$;

    set $\pi(s, i)=0$ for all $i\in V$.

    \While{$\exists i\in V$ such that $r(s,i)/|N(i)| > r_{max}$}{
        $\pi(s,i) = \pi(s,i)+\alpha\cdot r(s,i)$;

        \ForEach {$j\in N(i)$}{
            $r(s, j) = r(s,j) + (1-\alpha)\cdot \frac{r(s,i)}{|N(i)|};$
        }

        $r(s,i)=0;$
    }
\end{algorithm}

Here we introduce the Forward-Push method in more detail as it will be helpful to understand our main algorithm (see Algorithm~\ref{alg:FP}).
%The algorithm takes graph $G$, source node $s$, stopping probability $\alpha$, and a residue threshold $r_{max}$ as the input, and outputs the $\pi(s,i)$ for each node $i$.
The algorithm starts a PPR approximation on source node $s$, and two variables are defined on each node: (1) the reserve $\pi(s,i)$ represents the current estimation of the probability that a random walk terminates at node $i$ (i.e. the PPR value), which is always an underestimation; (2) and the residue $r(s,i)$ represents the approximation of the probability that the random walk is currently at node $i$.
%which may terminate at $i$ or move to a neighbor at the next step.
Note that $\sum_{i\in V}{\pi(s,i)}+\sum_{i\in V}{r(s,i)}=1$ holds at all times (the intuitive explanation is that the random walk either has terminated at some node or is currently at some node).
Initially $r(s,s)$ is set to $1$ while $\pi(s,i)=0$ for all $i\in V$, and the algorithm iteratively increases $\sum_{i\in V}{\pi(s,i)}$ to have better approximations to the PPR values. 
In each iteration, the algorithm finds a node $i$ with $r(s,i)/|N(i)|>r_{\max}$, then distributes the value of $r(s,i)$ to $i$'s neighbors: (1) it increases the reserve $\pi(s,i)$ by $\alpha\cdot r(s,i)$ (line 4); (2) it adds $(1-\alpha)\cdot \frac{r(s,i)}{|N(i)|}$ to each residue $r(s,j)$ for $j\in N(i)$ (line 5-7); (3) $r(s,i)$ is set to $0$.
The algorithm terminates if there is no node $i$ s.t. $r(s,i)/|N(i)|>r_{max}$. When there are multiple nodes satisfying the condition in line 3, we always pick the node $i$ with \emph{maximum} $r(s,i)/|N(i)|$ in our implementation, thus the number of iterations is greatly reduced as each iteration makes the most progress.

%The Forward-Push keeps all $\pi(s,i)$ as the approximations of the PPR values, while abandons all $r(s,i)$, the uncertainty part of the random walk.
Since the approximate PPR values are always underestimates, the smaller the total residue $\sum_{i\in V}{r(s,i)}$ is, the better the approximations are, while the total residue at the end is controlled by the residue threshold $r_{\max}$.

\subsection{Graph Matching and PGM algorithms} \label{2PGM}
A general way for matching graphs is to first assign each possible pair a \emph{matching score}, and then find a matching $M$ with maximum total scores, which can be casted as a Maximum Weight Bipartite Matching problem~\cite{cheng1996maximum}. However, it is highly nontrivial to design a good mechanism for measuring matching scores. Even if the scores are determined, computing a maximum matching is still time-consuming on large graphs.
%The task of seeded graph matching includes two parts: generating candidate pairs and doing matching.
%Consider two graphs $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$, $V_1 \times V_2$ is the set of all possible pairs.
% The size of problem even grows when multiple graphs are concerned.
There are a few works which directly examine and prune the whole set $|V_1| \times |V_2|$~\cite{lyzinski2017graph, lyzinski2014seeded, vogelstein2011fast, ji2016seed}, but are still impractical when the graphs are extremely large.

\noindent
\textbf{Candidate generation.}
The class of PGM algorithms instead iteratively generate candidate pairs by a percolation process and merely store and examine those candidates, which are more efficient in terms of space and time.
%the candidate pair set is generated incrementally: (1) at the beginning, each seed pair $[i,j]\in S$ percolates to its neighboring pairs, i.e., all $[i',j']\in N(i,j)$, and adds them into a candidate set $C$; (2) at each round, each candidate pair $[i,j]\in C$ that is matched based on some rules is added to the match set $M$; (3) each pair $[i,j]\in M$ that has not percolated before percolates to its neighboring pairs, and adds them into a candidate set. The process (2)(3) repeats until the seed set is empty and all candidate pairs are unqualified to be matches.
%Recent variations like ExpandWhenStuck (EWS)~\cite{kazemi2015growing} also expands the candidate pairs as the \emph{noisy seeds} when the seed set is exhausted, and has the noisy seed percolate to its neighboring pairs. This strategy effectively prevents the early-stop of traditional PGM algorithms and has strong robustness.

%However, the candidate generations of PGM algorithms suffer from the dependency of matching results: a pair is inserted into candidate set as the neighboring pair of matches or noisy seeds, i.e., it iteratively explores the first order unknown structure, thus a wrong match in an early stage may lead to the miss of true candidate pair.
\noindent
\textbf{Matching pairs.}
%To find a good matching, the algorithm assigns each candidate pair a \emph{matching score}. Note the graph matching problem can be transformed into Maximum Weight Bipartite Matching problem~\cite{cheng1996maximum}, if both the candidate set and the corresponding scores can be determinate ahead.
%A general way of doing matching is to assign each candidate pair with a $score$, and find a match set $M$ such that each node is matched at most once and the overall score is maximized. It's worth mentioning that such a problem can be transformed into Maximum Weight Bipartite Matching problem~\cite{cheng1996maximum} only if both the candidate set and the corresponding scores are determinate ahead.
The matching scores in PGM are also updated dynamically. Existing PGM algorithms often use the number of neighboring pairs that have been matched in previous round as the score of a pair. This is quite natural and effective, as a newly matched pair provides additional evidence for matching other pairs.
% i.e., $\mathtt{Score(i,j)}=\sum_{(i',i)\in E_1, (j',j)\in E_2}{I([i',j']\in M)}$.
%There is no trivial way to find a matching solution with the maximum summed scores, as in Maximum Weight Bipartite Matching problem, because the candidate set and the corresponding scores in PGM are both dynamic. Instead, the PGM exploits an efficient greedy strategy by matching a pair whenever its score reaches a predefined threshold (or meet additional criteria).


==> 4approx_-_Copy.tex <==



\section{PPRGM Algorithm}\label{4approx}

%The core idea of PPRGM is to build the connection between each matched vertex and the vertex to be matched with personalized PageRank. Based on PPR values, we propose a function
%which measures the matching score of a pair $[v,u]\in V_1\times V_2$ by comparing the PPR values of $v$ and $u$ with respect to each matched pair of vertices $s$ and $s'$ respectively.
%provide a function to measure the matching score of each candidate pair by comparing their PPR values with respect to the matched pairs including the seed pairs (i.e., compare two vectors of PPR values).
%We first provide the function that is used in our algorithm to measure the matching scores of a pair, which is a function of the PPR vectors of  two vertices. %The score of a pair represents the likelihood of its being matched.

%  percolation framework + use matched vertices + matching criteria + forward push + matching score.

%In this section, we present the details of our Personalized PageRank based Graph Matching framework (PPRGM).
To improve the time efficiency, we do not compute all PPR values and matching scores in the beginning. Instead, PPRGM adopts a greedy expansion mechanism similar to the percolation process in PGM to generate candidates iteratively; only the matching scores of these candidate pairs will be computed. During this process, candidate pairs that satisfy certain criteria are marked as \emph{matched} and will be output as valid matches. To resolve the second issue mentioned above, in addition to the initial seeds, the matching score of a candidate pair will be augmented by the information of early matches. More precisely, the matching score of a candidate pair is now the summation of the score w.r.t. initial seeds and the score w.r.t. earlier matches that are added by the algorithm.

%It also exploits the vertex pairs matched by the algorithm to boost the matching precision.
%Practical matching criteria are designed on PPRGM to further improve the matching precision.
%Motivated by the observation that an evidence based on longer random walks is less reliable, we then propose to use a truncated random walk in building the connection between vertices,
%and accordingly, amend the matching score function to improve its robustness against small PPR values.
%Lastly, we provide an analysis on the effectiveness of the PPRGM algorithm.


%  forward push + matching score + percolation framework + use matched vertices + matching criteria
%
%In this section, we present the details of Personalized PageRank based Graph Matching framework (PPRGM).
%Motivated by the fact that longer random walks are more sensitive to
%structural differences and are less reliable, we propose to use a truncated random walk in building the connection between vertices,
%
%XXX Forward-Push mush be based using matched vertices. expansion strategies. great computational efficiency.
%
%Accordingly, we amend the former matching score function to improve its robustness, with reason explained.
%Additionally, rather than measuring all $|V_1|\times |V_2|$ candidate pairs,
%the PPRGM adopts an efficient percolation mechanism to generate candidates  and proposes to exploit the vertex pairs matched by the algorithm to boost the matching.
%Practical matching criteria %strategies
%to further improve the matching precision are also raised.
%Lastly, we provide an analysis on the effectiveness of the PPRGM algorithm.


\subsection{Main Framework}\label{32PPRGM}
To generate candidates, we use a similar idea as in PGM. Given any matched pair $[s,s']$ (either a seed or an early match), the hypothesis adopted by PGM is that the neighboring pairs of $[s,s']$ are more likely to be valid matches. So, in each iteration, PGM simply adds the neighboring pairs of any newly matched pair as candidates.  %of a matched pair $[s,s']$ as candidates.
In our PPRGM framework, we propose more general and effective strategies for generating candidate pairs.
% not sure yet any proof for PGM: Pr of true pairs included
%
%An idea of candidate pairs pruning (or candidate generation) comes directly from the class of PGM algorithms,
%which always takes each $[v,u]\in N(s,s')$ as candidate pair for each $[s,s']$ that has been matched.
%It is observed that the mechanism of percolation achieves great effectiveness in seeded graph matching, because
%(1) if $[s,s']$ is a correct match, then the correct match to each vertex $v\in N(s)$ is likely included by $N(s')$;
%(2) a vertex $v$ is measured to $u$ only if a vertex $s\in N(v)$ is matched to $s'\in N(u)$.
%Consequently, the total number of candidates is significantly reduced while each correct match still has large chance to be measured as a candidate. %(depend on the matching precision)
%
%We also propose to use the pairs matched during the matching process to further boost the matching precision.

%The core idea of the new graph matching framework is to use vertex pairs matched during the matching process to further boost the matching,
%which comes directly from the class of PGM algorithms. % which is exactly the main principle of  the class of PGM algorithms
%Firstly, we generate new candidate pairs based on the pairs that have been matched,
%we conduct candidate generation (or candidate pairs pruning w.r.t. the whole $|V_1|\times|V_2|$ set) based on the pairs that have been matched,
%e.g., assume a set $M$ is used to store all the initial seed pairs and the pairs matched by the algorithm,
%we can takes each $[v,u]\in N(s,s')$ as a candidate pair for each $[s,s']\in M$.
%It is observed that the mechanism of percolation achieves great effectiveness in seeded graph matching, because

%The mechanism of percolation achieves great effectiveness in candidate generation for seeded graph matching, because
%(1) if $[s,s']$ is a correct match, then the correct match to each vertex $v\in N(s)$ is likely included by $N(s')$;
%(2) a vertex $v$ is measured to $u$ only if a vertex $s\in N(v)$ is matched to $s'\in N(u)$.
%Consequently, the total number of candidates is significantly reduced while each correct match still has large chance to be measured as a candidate. %(depend on the matching precision)
%Secondly, we also exploit the pairs matched during the matching process as the new evidences in later matching. We can simply take the set $M$ as an \emph{extended seeds set} (though the pair matched later should have less credibility than the initial seeds, which will be discussed Section~\ref{42expansion}).
%Thus, similarly, the connection between each matched vertex $s$ and the vertex $v$ to be matched is quantified by the PPR value $\pi(s,v)$,
As discussed above, the matching score of a candidate pair $[v,u]$ w.r.t. each matched pairs $[s,s']$ will be computed according to~\eqref{ep_score1}. Assuming $M$ is the set of all the initial seed pairs and the pairs matched by the algorithm, then the matching score of $[v,u]$ is computed by $\mathtt{Score}_M(v,u) = \sum_{k=1}^{|M|} \mathtt{Score}_k(v,u)$.
\begin{algorithm}[!tb]
\caption{Personalized PageRank based Graph Matching (PPRGM)}\label{alg:PPRGM}
%\begin{algorithmic}[1]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input {$G_1(V_1, E_1), G_2(V_2, E_2)$, set $S$ of seed matches, stopping probability $\SP$.}
    \Output {The set of matched pairs $M$.}

    Let $C\leftarrow\Emptyset$ store the candidate pairs; \\ %let $Q\leftarrow\Emptyset$ store candidate pairs that satisfy matching criteria; \\

    Let $M'\leftarrow\Emptyset$ store the pairs that are matched but have not been added to $M$;

    \ForEach {seed pair $[s_k, s'_k]\in S$}{
       Insert $[s_k, s'_k]$ into $M'$; mark $s_k, s'_k$ as matched;\\
    }


    \While{$True$}{
        \ForEach {pair $[v,u]\in M'$}{
            Insert $[v,u]$ into $M$;\\
            \textbf{Neighbor-Expansion($v, u, C$)};\\
    		%Compute PPR on $G_1$ using source node $v$;\\
            %Compute PPR on $G_2$ using source node $u$;\\
    	}
       % \ForEach {pair $[v,u]\in M'$}{
%            \textbf{Neighbor-Expansion($v, u, C$)};
%        }

        $M'\leftarrow\Emptyset$. \\
        \ForEach {$[v,u]\in C$ satisfying matching criteria}{
           % \If {$v$ and $u$ are not unmatched}{
           %\ForEach {$[v,u]\in Q$}{
                Insert $[v,u]$ into $M'$; mark $v, u$ as matched;\\
                Remove pairs in $\{v\}\times{V_2}$ and ${V_1}\times \{u\}$ from $C$;\\
            %}
          % Insert $[v,u]$ into $Q$;\\
           % }
        }
        \If {$M'$ is empty}{%==\Emptyset$}{
            Relax the matching criteria, or break the while-loop if the matching criteria cannot be further relaxed;\\
        }
    }
    \Return {M}

\end{algorithm}

The main PPRGM framework is presented in Algorithm~\ref{alg:PPRGM}.
Given two graphs $G_1(V_1,E_1)$ and $G_2(V_2,E_2)$ and a set $S$ of seed matches.
The algorithm initializes a set $C$ to store the candidate pairs, %a set $Q$ to store the candidate pairs that satisfies certain matching criteria (which will be discussed shortly),
and a set $M'$ to store the pairs that are matched but have not been added to $M$ (line 1,2).
Firstly, PPRGM inserts each seed pair $[s_k,s'_k]\in S$ into $M'$, and marks $s_k$ and $s'_k$ as matched (line 3-5).
Then PPRGM starts a while-loop which iteratively expands the candidate set and matches vertex pairs: %on condition that $M'$ is not empty (line 6),
(1) For each pair $[v,u]\in M'$, the algorithm inserts $[v,u]$ into $M$, and calls a \emph{Neighbor-Expansion} procedure, which adds all neighboring pairs of $[v,u]$ to the candidate set $C$;
$M'$ is then set to empty (line 7-11);
(2) For each pair $[v,u]\in C$ that satisfies certain matching criteria (which will be discussed shortly), PPRGM inserts $[v,u]$ into $M'$ and marks $v$ and $u$ as matched, then the candidate pairs that belong to $\{v\}\times{V_2}$ or ${V_1}\times \{u\}$ are removed from $C$ (line 12-15). %and inserts $[v,u]$ into $Q$ (line 12-14);
 %and computes PPR on $G_1$ and $G_2$ using source node $v$ and $u$ respectively based on the same decaying factor $\SP$ (line 7-9);
%(2) PPRGM then adds the neighboring pairs ($N(v)\times N(u)$) of each $[v,u]\in M'$ to the candidate set $C$, and clears $M'$ (line 12-15);
%(3) If $Q$ is not empty, for each pair $[v,u]\in Q$, the algorithm inserts $[v,u]$ into $M'$ and marks $v$ and $u$ as matched, then the candidate pairs that belong to $\{v\}\times{V_2}$ and ${V_1}\times \{u\}$ are removed from $C$ (line 16-19); otherwise (if $Q$ is empty), the algorithm updates the matching criteria, or breaks the while-loop (line 21) if the criteria cannot be further updated. %(below a minimum requirement)

To reduce the chance of matching wrong pairs in the early stage, we introduce the \emph{postponing strategy}. Roughly speaking, we will apply more strict matching criteria in the early stage so that the decisions for matching ``uncertain" candidate pairs (in some sense) are postponed and only very strong candidate pairs are matched. However, the matching criteria will be relaxed periodically to match more pairs (line 16-18).
%Note that the matching score of a pair $[v,u]\in C$ is $Score_M(v,u)$, which is firstly computed based the current pairs in $M$, and updated when $M$ is expanded.

%We will then discuss the matching criteria for whether a candidate pair $[v,u]\in C$ should be matched.
%In PPRGM algorithm, the matching score of a candidate pair $[v,u]$ is $Score_M(v,u)$, which is computed based on ~\eqref{ep_score2} with respect to all matched pairs in $M$.

%whenever set $C$ is not empty, PPRGM greedily finds pair $[v,u]\in C$ with the highest matching score (computed based on Equation~\ref{ep_score2}) and removes $[v,u]$ from $C$. If both $v$ and $u$ are  unmatched and pair $[v,u]$ satisfies certain criteria (which will be discussed shortly), then PPRGM inserts $[v,u]$ into $M'$, and marks $v$, $u$ as matched (line 16-22).
%The criteria for whether a pair $[v,u]$ is qualified for a match will be discussed then.




%We recall that it is infeasible to find a matching solution to obtain the maximal summed score because computing the $\mathtt{PPRScore}$ for all possible pairs is costly in time (as discussed in Section~\ref{2PGM}).
%, and the score of each pair varies during the matching process.


%\begin{procedure}[!tb]
%\caption{1: Check-Strong-Candidate(C, i, j, $\beta$)}\label{proc:CSC}
%%\caption{CheckTie(set AC, set C, vertex i)}\label{proc:checkforAC}
%	\KwIn{set $C$, pair $[i,j]$, ratio $\beta$;}
%
%    \If{$\exists[i,j']\in C$ s.t. $(1+\beta)\cdot \mathtt{Score}(i,j')>\mathtt{Score}(i,j)$}
%    {
%        \Return {False;}
%    }
%    \If{$\exists[i',j]\in C$ s.t. $(1+\beta)\cdot \mathtt{Score}(i',j)>\mathtt{Score}(i,j)$}
%    {
%        \Return {False;}
%    }
%    {
%        \Return {True;}
%    }
%\end{procedure}

%[!t]
%
%
%%[!t]
%\begin{algorithm}[!tb]
%\caption{PPRGM}\label{alg:PPRGM}
%%\begin{algorithmic}[1]
%    \SetKwInOut{Input}{Input}
%    \SetKwInOut{Output}{Output}
%    \Input {$G_1(V_1, E_1), G_2(V_2, E_2)$, seed set $S$ of correct matches, stopping probability $\SP$, residue threshold $r_{max}$}
%    \Output {The set of matched pairs $M$}
%
%    initialize candidate pair set $C\leftarrow\Emptyset$, strong candidate pair set $Q\leftarrow\Emptyset$, $\beta\leftarrow2$;
%
%    \ForEach {seed pair $[s^1_k, s^2_k]$}{
%       $R^1_k$ $\leftarrow$ Forward-Push$(G_1, s^1_k, \SP, r_{max})$;\\
%       $R^2_k$ $\leftarrow$ Forward-Push$(G_2, s^2_k, \SP, r_{max})$;
%    }
%
%    insert each seed pair $[s^1_k, s^2_k]$ into $Q$;
%
%    \While{$C\ne \Emptyset$ and $\beta>1+\epsilon$}{
%    	\ForEach { strong candidate pair $[i,j]\in C$  w.r.t. $\beta$}{
%    		insert $[i,j]$ into $Q$;
%    	}
%    	\While{$Q \ne \Emptyset$}{
%    		find $[i,j]\in Q$ with highest $\mathtt{Score}(i,j)$;\\
%    		%\If {$\mathtt{Score}(i,j)<\gamma$}{
%    		%	break;
%    		%}
%    		mark $i, j$ as matched, insert $[i,j]$ into $M$;\\
%    		remove all adversary pairs of $[i,j]$ from $C$;\\ %$[i,j']$ and $[i',j]$
%            \textbf{Neighbor-Expansion($i, j$)};
%    	}	
%        update $\beta \leftarrow (\beta+1)/2$;\\
%    }
%    \Return {M}
%
%\end{algorithm}


% how to follow from the above part.
%\vspace{0.1cm}
%\noindent
\subsection{The Postponing Strategy and Matching Criteria.}
 % (line 12 in Algorithm~\ref{alg:PPRGM}).
%We additionally propose new postponing strategies to improve the matching precision:
%the match of a \emph{uncertain} pair should be postponed even if it currently has the highest score among the candidate set.
%We first introduce a few more definitions.
%\theoremstyle{definition}
We define \emph{adversary pairs} of $[v,u]$ as the set of all pairs in $\{v\}\times V_2$ and $V_1\times \{u\}$ excluding $[v,u]$, which are the direct competitors of $[v,u]$. Note that a pair will not be matched if any one of its adversary pairs is matched first. A simple idea is then to match the pairs whose adversary pairs in the candidate set all have smaller matching scores.

Suppose $[v,u]$ is a correct pair. Since the candidates are generated and matched iteratively, the following \emph{undesirable cases} may happen:

(1) $[v,u']\in C$ but currently $[v,u]\notin C$, although $\mathtt{Score}(v,u)>\mathtt{Score}(v,u')$; %and hereby $[i,j]$ is wrongly matched;

(2) $[v,u]\in C$ and $[v,u']\in C$, but currently $\mathtt{Score}(v,u')$ is slightly higher than $\mathtt{Score}(v,u)$.

To reduce the chance of making wrong decisions in these cases (especially in the early stages), we adopt a  \emph{postponing} strategy, which aims to postpone the matching of $uncertain$ pairs.
We call $[v,u]$ a \emph{strong pair}\footnote{if a pair is not strong, then it is uncertain}, if:
(1) $\mathtt{Score}(v,u)> \gamma$ where $\gamma$ is a predefined score threshold;
(2) $[v,u]$ has no $\beta$-close adversary candidate pairs, where $\beta$-close adversary is defined as follows.

\begin{definition}
	For any score function $\mathtt{Score}(,)$ and some $\beta>0$, we say a candidate pair $[v',u']$ is a $\beta$-close adversary pair of another candidate pair $[v, u]$, if $(1+\beta)\cdot \mathtt{Score}(v',u')\ge \mathtt{Score}(v,u)$ and $[v',u']$ is a adversary pair of $[v,u]$.
\end{definition}
Then we say a pair $[v,u]$ has no $\beta$-close adversary (candidate) pairs,
if $\mathtt{Score}(v,u)>(1+\beta)\cdot \mathtt{Score}(v',u')$ for all adversary pairs $[v',u']$ of $[v,u]$ which are also in the candidate set $C$.


%Let $C$ be the candidate set.
%The details of checking strong candidate pairs is shown in Procedure 1. %~\ref{proc:CSC}.

%The reasons behind that are obvious:
%(1) since the candidate pairs are generated gradually, an incorrect pair in the candidate set may have lower score than its corresponding true matches, which have not been added to candidate set;
%(2) the identification of an uncertain pair will be assisted by the matching of its neighboring pairs.
  %and $[i,j]$ is wrongly matched.


In each iteration, \emph{the algorithm only matches strong pairs in the candidate set.} Note that there will be no tie. If $\gamma$ and $\beta$ are set to be large, using this strategy, we may avoid wrongly matching the pair $[v,u']$ above.
%if either $\mathtt{Score}(v,u')\le \gamma$ (case 1,2) or $\mathtt{Score}(v,u')\le \beta\cdot\mathtt{Score}(v,u)$ (case 2).
On the other hand, after PPRGM adds more pairs to $M$ along with candidate set expansion, the matching priorities of $[v,u]$ and $[v,u']$ might be reversed and the correct match would be identified.

We employ strict matching criteria by assigning $\beta$ and $\gamma$ with relatively large values in the beginning (Empirically, we set $\beta=1$ and $\gamma=|S|/2$) to only match the most ``certain" pairs. We will relax the criteria by decreasing $\beta$ and $\gamma$ ($\beta=\beta/2$, $\gamma=(\gamma+1)/2$), when there are currently no vertex pair in $C$ satisfying the matching criteria.
%until $\gamma<1+\epsilon_1$ and $\beta<\epsilon_2$, where $\epsilon_1$ and $\epsilon_2$ are small positive constants.

The effectiveness of the postponing strategy will be analysed at the end of this Section.





%$\SP$ the choice of $\SP$ corresponds to different biases on either the region information ($\pi_1(s, v)$) or the local structural information ($LS(v)$).
%With a very large value of $\SP$, assume $[s,s']\in S$,
%whether $\pi(s,v)$ and $\pi(s',u)$ are close to each other greatly depends on the hitting probability of the random walk,
%i.e., the vertices near to the source vertex tend to have large PPR values; and the algorithm conducts much more forward-push iterations on these vertices with high PPR values.
%But in this case, the algorithm is sensitive to the unaligned structures in two network graphs.
%While the low value of $\SP$ shows a bias on the vertices' local structure information.
%Thus we empirically use $\SP=0.3$ to balance the two kinds of biases and make labelling be robust to the cross-network unaligned structures.




%The influence of vertices far away can have large variance. Simply consider the neighbors within a local range. FOE, HOE.
%Candidate generation. (Assume only the neighboring pairs of matched pair is added.) XX  not mention early-stop. Then may lead to early-stop when the matching scores of these pairs happen to be close.
%Or miss the true candidate pair because the edges set are not identical across two graphs.
%Thus, in some cases, consider more than neighboring pairs as the candidate pairs. Leads to HOE.



%
%
%%\ForEach {neighboring pair $[v',u']$ of $[v,u]$}{
%%              \If {Both $v'$ and $u'$ are not matched}{
%%    			 Insert $[v',u']$ into $C$.
%%    		  }
%%            }
%
%
%\begin{procedure}[!tb]
%\caption{2: Neighbor-Expansion($i, j$)}\label{proc:NE}
%	\ForEach {neighboring pair $[i_p,j_q]$ of pair $[i,j]$}{
%    	\If {$i_p$ or $j_q$ is matched or $[i_p, j_q]\in C$}{
%            continue;
%        }
%
%    	$\mathtt{Score}(i_p, j_q)\leftarrow \mathtt{PPRScore}(R^1(i_p), R^2(j_q))$;\\
%    	insert $[i_p, j_q]$ into set $C$;\\
%        \If {$[i_p, j_q]$ is a strong candidate pair w.r.t. $\beta$}{
%    		insert $[i_p, j_q]$ into $Q$;
%        }
%    }
%\end{procedure}

%
%\noindent
%\textbf{Algorithm.} The PPRGM algorithm is presented in Algorithm~\ref{alg:PPRGM}.
%Given two graphs $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$ to be matched and a seed set $S$. %with correct matches.
%The algorithm initializes a set $C$ for storing candidate pairs and a set $Q$ for storing strong candidate pairs. The parameter $\beta$ in the definition of strong candidate is initialized to $2$.
%Firstly, the algorithm conducts a pair of personalized PageRank computation for each seed pair, and labels the vertices on each graph with a PPR vector (line 2-5).
%Then each seed pair is inserted into candidate set $Q$ (line 6).
%In the process of matching, the algorithm starts a while-loop, which repeats as long as the candidate set is not empty and the factor $\beta$ is greater than a threshold.
%In each round, it checks each candidate pair and inserts it into $Q$ if it is a strong candidate pair w.r.t. $\beta$ (line 8-10).
%In the nested while-loop, whenever the set $Q$ is not empty, the algorithm always fetches the pair $[i,j]$ with the highest score (the score is greater than $\gamma$ because $[i,j]$ is a strong candidate pair) as a match, removes %the pairs that will not be matched ($[i,j']$ or $[i',j]$)
%all adversary pairs of $[i,j]$ from $C$, and calls the procedure \emph{Neighbor-Expansion} (line 11-19). The \emph{Neighbor-Expansion} (see Procedure 2) inserts the neighboring pairs of $[i,j]$ into $C$ along with their scores, and inserts the strong candidate pairs among them into $Q$.
%When there are no available elements in $Q$, the algorithm relaxes the requirement for strong candidate pairs by decreasing the $\beta$ (line 20), and repeats the outer-loop.
%Finally, the algorithm terminates when the candidate set is empty or when $\beta$ is below a threshold.
%
%\vspace{0.1cm}
%\noindent
%\textbf{Limits of basic PPRGM}


%\subsection{Approximate PPR on random graph.}\label{42analysis}
%
%\vspace{0.1cm}
%\noindent
%\textbf{Approximate PPR on random graph.}




\subsection{Heavy Hitters and Candidate Set Expansion}\label{42expansion}
Recall that, in PPRGM, each time a pair $[v,u]$ is inserted to $M$ (i.e., matched), its neighborhood will be added to the candidate set. Computing the score function of a new candidate requires computing $|M|$ PPR values, which is too high when $M$ becomes large.

On the contrary, when a new pair $[v, u]$ is added to $M$, we conduct a single source PPR computation for $v$ and $u$ respectively computing the PPR values for all nodes, which will be stored in the memory. However this still takes too much time and space.

Our solution is to only compute and store the ``heavy hitters" of all PPR values, i.e., PPRs that are relatively large. Computing the heavy hitters can be much faster than a full single-source PPR computation~\cite{wang2018efficient}. In particular, when a pair $[v, u]$ is added to $M$, we compute and store the PPR heavy hitters of $v$ and $u$, and regard all non-heavy PPRs as $0$. This approximate approach is time and space efficient, and produces high-quality matchings as shown in our experimental studies.



\begin{algorithm}[!tb]
\caption{Forward-Push method}\label{alg:FP}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input {$G(V, E)$, source vertex $s$, stopping probability $\SP$, residue threshold $r_{max}$}
    %\Output {$\pi^o(s, v)$ for all vertices $v\in V$}
    \Output {$FP(s)$ containing all positive $\pi^o(s, v)$ for $v\in V$}

    set $r(s, s)=1$, and $r(s,v)=0$ for all vertices $v\ne s$;

    set $\pi^o(s, v)=0$ for all $v\in V$.

    \While{$\exists v\in V$ such that $r(s,v)/|N(v)| > r_{max}$}{
        $\pi^o(s,v) = \pi^o(s,v)+\SP\cdot r(s,v)$;

        \ForEach {$u\in N(v)$}{
            $r(s, u) = r(s,u) + \PP\cdot \frac{r(s,v)}{|N(v)|};$
        }

        $r(s,v)=0;$
    }
    \Return {$FP(s)=\{\pi^o(s,v)|\pi^o(s,v)>0, v\in V\}$}
\end{algorithm}

\vspace{0.1cm}
\noindent
\textbf{Forward-Push.}
Although more efficient algorithms exist for computing PPR heavy hitters~\cite{wang2018efficient}, we use the classic Forward-Push algorithm of~\cite{andersen2007local}. This is because Forward-Push is a local algorithm, which is simple, efficient and deterministic. Moreover, the accuracy of Forward-Push is controlled by a residue threshold $r_{max}$, which is suitable for our purpose. Next we give an brief overview of the Forward-Push algorithm.
%Motivated by the first observation above, we propose to quantify the connection between a matched vertex $s$ and an unmatched vertex $v$ only if they are within a certain range in the graph, more specifically, if $v$ can be reached by a truncated random walk starting from $s$ (with positive probability). In general, we will truncate a decaying random walk starting from $s$ when its current probability is small (compared to a threshold) s.t. the truncation will not greatly affect the probabilities that the random walk terminates at any $v\in V$ (i.e., the PPR value of $v$). This is exactly the core idea of Forward-Push~\cite{andersen2007local}.  % proposed in~\cite{andersen2007local}. %, works in Algorithm~\ref{alg:FP}.

The pseudo code is presented in Algorithm~\ref{alg:FP}.
%Then we will introduce the Forward-Push method (see Algorithm~\ref{alg:FP}) in details, as it will be helpful to understand our expansion strategies.
%The algorithm takes graph $G$, source vertex $s$, stopping probability $\SP$, and a residue threshold $r_{max}$ as the input, and outputs the $\pi^o(s,i)$ for each vertex $v$.
It starts a PPR approximation on source vertex $s$.
Given graph $G(V,E)$, the source node $s$, the stopping probability $\alpha$, and a residue threshold $r_{max}$. The Forward-Push algorithm defines two variables on each vertex in graph all the time: (1) the reserve $\pi^o(s,v)$ represents the current estimation of the probability that a random walk terminates at vertex $v$ (i.e. the PPR value), which is always an underestimation of $\pi(s,v)$; (2) the residue $r(s,v)$ represents the probability that the random walk is currently at vertex $v$.
%which may terminate at $v$ or move to a neighbor at the next step.
Note that $\sum_{v\in V}{\pi^o(s,v)}+\sum_{v\in V}{r(s,v)}=1$ holds at all times (the intuitive explanation is that the random walk either has terminated at some vertex or is currently at some vertex).
Initially $r(s,s)$ is set to $1$ while $\pi^o(s,v)=0$, $\forall v\in V$, and the algorithm iteratively increases $\sum_{v\in V}{\pi^o(s,v)}$ to have better approximations to the PPR values.
In each iteration, the algorithm finds a vertex $v$ with $r(s,v)/|N(v)|>r_{\max}$\footnote{When there are multiple vertices satisfying the condition $r(s,v)/|N(v)|>r_{\max}$, the algorithm always picks the vertex $v$ with \emph{maximum} $r(s,v)/|N(i)|$, thus the number of iterations is greatly reduced as each iteration makes the most progress.} (line 3), then distributes the value of $r(s,v)$ to $v$'s neighbors: (1) it increases the reserve $\pi^o(s,v)$ by $\SP \cdot r(s,v)$ (line 4); (2) it adds $\PP \cdot \frac{r(s,v)}{|N(v)|}$ to each residue $r(s,u)$ for each $u\in N(v)$ (line 5-7); (3) $r(s,v)$ is set to $0$.
%When there are multiple vertices satisfying the condition in line 3, we always pick the vertex $v$ with \emph{maximum} $r(s,v)/|N(i)|$ in our implementation, thus the number of iterations is greatly reduced as each iteration makes the most progress.
%The Forward-Push terminates if there is no vertex $v$ s.t. $r(s,v)/|N(v)|>r_{max}$,
The Forward-Push algorithm terminates when $r(s,v)/|N(v)|\le r_{\max}$ for all $v\in V$ simultaneously,
i.e., the algorithm does not care the effect of all remaining probabilities $r(s,v)$, $\forall v\in V$; in other words, the random walk from $s$ is then \emph{truncated}.

%Since the approximate PPR values are always underestimates, the smaller the total residue $\sum_{v\in V}{r(s,v)}$ is, the better the approximations are, while the total residue at the end is controlled by the residue threshold $r_{\max}$.

%
%Recall that the Forward-Push algorithm also truncates the random walk from $s$, given a residue threshold $r_{\max}$, with the following strategy:
%(1) The Forward-Push conducts local-push (distribute the value of $r(s,v)$ to $v$'s neighbors) on vertex $v\in V$ if $r(s,v)/|N(v)|>r_{\max}$, i.e., if the probability of a random walk stopping by $v$ is still large and will make an impact;
%(2) The Forward-Push terminates when $r(s,v)/|N(v)|\le r_{\max}$ for all $v\in V$ simultaneously, i.e., the algorithm does not care the effect of all remaining probabilities $r(s,v)$ for $v\in V$; in other words, the random walk from $s$ is then \emph{truncated}.



\subsection{A Robust Matching Score Function}
The approximate PPR values from Forward-Push are used in measuring the matching score of a pair.
We also introduce a parameter $\sigma$ to~\eqref{ep_score1} to amend its deficiency in dealing with the approximate PPR values. Formally, we define the matching score of $[v,u]$ w.r.t. a seed pair (or a matched pair) $[s_k, s'_k]$ by
\begin{equation}\label{ep_score3}
\mathtt{Score_k}(v,u) = \frac{\min{(\pi^o(s_k, v),\pi^o(s'_k, u))}}{\max{(\pi^o(s_k, v),\pi^o(s'_k, u))}+\sigma}.
\end{equation}
And the matching score of $[v,u]$ with respect to a set of matched pairs is still defined by the summed score over all matched pairs.

We use the additional $\sigma$ in~\eqref{ep_score3} mainly because we don't want to rely too much on small PPR values:
%The parameter $\sigma$ is used for the following purposes:
(1) the vertices with small PPR values are often far away from the corresponding seed, and thus two similar but small PPR values may not be a good evidence for matching;
%and is likely to suffer from the unmatched structures assuming the cross-graph unaligned structures are uniformly distributed, thus it is not trusty;
(2) a small PPR value is likely to have large relative error due to either limited numerical precision or computational errors from the PPR computation (e.g., in Forward-Push method, the computational error is relevant to $r_{max}$),
which makes the score unstable.
Therefore, we put an additional term $\sigma$ in the denominator to reduce the impact from small PPR values and make the score function more stable against numerical errors.

We empirically set $\sigma$ to be $10$ times the residue threshold $r_{max}$ used in Forward-Push.



%xx why unbiased push, rather than together push.%

% .. why different r_max for seed pairs and matched pairs or just r_max. definite not good for FOE.
% More motivation. And why treat initial seed (deeper with smaller $r_{max}$) and later matched pairs differently (shallow with larger $r'_{max}$)
% XX the former framework is, initial seed PPR only. then improved to use all matched pairs.

%When there are multiple vertices satisfying the condition in line 3, we always pick the vertex $v$ with \emph{maximum} $r(s,v)/|N(i)|$ in our implementation, thus the number of iterations is greatly reduced as each iteration makes the most progress.

%The Forward-Push keeps all $\pi^o(s,i)$ as the approximations of the PPR values, while abandons all $r(s,i)$, the uncertainty part of the random walk.


%The following part is still on revision.


\begin{procedure}[!tb]
\caption{3: High-Order-Expansion($s, s', C$)}\label{proc:HOE}
    $FP(s)$  $\leftarrow$  Forward-Push$(G_1, s, \SP, r'_{max})$;\\
    $FP(s')$ $\leftarrow$  Forward-Push$(G_2, s', \SP, r'_{max})$;

	\ForEach {pair $[v,u]$ s.t. $\pi^o(s,v)\in FP(s)$ and $\pi^o(s',u)\in FP(s')$}{
    	\If {either $v$ or $u$ is matched}{
            Continue;
        }
        \If {not exist $\mathtt{Score}(v, u)$}{
            $\mathtt{Score}(v,u)$ $\leftarrow$ $\sum_{k=1}^{|S|} \mathtt{Score_k}(v,u)$;
        }
        %Compute $\mathtt{Score}_k(v, u)$ based on $\pi^o(s_k,v)$ and $\pi^o(s'_k,u)$ w.r.t. seed pair $[s_k,s_k']$;\\
        %$\mathtt{Score}(v,u)$ $\leftarrow$ $\frac{\min{(\pi(s, v),\pi(s', u))}}{\max{(\pi(s, v),\pi(s', u))}+\sigma}$;\\
        $\mathtt{Score}(v, u)$ $\leftarrow$ $\mathtt{Score}(v,u)+\frac{\min{(\pi^o(s, v),\pi^o(s', u))}}{\max{(\pi^o(s, v),\pi^o(s', u))}+\sigma}$;

        \If {$[v,u]\not\in C$}{
            Insert $[v,u]$ into set $C$;\\
        }
    }
\end{procedure}


\begin{procedure}[!tb]
\caption{4: Neighbor-Expansion($s, s', C$)}\label{proc:NE}
	\ForEach {pair $[v,u]\in N(s,s')$}{
    	\If {either $v$ or $u$ is matched}{
            continue;
        }
        \If {not exist $\mathtt{Score}(v, u)$}{
            $\mathtt{Score}(v,u)$ $\leftarrow$ $\sum_{k=1}^{|S|} \mathtt{Score_k}(v,u)$;
        }
        $\pi^o(s, v)\leftarrow\frac{\SP\PP}{|N(s)|}$; $\pi^o(s', u)\leftarrow\frac{\SP\PP}{|N(s')|}$;\\
        $\mathtt{Score}(v, u)$ $\leftarrow$ $\mathtt{Score}(v,u)+\frac{\min{(\pi^o(s, v),\pi^o(s', u))}}{\max{(\pi^o(s, v),\pi^o(s', u))}+\sigma}$;\\
        \If {$[v,u]\not\in C$}{
            Insert $[v,u]$ into set $C$;\\
        }    }
\end{procedure}

\subsection{Expansion Strategies}
%Moreover, rather than simply adding set of pairs $N(s,s')$ of each matched pair $[s,s']$ to candidate set $C$,
%we also propose to consider a pair $[v,u]$ as a candidate pair
%if $v$ and $u$ can be reached by truncated random walks starting from $s$ and $s'$ respectively for any seed pair $[s,s']\in M$, such that the first kind of bad case is likely be to avoided.
%Formally, denote $FP(s)$ the
%set of positive values $\pi^o(s,v)$ obtained from a Forward-Push process from $s$, then we propose to add each $[v,u]$ s.t. $\pi^o(s,v)\in FP(s)$ and $\pi^o(s',u)\in FP(s')$ to candidate set $C$.
Consequently, we propose new procedures that efficiently make use of each matched pair $[s,s']$ to increase the credibilities (matching scores) of the pairs to be matched.

In our new strategies, firstly, we propose to treat the initial seed pairs (in $S$) and the pairs matched by the algorithm (in $M-S$) differently by setting for them different range of impact (with Forward-Push).
This is because the seed pairs intuitively have higher credibilities than the pairs matched later, thus we should allow the seed vertices to provide evidences for more unmatched vertices (with relative longer random walk paths). %even a relative long random walk from a seed vertex can be reliable.
More specifically, at the beginning of algorithm, we conduct Forward-Push on each seed vertex $s$ ($s'$) with a relative small $r_{max}$,
after which each vertex $v\in V_1$ ($u\in V_2$) gets a number of approximate PPR values, i.e.,  $\pi^o(s_k, v)\ge 0$ for $1\le k \le |S|$. %, with respect to $S$. %, i.e., $\pi^o(s_k, v)\ge 0$ for $1\le k \le |S|$.
Thus, in PPRGM, the basic matching score %$\mathtt{Score}_S(v,u)$
of a pair
$[v,u]$ is %defined by
$\sum_{k=1}^{|S|} \mathtt{Score_k}(v,u)$ w.r.t. all initial seeds; the algorithm only computes the basic matching score of $[v,u]$ when $[v,u]$ is added to $C$ as a candidate pair.
Then, when new pairs are matched during the algorithm, we use different strategies to allow these matches to infect unmatched pairs;
two expansion strategies will be presented in replace of the \emph{Neighbor-Expansion} function in Algorithm~\ref{alg:PPRGM} (line 9).
%We then propose two strategies of percolation with different percolation range, namely the First-Order-Expansion (FOE) and Higher-Order-Expansion (HOE).%, as shown in Procedure 3 and Procedure 4 respectively.

\vspace{0.1cm}
\noindent
\textbf{The High-Order-Expansion.}
The High-Order-Expansion method (HOE, see Procedure 3) starts two Forward-Push procedures on $s$ and $s'$ respectively, for each matched pair of $[s,s']\in M'$,
using the same $\SP$ and the same residue threshold $r'_{max}$ (line 1-2).
Note that $r'_{max}$ is set greater than $r_{max}$ that is used by Forward-Push on seed vertices.
The Forward-Push procedures return $FP(s)$ and $FP(s')$ which contain that vertices infected by $s$ and $s'$ respectively, as well as their approximate PPR values.
Then HOE considers each vertex pair $[v,u]$ s.t. $\pi^o(s,v)\in FP(s)$ and $\pi^o(s',u)\in FP(s')$ (i.e., $[v,u]$ is infected by $[s,s']$).
If either $v$ or $u$ is already matched, the algorithm does nothing and continues to consider the next infected pair (line 4-6).
If $\mathtt{Score}_S(v,u)$, the basic matching score of $[v,u]$ w.r.t. the set $S$ of initial seed pairs, has not been computed before,
then HOE assigns $\mathtt{Score}(v,u)$ with $\sum_{k=1}^{|S|} \mathtt{Score_k}(v,u)$ (line 7-9).
Next, the HOE method computes an increment $\frac{\min{(\pi^o(s, v),\pi^o(s', u))}}{\max{(\pi^o(s, v),\pi^o(s', u))}+\sigma}$ based on Equation~\eqref{ep_score3}, as the new evidence to the matching of $[v,u]$ contributed by $[s,s']$, and adds it to $\mathtt{Score}(v,u)$ (line 10).
Finally, the HOE method inserts pair $[v,u]$ into to the candidate set $C$ if $[v,u]\not\in C$ (line 11-13).

\vspace{0.1cm}
\noindent
\textbf{The Neighbor-Expansion.} We also present a more efficient variation, namely the Neighbor-Expansion (NE, see Procedure 4).
The NE method is more reserved
in both impact expansion %(from a matched pair)
and candidate selection.
Given a pair of matched vertices $[s,s']$, NE conducts Forward-Push on $s$ and $s'$ respectively for only $1$ step, i.e.,
for each $v\in N(s)$ and $u\in N(s')$,
it assigns $\pi^o(s,v)$ with $\frac{\SP \PP}{|N(s)|}$ and $\pi^o(s',u)$ with
$\frac{\SP \PP}{|N(s')|}$ respectively (line 8). Then the increment on matching score $\mathtt{Score}(v,u)$ is computed based on $\pi^o(s,v)$ and $\pi^o(s',u)$ using the score function in Equation~\eqref{ep_score3} (line 9). NE also ensures that the pair $[v, u]$ is included by the candidate set $C$ (line 10-12).

%The main difference between the First-Order-Expansion and the percolation in traditional PGM algorithms, given a matched pair $[s,s']$ and a pair $[v,u]\in N(s,s')$, is:
%the traditional percolation always adds $1$ mark to $[v, u]$; in the FOE, the increment added to $\mathtt{Score}(v, u)$ is

%An interesting observation on the FOE strategy is:
%The FOE has the following pro
We simply use the expansion in NE to illustrate one advantage of exploiting the random walk in quantifying the connections between vertices.
Given a matched pair $[s,s']$ and a pair $[v,u]\in N(s,s')$, in FOE, the increment added to $\mathtt{Score}(v, u)$ by $[s,s']$ is
$\frac{\min{(\pi^o(s, v),\pi^o(s', u))}}{\max{(\pi^o(s, v),\pi^o(s', u))}+\sigma}=
\min\{\frac{|N(s)|}{|N(s')|+\sigma'},\frac{|N(s')|}{|N(s)|+\sigma'}\}$,
where $\sigma' = \frac{\sigma}{\SP\PP}$.
%The FOE defines the increment in this way such that (1) the evaluation of local labels and global labels can be aligned by the same formulation; (2)
The FOE method has a vertex pair $[s,s']$ with smaller relative degree difference contribute higher increment to the matching scores of its neighboring pairs. In other words, a matched pair with smaller degree difference is considered as a stronger evidence for later matching, which is in the same spirit as the matching preference used in EWS~\cite{kazemi2015growing}.
%(not same)
%and when $|N(i)|=|N(j)|$, $\mathtt{inc}_{i,j}(i_p,j_q)$ is maximized ($\approx 1$).


\vspace{0.1cm}
\noindent
\textbf{Comparison of HOE and NE.}
When $r'_{max}$ is large enough, HOE is simply equal to FOE, i.e., a matched pair percolates to its neighboring pairs only. %We simply assume the $r'_{max}$ in HOE is small in the following comparison thus each matched pair affects more than its neighboring pairs .

The FOE method is more efficient than HOE, because it infects less number of vertices in each expansion and includes less candidate pairs overall;
HOE may have higher recall (more correct matches) than FOE,  because more candidate pairs are considered by HOE.
We also compare two algorithms in another perspective.
The final matching score of a candidate pair is the combination of the (global) scores w.r.t. initial seeds and the (local) scores w.r.t. pairs matched by algorithm in the former rounds.
In HOE, a matched pair can infect many unmatched pairs, thus each candidate pair is likely to receive many local credits, the overall effect of which may overwhelm the effect of initial seeds.
While in FOE, the effect of initial seed matches may play a more important role than the local early matches.
Detailed comparison between HOE and FOE, as well as the effect of various $r'_{max}$ will be presented in the experiment section.




%
%the score of any pair is computed based on the PPR values w.r.t. the initial seed set only. However, it is natural to consider the early matched pairs as new evidence to match other unmatched pairs as in the PGM framework; utilizing more evidence is helpful to eliminate the bad case (2) above.
%On the other hand, the above PPRGM only adds the neighboring pairs of already matched pairs to the candidate set. To avoid the bad case (1) mentioned above, we will expand more aggressively by including a local neighborhood of a matched pair.

%\noindent
%\textbf{Motivation.}
%Though the graph labelling based on Personalized PageRank vector is effective in graph matching, it has limitations. The PPRGM framework tends to match pairs with the high $\mathtt{PPRScore}$ first. The effectiveness of evaluating the pairs based on PPR vectors decays while the algorithm is dealing with the pairs with low $\mathtt{PPRScore}$.
%Note that a correct match $[i,j]$ can have a low $\mathtt{PPRScore}$  as a result of the structural difference across two graphs. In this case, pair $[i,j]$ is more likely to have adversary pairs with higher $\mathtt{PPRScore}$, thus may not be correctly matched.
%To amend this, we turn to the pairs that have been matched before $[i,j]$, which have higher credibility ($\mathtt{PPRScore}$) and may suffer less from the unaligned structure. These matched pairs can provide guidance in eliminating the effect of structural difference that lies on the paths from the seeds to them.

%A straightforward idea is to align two PPR vectors of each matched pair by editing two graphs (deleting the edges and vertices). If  two graphs are isomorphic after being edited, then the corresponding vertices have the identical PPR vectors. For example, assume $N(i_1)=\{i_2,i_3\}$ for $i_{1,2,3}\in V_1$ and $N(j_1)=\{j_2\}$ for $j_{1,2}\in V_2$, once $[i_1,j_1]$ and $[i_2, j_2]$ are matched, we remove $(j_1,j_3)\in E_2$ to align the structures in two graphs, and update the PPR vectors of vertices in $V_2$ with an efficient dynamic PPR approximation method~\cite{zhang2016approximate}.
%However, the graph editing method above is not robust to the wrong matches, because it trusts each matched pair and edits graphs accordingly, which fully determines the evaluation of unmatched pairs.
%Besides, a large number of graph edits and dynamic PPR approximation incurred lead to a high time cost.

%Instead of adopting the graph edit method, we use a percolation and local labelling method to exploit the matched pairs in this paper. Note that the influence of early matches on the unmatched pairs can be regarded as a bias, w.r.t. the effect of global labelling applied by the seeds. The proposed method achieves a balance between both kinds of effect (from the  seeds and from the early matches), and it is more efficient than the graph edit method because it has each match affect the pairs within a local range only.

%We use a percolation and local labelling method to exploit the matched pairs in this paper. Note that the influence of early matches on the unmatched pairs can be regarded as a bias, w.r.t. the effect of global labelling applied by the seeds. The proposed method achieves a balance between both kinds of effect (from the  seeds and from the early matches). %, and it is more efficient than the graph edit method because it has each match affect the pairs within a local range only.



%\begin{algorithm}[!tb]
%\caption{Not decide if keep. add beta, gamma, Forward-Push}\label{alg:ESPPRGM}
%    \SetKwInOut{Input}{Input}
%    \SetKwInOut{Output}{Output}
%    \Input {$G_1(V_1, E_1), G_2(V_2, E_2)$, seed set $S$ of correct matches, stopping probability $\SP$, residue threshold $r_{max}$}
%    \Output {The set of matched pairs $M$}
%
%%\Procedure{PPRGM}{$ $}
%    %initialize set of matched pairs $M=\Emptyset$, set of matched vertices $VM_1=\Emptyset$ and $VM_2=\Emptyset$,
%    %, ratio for checking strong candidate $\beta=2$, and score threshold $\gamma$;
%    initialize candidate pair set $C\leftarrow\Emptyset$, strong candidate pair set $Q\leftarrow\Emptyset$, expanding seed set $A\leftarrow\Emptyset$, and $\beta\leftarrow2$;
%
%    \ForEach {seed pair $[s^1_k, s^2_k]$}{
%       $R^1$ $\leftarrow$ Forward-Push$(G_1, s^1_k, \SP, r_{max})$;\\
%       $R^2$ $\leftarrow$ Forward-Push$(G_2, s^2_k, \SP, r_{max})$;
%    }
%
%    insert each seed pair $[s^1_k, s^2_k]$ into $Q$;
%
%    \While{$C\ne \Emptyset$ and $\beta>1+\epsilon$}{
%        \ForEach { strong candidate pair $[i,j]\in C$  w.r.t. $\beta$}{
%    		insert $[i,j]$ into $Q$;
%    	}
%    	\While{$Q \ne \Emptyset$}{
%    		find $[i,j]\in Q$ with highest $\mathtt{Score}(i,j)$;\\
%    		%\If {$\mathtt{Score}(i,j)<\gamma$}{
%    		%	break;
%    		%}
%    		mark $i, j$ as matched, insert $[i,j]$ into $M$;\\
%    		remove all $[i,j']$ and $[i',j]$ w.r.t. $i$ and $j$ from $C$;\\
%            insert $[i,j]$ into $A$;
%    	}
%        \eIf {$A\ne\Emptyset$}{
%            \ForEach {pair $[i,j]\in A$}{
%        		\textbf{First-Order-Expansion($i, j$)};
%        	}
%            $A\leftarrow\Emptyset$;
%        }
%        {
%        	update $\beta \leftarrow (\beta+1)/2$;\\
%        }
%    }
%    \Return {M}
%\end{algorithm}


%\noindent
%\textbf{Extended PPRGM.}
%%The PPRGM framework with percolation is introduced then.
%In the extended PPRGM, each pair $[i,j]$ that is added to the matching set is considered as a new and unused seed pair. We may start a Forward-Push from $[i,j]$ to compute the PPR values of other vertices w.r.t. the new seed, then add a new label to the PPR labeling of each vertex. However, to save the computation time, the Forward-Push from new seeds will stop much earlier. We distinguish two cases.
%%the new seeds from the initial ones by stopping .
%In the first case, we only allow the Forward-Push from new seeds to infects its neighboring pairs, which is referred to as First-Order-Expansion (FOE); in the second case, we allow the Forward-Push to infect pairs within a small local range by setting a relatively large residue threshold, which is referred to as Higher-Order-Expansion (HOE). %determined by the $r_{max}$ in Forward-Push process.
%%For each infected pair $[i_p, j_q]$, the PPR values of vertex $i_p$ and $j_q$ from the Forward-Push method are assigned to them as the new local labels.
%In both cases, each infected pair $[i_p, j_q]$ in the Forward-Push process is then included to the candidate set, and two local labels computed in FOE or HOE are assigned to vertex $i_p$ and $j_q$ respectively.
%Meanwhile, an increment $inc_{i,j}(i_p,j_q)$ computed from the new labels (according to the score function) is added to the score of $[i_p,j_q]$. %which is computed based on the newly assigned PPR values (local labels) using the Equation (\ref{pprscore1}).
%To avoid the ambiguity, we then use $\mathtt{PPRScore}$ specifically for the score measuring the global labels (w.r.t. initial seeds).
%Thus the overall score of each candidate pair $[i_p,j_q]$ is computed by
%\begin{equation}\label{totalscore}
%\mathtt{Score}(i_p,j_q) = \mathtt{PPRScore}(i_p,j_q) + \sum_{[i,j]~\textrm{infects}~[i_p,j_q]} \mathtt{inc}_{i,j}(i_p,j_q).
%\end{equation}
%
%The extended PPRGM framework is presented in Algorithm~\ref{alg:ESPPRGM}. %We will introduce its difference from the Algorithm~\ref{alg:PPRGM}.
%%Compared to the PPRGM algorithm in Algorithm~\ref{alg:PPRGM},
%A set $A$ is used to store the newly matched pairs. When a pair is matched, it is added to both $M$ and $A$. After a round of matching (line 11-16), if the set $A$ is not empty, the algorithm does FOE (or HOE) for each pair in $A$ and then empties $A$  (line 17-21).
%%i.e., there are no matches that have not percolated, then ;
%Otherwise, the algorithm relaxes the requirement for strong candidate pairs by decreasing $\beta$ as before (line 23).
%%the algorithm starts a round of percolation. Each match $[i,j]\in A$ calls a procedure of expansion (i.e., percolation and local labelling, which will be discussed in details later),
%Note that all scores considered in the Algorithm~\ref{alg:ESPPRGM} is computed with Equation (\ref{totalscore}), contributed by both the global labels and local labels.



%\noindent
%\textbf{Comparison with ExpandOnce algorithm.}
%It is worth mentioning the ExpandOnce algorithm in~\cite{kazemi2015growing} is a special case of our PPRGM framework with HOE strategy. The ExpandOnce doesn't use the global labelling method, and it has each matched pair $[i,j]$ add $\mathtt{inc}(i_p,j_q)=1$ to the score of pair $[i_p,j_q]$, if $dist(i,i_p)=dist(j,j_q)\le k$ where $k$ is a given constant. Formally, the overall score of each candidate pair defined by the ExpandOnce algorithm is
%\begin{equation}\label{EWSscore}
%\mathtt{Score}(i_p,j_q) = \sum_{[i,j]~\emph{infects}~[i_p,j_q]} 1.
%\end{equation}
%Our HOE method achieves better effectiveness than the ExpandOnce algorithm by introducing both the global labelling and the PPR-based local labelling. It is also noted that Theorem 1 in~\cite{kazemi2015growing} proves the robustness of \emph{noisy seed} method in ExpandOnce algorithm, which can be extended to prove the robustness of our local higher-order labelling strategy as well.
%Moreover, the start-of-the-art algorithm EWS~\cite{kazemi2015growing} is based on the same robustness analysis, but practically performs better than the ExpandOnce.
%The comparison between the EWS algorithm and the proposed FOE and HOE will be presented in the experiment section.

%As a result, the value of $N_m(i,j)$ suffers from the incorrect matches, as the \emph{noisy seed set} in PGM algorithms.
%The affect of incorrect matches on PGM has been analysed in~\cite{kazemi2015growing}. The \emph{noise} in $N_m(i,j)$ has a more minor influence on PPRGM compared to that in PGM:
%(i) the effect of bias is limited, while PGM relies only on the noisy neighboring matches;
%(ii) the framework of PPRGM tends to select the trustiest vertex pairs at each step, thus overall influence of incorrect matches along the process is diminished.



%\subsection{An analysis of $\Omega(\sqrt(n))$ seeds and the comparison with IsoRank}
%(1) simple proof: how postponing the adversary pairs works.

%(2) medium proof: how pprscore additionally helps distinguishing compared to EWS.

%(3) hard proof: how ppr works on random graph with edge sampling.
 %   sub: may prove the number of seeds required to label all vertices differently with PPR vectors, on two isomorphic random graphs. Though $\Omega(\log(n))$ has been proved in seeded graph matching.

%An analysis on the effectiveness of the PPRGM algorithm will be provided.
%
%We first introduce the $G(n,p;p_n,p_e)$ random graph model that has been used in~\cite{pedarsani2011privacy, kazemi2015growing}. The $G(n,p;p_n,p_e)$ random graph model generates two corrected graphs as follows: (1) a graph $G(V,E)$ is generated from Erd\"os-Renyi random graph, i.e., in a graph of $n$ vertices, each of ${n}\choose{2}$ possible edges occurs with probability $0<p<1$; (2) $V_1$ and $V_2$ are two independent sample sets of $V$, in which each vertex $v\in V$ is sampled with probability $p_n$; (3) each edge $(i,j)\in E$ s.t. $i,j\in V_1$ is included in $E_1$ with probability $p_e$, and $E_2$ is generated in the same way. We assume that the average degree $np$ is constant, satisfying that the Erd\"os-Renyi random graph has a unique giant component containing a positive fraction of the vertices
%with high probability.
%The task of graph matching is to identify the correct matches between $V_1$ and $V_2$.

%%!! we should first analyse how 1/deg works in PGM.

%%In the following part, we will show (1) the strategy of postponing the matching of pairs with close adversary pairs (referred as to the postponing strategy) helps improve the precision while not affecting the recall; (2) the vertices on random graph can be distinguished by the PPR vector with a limited number of seeds.

%% Currently we analyse the postponing strategy based on a general percolation framework.
%% It is more complicated to prove it in our framework even with order-1 setting. We should deal with differentiation of 1/degree.
%% If connected, label $\pi$ is expected $1/(npp_e)$; otherwise, label is $0$.

%\subsubsection{Effectiveness of Postponing Strategy.} \label{4analysis1}
%We propose the postponing strategy in Section~\ref{4main}: the match of a pair having close adversary pairs should be delayed.
%It will be shown that the postponing strategy greatly decreases the number of pairs that are wrongly matched.
%
%Recall that the adversary pairs of $[i,j]$ are the set of all pairs in $\{i\}\times V_2$ and $ V_1\times \{j\}$. Any wrong vertex pair $[i,j]$ always corresponds to two correct adversary pairs $[i_1,j]$ and $[i,j_1]$.
%Denote $n_c$ the number of correctly matched pairs in the seed set $S$, and $n_w$ the number of wrongly matched pairs in $S$.
%For simplicity, we consider a special case in the analysis:
%(1) the order-1 information is considered only, and each seed pair adds $1$ mark to its neighboring pair;% (as in Equation~\ref{EWSscore});
%(2) a pair can be matched if it has at least $2$ marks, and its score is greater than that of all its adversary pairs.
%% new setting
%%(1) the order-1 information is considered only; % i.e., a matched pair $[u,v]$ adds $min\{\frac{deg(u)}{deg(v)}, \frac{deg(v)}{deg(u)}\}$ to each of its neighboring pairs.
%%(2) a pair can be matched if it receives score from at least 2 neighboring pairs, and its score is greater than that of all its adversary pairs by a factor $\beta$. % relevant to maximal degree
%
%\begin{lemma}\label{lemma1}
%In the $G(n,p;p_n,p_e)$ random graph model, assume the above percolation method and matching criteria are adopted, the postponing strategy decreases the probability of a wrong pair being matched
%from $(n_c+n_w)^2 p^4p_e^4$ to $(n_c+n_w)^2 p^4 p_e^4 - n_c^2 p^4 p_e^4 (2p_e^4-p_e^8+ 2 p_n^2 p_e^4 - 2p_n^4 p_e^4)$, and decreases the probability of a correct pair being matched
%from $n_c^2 p^2 p_e^4$ to $n_c^2 p^2 p_e^4 (1-np^2)$.
%\end{lemma}
%
%The proof of Lemma~\ref{lemma1} is included in appendix. Obviously, the postponing strategy greatly decreases the number of pairs that are wrongly matched.
%Assume $p_n=1$ (say $V_{1,2}=V$) and $n_w=0$ (no wrong matches in the seed set), then the probability of a wrong pair $[i,j]$ being matched in the next iteration is $p^4p_e^4 n_c^2(1-p_e^4)^2$, which is decreased nearly by $10$ times when the edge sampling probability $p_e=0.9$, compared to a probability of $p^4 p_e^4 n_c^2$ without the postponing strategy. In two isomorphic graphs, as $p_n=1$ and $p_e=1$, then no wrong pairs can be matched if all initial seeds are correct. This will also be verified in the experiments as our algorithm achieves a precision of $1$ in matching two isomorphic graphs.
%Because $np$ is a constant greater than $1$, $\frac{1}{p^2}\gg n$, thus $n_c^2 p^2 p_e^4 (1-np^2)$ is very close to $n_c^2 p^2 p_e^4$. By replacing the matching probability (for correct pairs and wrong pairs) in Theorem 1~\cite{kazemi2015growing} with the new probabilities derived above, we can conclude that the postponing strategy increases the matching precision greatly while not affecting the overall recall by much.

% the ratio of the number of correct matches over the number of wrong matches in each iteration is $\frac{np^2s^4c^2}{n^2p^4s^4(c+w)^2}$, thus postponing strategy will not affect the overall recall.





% shortest path with decaying factor + (distance=1,2,3,... + multiple paths + 1/deg) = PPR
% but hard to say: different shortest distance -> different PPR.
% intuitively, cannot be distinguished by shortest distance vector -> cannot be distinguished by PPR vector
% 1. discard the setting of 1/deg: set decaying factor = 1/2np, the summed value still converges to c<1
% a random decaying factor w.r.t. a vector of all distances  multiple distances or multiple paths may lead to dependency.

% what if $np\to \log(n)$

%\textbf{Part3.}
%Recall that the ExpandOnce algorithm has been shown as a special case of our PPRGM framework with HOE in Section~\ref{4expand}. The outstanding matching ability of ExpandOnce algorithm as well as its robustness has been proved in Theorem 1 of~\cite{kazemi2015growing}. Here we take the PPR labelling method as an additional strategy based on ExpandOnce, and show how it additionally increases the matching precision.

%For simplicity,
%have to re-read part 1 first.

%Given random seed $s$ and vertex $i$, the PPR value of $i$ follows a distribution $\mathcal{D}$. When the random graph is constructed, i.e., each edge is sampled with probability $p$, the PPR value of $i$ follows another distribution $\mathcal{D}_i$ derived from $\mathcal{D}$ w.r.t. edge sampling. $\mathcal{D}_i$ and $\mathcal{D}_j$ have dependency as the computation shares the same set of edges. Prove $v_1$, $v_2$ from $\mathcal{D}_i$ has higher score w.r.t. the score function than that of $v_1$, and $v_3$ from $\mathcal{D}_j$.

% try to prove:
%with a certain probability, cannot be distinguished, e.g., same PPR vector. with subtle probability score(i,i')<score(j,i'), may be solved by the postponing strategy.
%with a certain probability, score(i,i')\gg score(j,i'), can be distinguished.







%add or not
%\subsection{Merge seeds}
%\textbf{Not sure if need this part.}
%Whenever a pair is inserted into the candidate set, the algorithm calls the function in equation (\ref{pprscore2}) to compute $\mathtt{PPRScore}$, with $O(|S|)$ complexity. We propose a strategy to speed up the computation by merging the seeds, more precisely, merging the PPR values of each vertex w.r.t. to the initial seed set.
%
%Intuitively, we always merge two seeds that are most relevant, i.e.,  seed $p$ and $q$ has highest PPR value w.r.t. each other, against any other pair of seeds.
%For each seed in the graph, we compute a personalized PageRank with it as the source vertex. Then we sort all vertices labelled by this PPR in a descending order of PPR value and have a PPR sequence w.r.t. this seed.
%Given any two seeds $p$ and $q$ in a graph, we obtain two sequences. XXX We find two longest consecutive sub-sequence that are highly similar, i.e., two seeds have the similar effect in labelling this subsequence.  When all vertices before this sub-sequence are matched, then two seeds should be merged.
%XXX.
%%add or not
%\subsection{Flexibility of PPRGM}
%
%\textbf{Not sure if need this part.}
%%\subsubsection{PPRGM on dynamic graph}
%In this section, we will show the flexibility of PPRGM with two cases.
%
%\subsubsection{PPRGM on real graph}
%\textbf{Not sure if need this part.}
%\textbf{have not proved in experiments.}
%
%In the literature of graph matching, the analysis always focus on a special way of constructing the aligned graphs: given an original graph $G(V,E)$, firstly the algorithm samples each vertex $i\in V$ with a probability of $pn$ and obtains $V' \subset V$, then the algorithm samples each edge $(i,j)$ s.t. $i\in V'$ and $j\in V'$ with probability of $pe$ and obtains $E'\subset E$, thus $G'(V', E')$ is a subgraph of $G$. Each graph to be matched is constructed in this way.
%However, in the real world applications, the overlap between the graphs is not always uniformly distributed. For example, in the social network, a relationship between two users who share multiple common friends is more likely to exist in aligned networks, i.e., the probability of a edge $(i,j)$ existing in the subgraph is proportional to the number of common neighbors shared by $i$ and $j$.
%
%Our PPRGM framework can deal with this skewed graph generation model with a slight modification, i.e., PPRGM adopts a biased random walk while doing labelling with the personalized PageRank. The reason behind this is that we tend to trust the vertices that share more common neighbors with the matched vertices. XXX . While none of the former works can be easily transferred to deal with this graph model.
%
%
%\subsubsection{PPRGM on weighted graph}
%\textbf{Not sure if need this part.}
%analysis for weighted graph.
%Two isomorphic graph with different edge weight.
%PPR denote the LS difference.
%EWS cannot easily extend to because integer
%graph matching

%\section{Personalized PageRank in Graph Labelling} \label{3PPR}
%
%Personalized PageRank has been extensively adopted in graph structure analysis, such as community detection~\cite{avron2015community}, graph ordering~\cite{benson2016higher, yin2017local}, and other applications~\cite{gleich2015pagerank}. The Personalized PageRank value plays different roles in various phenomena, such as denoting the local range or measuring the importance of vertices. In this paper, we exploit the power of personalized PageRank in graph labelling.
%
%Given a set of seeds $S$ on graph $G$, we conduct a personalized PageRank approximation on each seed $s_k$ (as the source) by using the Forward-Push with the same stopping probability $\SP$ and the same residue threshold $r_{max}$. The PPR value of vertex $i\in V$ w.r.t. $s_k$ is $\pi(s_k, i)$, and the PPR vector of vertex $i$ is $R(i) = \{\pi(s_1, i), \pi(s_2, i), \cdots, \pi(s_{|S|}, i) \}$. We take the PPR vector as the global label for each vertex. It can be shown the PPR vector of each vertex illustrates both its region information and local structure information in Appendix~\ref{7ppr}.

%\subsection{PPR labelling} \label{3labelling}


%\textbf{Puzzle:} The setting of Residue threshold with respect to different stopping probability is still a mystery$\cdots$ May relevant to the size of datasets, the property of dataset graph, the number of seeds, and so on. Waiting the results of experiments on data sets.
%
%Results of exp: set all $\SP=0.3$. For social network with a large number of triangles (facebook and twitter), $r_{max}=1e-6$; for others (Email and sx-mathflow) with fewer triangles, $r_{max}=1e-5$.
%Likely for graphs with more triangle, the PPR residue decays fast with respect to distance, thus use smaller $r_{max}$.
%Now we think twitter with more triangles should use larger $r_{max}$ (1e-5~1e-6) than amazon with fewer triangles (1e-7+).



\subsection{Analysis} \label{33analysis}


\vspace{0.1cm}
\noindent
\textbf{Time complexity analysis.}
% rough result.. too many expression of on average. E/V
We assume both graphs in matching contain $O(|V|)$ vertices and $O(|E|)$ edges for simplicity. A lemma is given as follows.

\begin{lemma}\label{lemma:time}
Given graphs $G_1$ and $G_2$ to be matched, each with $O(|V|)$ vertices and $O(|E|)$ edges, and a set $S$ of seed pairs, PPRGM takes
$O(\frac{|S|}{r_{max}r'^2_{max}}+\frac{|V|}{r'^2_{max}})$ complexity to match two graphs,
where $r_{max}$ and $r'_{max}$ are the residue thresholds used in Forward-Push on seed vertices and matched vertices respectively.
\end{lemma}

\begin{proof}
PPRGM mainly conducts Forward-Push and matching score computation. The two jobs will be discussed separatively.

The Forward-Push (see Algorithm~\ref{alg:FP}) uses residue threshold $r_{max}$ to determine the termination of pushing forward.
%Forward-Push method is presented in Algorithm~\ref{alg:FP}, with $r_{max}$ determining the termination of pushing forward.
~\cite{andersen2006local} proves a Forward-Push process takes $O(1/r_{max})$ time.
PPRGM uses different residue thresholds $r_{max}$ and $r'_{max}$ in Forward-Push on seed vertices and matched vertices respectively.
Thus, all Forward-Push processes take totally $O(\frac{|S|}{r_{max}}+\frac{|V|}{r'_{max}})$ time.
In particular,
if each matched vertex is only allowed to percolate its neighbors (the FOE method),
then all Forward-Push processes take $O(\frac{|S|}{r_{max}}+|E|)$ time; in this case we can regard $r'_{max}$ as $O(|V|/|E|)$.
%\footnote{ If each matched vertex is only allowed to percolate its neighbors (the FOE),
%then all Forward-Push processes take $O(\frac{|S|}{r_{max}}+|E|)$ time, i.e., we can regard $r'_{max}$ as $O(|V|/|E|)$ in this case.}. %We often in practice set $r_{max}$ s.t. $\frac{|S|}{r_{max}}=c\cdot|V|$ where $c$ is a constant.

%Next, we consider the cost of matching score computation.
The computation of matching score for a candidate pair $[v,u]$, where vertex $v$ has $m$ positive PPR values and vertex $u$ has $n$ positive PPR values, takes $O(\min(m,n))$ time.
Firstly, a single Forward-Push on $v$ with a residue threshold $r'_{max}$ assigns $O(\frac{1}{r'_{max}})$ vertices each with one positive PPR value. Therefore, the matching score computation w.r.t. the PPR values assigned by a matched pair $[v,u]$ takes $O(\frac{1}{r'^2_{max}})$ complexity.
Regarding a maximum number of $|V|$ matched pairs, the cost is $O(\frac{|V|}{r'^2_{max}})$.
Secondly, each vertex receives on average $O(\frac{|S|}{r_{max}|V|})$ positive PPR values w.r.t. all initial seeds;
denote $C$ the set of all candidate pairs that are considered by our algorithm, the matching score computation w.r.t. the PPR values assigned by the initial seeds takes
$O(\frac{|S|\cdot|C|}{r_{max}|V|})$ time.
%Thus each vertex receives on average $O(\frac{|S|}{r_{max}|V|}+\frac{1}{r'_{max}})$ positive PPR values w.r.t. all initial seeds and matched vertices.
%Denote $C$ the set of all candidate pairs that are considered by our algorithm. %Then a vertex is measured with on average $O(\frac{|C|}{|V|})$ vertices from the other graph.
%Then, the matching score computation of all candidate pairs totally takes $O(\frac{|S|\cdot |C|}{r_{max}|V|}+\frac{|C|}{r'_{max}})$ time.
We also claim $|C|$ is bounded by $O(\frac{|V|}{r'^2_{max}})$.
Because the number of matched pairs is bounded by $O(|V|)$ and a Forward-Push procedure on a matched pair $[v,u]$ leads to $O(\frac{1}{r'^2_{max}})$ candidate pairs
(the Cartesian product of two sets of vertices with PPR values in $FP(v)$ and $FP(u)$ respectively)
\footnote{The sets of candidate pairs expanded from different matched pairs are actually greatly overlapped, thus in practice the total number of candidate pairs is much smaller than $O(\frac{|V|}{r'^2_{max}})$. The measurement of the number of candidate pairs will be presented in the experiment section.}.
In conclusion, the overall time complexity of our algorithm is $O(\frac{|S|}{r_{max}} + \frac{|V|}{r'_{max}} + \frac{|V|}{r'^2_{max}} + \frac{|S|}{r_{max}r'^2_{max}})=O(\frac{|V|}{r'^2_{max}}+ \frac{|S|}{r_{max}r'^2_{max}})$ (dominated by the cost of matching score computation).
\end{proof}

In practice, we often set $r_{max}$ s.t. $\frac{|S|}{r_{max}}=c\cdot|V|$ where $c$ is a constant, which leads to an overall time complexity of $O(\frac{|V|}{r'^2_{max}}$).
As discussed above, in the PPRGM framework, an upper bound for $r'_{max}$ should be $O(|V|/|E|)$, corresponds to the FOE strategy; the overall time complexity increases as smaller $r¡¯_{max}$ is used, which corresponds to larger range of expansion and more candidate pairs.

We also provide the time complexity analysis of EWS algorithm in Appendix \ref{7EWS}.

\begin{figure}[!tb]
\begin{centering}
\includegraphics [width=3.0in]{fig/fig3.eps}
\vspace*{-2mm}
\caption{$G(n,p;p_n,p_e)$ Random Graph Model. }
\label{randomgraph}
\vspace*{-4mm}
\end{centering}
\end{figure}

\vspace{0.1cm}
\noindent
\textbf{Effect of postponing strategy.}
%Before the analyzing effectiveness of the postponing strategy,
We first introduce the $G(n,p;p_n,p_e)$ random graph model that has been used in~\cite{pedarsani2011privacy, kazemi2015growing}.
The $G(n,p;p_n,p_e)$ random graph model (see Figure~\ref{randomgraph}) generates two corrected graphs as follows:
(1) A graph $G(V,E)$ is generated from Erd\"os-Renyi random graph, i.e., in a graph of $n$ vertices, each of ${n}\choose{2}$ possible edges occurs with probability $0<p<1$;
(2) $V_1$ and $V_2$ are two independent sample sets of $V$, in which each vertex $v\in V$ is sampled with probability $p_n$;
(3) Each edge $(v,u)\in E$ s.t. $v,u\in V_1$ is included in $E_1$ with probability $p_e$, and $E_2$ is generated in the same way.
We assume that the average degree $np$ is constant, %satisfying that the Erd\"os-Renyi random graph
thus $G(V,E)$ has a unique giant component containing a positive fraction of the vertices with high probability. The task of graph matching is to identify the correct matches between $V_1$ and $V_2$.
%An example of $G(n,p;p_n,p_e)$ random graph model is shown in Figure \ref{randomgraph}:
%the graph $G(V,E)$ is generated with $n=6$ and $p=0.7$; two graphs $G(V_1, E_1)$ and $G(V_2, E_2)$ are sampled based on $G(V,E)$ with $p_n=0.9$ and $p_e=0.8$.

To prove the effectiveness of postponing strategy, we consider a special case here:
(1) the order-1 (neighboring) information is considered only, and each seed match adds $1$ mark to its neighboring pair, i.e., the matching score of pair $[v,u]$ is the number of matched pairs in $N(v,u)$;
(2) we fix $\gamma=1+\epsilon_1$ and $\beta=\epsilon_2$ where $\epsilon_1$ and $\epsilon_2$ are small positive constants. That is to say, a pair $[v,u]$ can be matched if $\mathtt{Score}(v,u)\ge 2$,
and $\mathtt{Score}(v,u)\ge\mathtt{Score}(v',u')+1$ for any $[v',u']\in \{(\{v\}\times V_2)\cup (V_1\times \{u\})-[v,u]\}$.


Denote $n_c$ the number of correctly matched pairs in set $S$ of seed matches, and $n_w$ the number of wrongly matched pairs in $S$. We give Lemma~\ref{lemma1} as follows.
% new setting
%(1) the order-1 information is considered only; % i.e., a matched pair $[u,v]$ adds $min\{\frac{deg(u)}{deg(v)}, \frac{deg(v)}{deg(u)}\}$ to each of its neighboring pairs.
%(2) a pair can be matched if it receives score from at least 2 neighboring pairs, and its score is greater than that of all its adversary pairs by a factor $\beta$. % relevant to maximal degree

\begin{lemma}\label{lemma1}
In the $G(n,p;p_n,p_e)$ random graph model, assume the above percolation method and matching criteria are adopted, in each iteration, the postponing strategy decreases the probability of a wrong pair being matched
from $(n_c+n_w)^2 p^4p_e^4$ to $(n_c+n_w)^2 p^4 p_e^4 - n_c^2 p^4 p_e^4 (2p_e^4-p_e^8+ 2 p_n^2 p_e^4 - 2p_n^4 p_e^4)$, and decreases the probability of a correct pair being matched
from $n_c^2 p^2 p_e^4$ to $n_c^2 p^2 p_e^4 (1-np^2)$.
\end{lemma}

The proof of Lemma~\ref{lemma1} is included in appendix. Obviously, the postponing strategy greatly decreases the number of pairs that are wrongly matched.
Assume $p_n=1$ (say $V_{1,2}=V$) and $n_w=0$ (no wrong matches in the seed set),
then the probability of a wrong pair $[v,u]$ being matched in the next iteration is $p^4p_e^4 n_c^2(1-p_e^4)^2$, which is decreased nearly by $10$ times when the edge sampling probability $p_e=0.9$, compared to a probability of $p^4 p_e^4 n_c^2$ without the postponing strategy. In two isomorphic graphs, with $p_n=1$ and $p_e=1$, then no wrong pairs can be matched if all initial seeds are correct. This will also be verified in the experiments as our algorithm achieves a precision of $1$ in matching two isomorphic graphs.
Because $np$ is a constant greater than $1$ and $\frac{1}{p^2}\gg n$, thus $n_c^2 p^2 p_e^4 (1-np^2)$, the new matching probability of a correct pair, is very close to $n_c^2 p^2 p_e^4$. By replacing the matching probability (for correct pairs and wrong pairs) in Theorem 1~\cite{kazemi2015growing} with the new probabilities derived above, we can conclude that the postponing strategy increases the matching precision greatly while not affecting the overall recall by much.



\vspace{0.1cm}
\noindent
\textbf{Property of PPR.}
We will show that the $signature$ vector $R(v)$ of vertex $v$ illustrates $v$'s region information and local structure information.
The PPR value $\pi(s, v)$ of $v$ w.r.t. any seed $s$ can be decomposed into two parts:
(1) the probability that a decaying random walk terminates at vertex $v$ the first time it arrives at $v$, denoted by \textbf{$\pi_1(s, v)$};
(2) the probability that a decaying random walk terminates at vertex $v$ after arriving at vertex $v$ for more than once, denoted by \textbf{$\pi_2(s, v)$}.

Following the analysis in Section~\ref{22PPR}, we use $LS(v) = [\sum_{t=1}^{\infty}\PP^{t}\cdot P^{t}\cdot e_v]_v$ to denote the summed probabilities that a decaying random walk starting from $v$ reaches $v$ after step $1,2,3 \cdots$, then
\begin{equation}\label{LS}
\pi_2(s, v) = \pi_1(s, v) \times LS(v).
\end{equation}
Thus the PPR value $\pi(s, v)$ can be presented by
\begin{equation}\label{ep_PPRdecompose}
\begin{split}
\pi(s, v) = \pi_1(s, v) +\pi_2(s, v) & = \pi_1(s, v) \cdot(1+LS(v)). %\pi_1(s, v) + \pi_1(s, v)\cdot LS(v) \\
                                           % & =
\end{split}
\end{equation}

We first provide the analysis for $\pi_1(s, v)$.
Note that  $\frac{\pi_1(s, v)}{\SP}$ represents the summed probability that a decaying random walk from $s$ hits vertex $v$ for the first time at iteration $0, 1, 2\cdots$.
With a sufficient number of source vertices in $S$, the region information of vertex $v$ can be represented in a way by all $\frac{\pi_1(s_k, v)}{\SP}$ for $1\le k \le |S|$.
To be more specific, given a number of correct seed matches as the source vertices on two graphs, w.h.p. $v\in V_1$ and $u\in V_2$ are on the aligned region over two graphs if and only if $\frac{\pi_1(s_k, v)}{\SP}$ and $\frac{\pi_1(s'_k, u)}{\SP}$ are relatively close w.r.t. a certain number of seed pair $[s_k, s'_k]$.

We further analyse the property of $LS(v)$.
Recall that $LS(v) = [\sum_{t=1}^{\infty}\PP^{t}\cdot P^{t}\cdot e_v]_v$ is independent of the source vertex of random walk, but relevant to vertex $v$ and graph $G$.
We say $LS(v)$ demonstrates the graph structure information around vertex $v$, and vertices with similar local structures tends to have close $LS$ values.
For instance, consider the probability that a random walk arrives at $v$ at the first two iterations, we denote it by $LS^{(2)}(v)$.
Assume there is no self-loop in graph, a random walk from $v$ cannot return $v$ after one step, then % we have
\begin{equation}
\begin{split}
LS^{(2)}(v) & = [\PP^{2}\cdot P^{2}\cdot e_v]_v  \\
            & = \PP^{2}\cdot \frac{1}{|N(v)|} \sum_{(v,u)\in E}\frac{1}{|N(u)|}
\end{split}
\end{equation}
Thus $LS^{(2)}(v)$ represents the average reciprocal of degree of all neighbors of vertex $v$, containing the order-2 structural information of $v$.
Accordingly, the arriving probability of further iterations $LS^{(t)}(v)$ ($t>2$) contains the higher order structural information of $v$, the impact of which, however, is decayed by the factor $\PP^t$ over iterations.


\vspace{0.1cm}
\noindent
\textbf{Analysis of $\SP$.}
The proceeding probability of random walk in PageRank often varies in different cases. A discussion has been presented in~\cite{gleich2010inner}.
Most works on web search~\cite{kamvar2003extrapolation, najork2007hits} adopt the large stopping probability ($\SP=0.95$ or $0.9$) s.t. the power method can converge fast.
\cite{avrachenkov2007distribution} selects small $\SP$ ($\SP = 0.5$) to prevent
the Pure-Out vertices (which have links from strongly connect components but not back) from having very large PageRank values.
We also set a small $\SP$ (empirically $1-\frac{\sqrt{2}}{2} \approx 0.3$) in this paper, but for a different reason.

In PPRGM, we measure the matching score of $[v,u]$ w.r.t. matched pair $[s,s']$ by comparing $\pi(s,v)$ and $\pi(s',u)$.
When $\mathtt{Score}_k(v,u)$ is computed,
the difference between $q_{s_kv}^{(t)}$ and $q_{s'_ku}^{(t)}$, two probabilities w.r.t. $t$-step non-decaying random walks,
is scaled by $\PP^t$ (see Equation~\ref{ep_score11}). Consequently, the choice of $\SP$ corresponds a leverage over the effect of random walk paths of different lengths:
(1) If a large $\SP$ is set, the matching score is likely sensitive to low-order structural difference, while be blind to higher order structure.
Recall that we need to set $\lambda>2/3$ (i.e., $\alpha\le 1/3$) in the case of Figure~\ref{MatchingExample},
otherwise $[v_2,u_1]$ is wrongly matched because the order-1 alignment of $(s_2,v_2)\in E_1$ and $(s'_2,u_1)\in E_2$ suppresses the order-2 structural difference between $v_2$ and $u_1$;
(2) If a very small $\SP$ is set, the effect of long random walk paths on matching score, which is less reliable, cannot be properly depreciated.
Thus we empirically use $\SP=0.3$ to balance the impact of low-order
structural information and higher-order structural information and make the matching score robust to the cross-graph structural difference.


==> 4pprgm.tex <==

\section{PPRGM Algorithm} \label{4PPRGM}
In this section, we present the details of our PPRGM framework. %an effective and robust graph matching method.
We first provide the function that is used in our algorithm to measure the matching scores of a pair, which is a function of the PPR vectors of the two nodes. %The score of a pair represents the likelihood of its being matched.
Then we present our main algorithm followed by
several practical strategies to further boost the matching precision. %by postponing matching pairs of low credibility.
%Next, we introduce a percolation and local PPR-based labelling method, which complements the deficiency of the global labelling. The algorithm exploits all global and local labels to evaluate each node pair.
Lastly, we provide an analysis on the effectiveness of the PPRGM algorithm on random graphs.

\subsection{Score Function} \label{4score}
%A score function is defined on two PPR vectors to measure the likelihood that the two nodes are aligned.

%Given a set of seeds $S$ on graph $G$, we conduct a personalized PageRank approximation on each seed $s_k$ (as the source) by using the Forward-Push with the same stopping probability $\alpha$ and the same residue threshold $r_{max}$. The PPR value of node $i\in V$ w.r.t. $s_k$ is $\pi(s_k, i)$, and the PPR vector of node $i$ is $R(i) = \{\pi(s_1, i), \pi(s_2, i), \cdots, \pi(s_{|S|}, i) \}$. We take the PPR vector as the global label for each node. It can be shown the PPR vector of each node illustrates both its region information and local structural information in Appendix~\ref{7ppr}.

Given the vectors  $R^1(i)= \{\pi(s^1_1, i), \pi(s^1_2, i), ..., \pi(s^1_{|S|}, i) \}$ for node $i\in V_1$ and $R^2(j)= \{\pi(s^2_1, j), \pi(s^2_2, j), ..., \pi(s^2_{|S|}, j) \}$ for node $j\in V_2$, the $\mathtt{PPRScore}$ w.r.t. the $k$th seed pair is defined as
\begin{equation}\label{pprscore1}
\mathtt{PPRScore_k}(i,j) = \frac{\min{(\pi(s^1_k, i),\pi(s^2_k, j))}}{\max{(\pi(s^1_k, i),\pi(s^2_k, j))}+\sigma}.
\end{equation}
The score of $[i,j]$ is simply the sum over all seeds:
\begin{equation}\label{pprscore2}
\mathtt{PPRScore}(i,j) = \sum_{k=1}^{|S|} \mathtt{PPRScore_k}(i,j).
\end{equation}
Here $\sigma$ is a parameter that will be explained shortly.

%We assume that the pair with a higher $\mathtt{PPRScore}$ is more likely to be a true match, i.e., for two pairs $[i,j]$ and $[i,j']$, if $\mathtt{PPRScore}(i,j)>\mathtt{PPRScore}(i,j')$, then node $i$ is more likely to be matched with node $j$ rather than the node $j'$.
% (No result yet) A mathematical analysis on random graph will be presented later to show the score function works.

%Recall that $\pi(s_k, i)= \pi_1(s_k, i) \cdot(1+LS(i))$, the $|\pi^1(s^1_k, i)-\pi^2(s^2_k, j)|$ measures the absolute difference between node $i$ and node $j$ with respect to both the region information in the perspective of seed pair $[s^1_k, s^2_k]$ and the structural information.
%It should be noticed that there is no trivial way to approximately decompose $\pi(s_k, i)$ into $\pi_1(s_k, i)$ and $(1+LS(i))$ for each node $i$ efficiently with time complexity quadratic in $|V|$.
For each $k$, we consider pairs with closer PPR values w.r.t. the $k$th seed as pairs that are more likely to be valid matches, which is reflected in Equation \eqref{pprscore1}. % mainly due to the decaying factor $\alpha$ of the random walk.
On the other hand, we don't want to rely too much on small PPR values:
%The parameter $\sigma$ is used for the following purposes:
(1) nodes with small PPR values are often far away from the corresponding seed, and thus two similar but small PPR values may not be a good evidence for matching;
%and is likely to suffer from the unmatched structures assuming the cross-graph unaligned structures are uniformly distributed, thus it is not trusty;
(2) a small PPR value is likely to have large relative error either due to limited numerical precision or computational errors from the Forward-Push method (which is relevant to $r_{max}$), which makes the score unstable.
Therefore, we put an additional term $\sigma$ in the denominator to reduce the impact from small PPR values and make the score function more stable as well.
We empirically set $\sigma$ to be \emph{$10$ times the residue threshold} $r_{max}$ used in the Forward-Push.
Basically, a node with a very small PPR value compared to $\sigma$ can be regarded as \emph{unlabeled} in this dimension.

The overall $\mathtt{PPRScore}(i,j)$ is defined as the sum of scores over all seed pairs to make the scores more robust against wrong matches.
%Note that, for a pair of nodes that should be matched, their PPR vectors may have large relative differences on a few dimensions (i.e., small values of $\mathtt{PPRScore}_k(i,j)$), resulting from the unaligned structures or a portion of incorrect seed pairs.
%While the defined score function tolerates it by focusing on the overall difference w.r.t. all seed pairs.


\subsection{Main Algorithm}\label{4main}
We will first present a basic version of PPRGM.
Given two unlabeled graphs and a set of seed matches, the PPRGM algorithm first labels each node with a PPR vector; each dimension is the PPR value w.r.t. the corresponding seed.
Then PPRGM iteratively expands the candidate set and the matched set as follows: (1) the algorithm includes the neighboring pairs of matched pairs into the candidate set, and computes their scores using the Equation~\eqref{pprscore2}; (2) the PPRGM greedily matches the candidate pair with the highest score each time.
%We recall that it is infeasible to find a matching solution to obtain the maximal summed score because computing the $\mathtt{PPRScore}$ for all possible pairs is costly in time (as discussed in Section~\ref{2PGM}).
%, and the score of each pair varies during the matching process.


%\begin{procedure}[!tb]
%\caption{1: Check-Strong-Candidate(C, i, j, $\beta$)}\label{proc:CSC}
%%\caption{CheckTie(set AC, set C, node i)}\label{proc:checkforAC}
%	\KwIn{set $C$, pair $[i,j]$, ratio $\beta$;}
%
%    \If{$\exists[i,j']\in C$ s.t. $(1+\beta)\cdot \mathtt{Score}(i,j')>\mathtt{Score}(i,j)$}
%    {
%        \Return {False;}
%    }
%    \If{$\exists[i',j]\in C$ s.t. $(1+\beta)\cdot \mathtt{Score}(i',j)>\mathtt{Score}(i,j)$}
%    {
%        \Return {False;}
%    }
%    {
%        \Return {True;}
%    }
%\end{procedure}

\noindent
\textbf{Postponing strategies.}
In addition, we propose new postponing strategies to improve the matching precision: the match of a \emph{uncertain} pair should be postponed even if it currently has the highest score among the candidate set.
To illustrate this,  we first introduce a few definitions.
We define \emph{adversary pairs} of $[i,j]$ as the set of all pairs in $\{i\}\times V_2$ and $ V_1\times \{j\}$, which are the direct competitors of $[i,j]$.
%Any correct match $[i,j]$ cannot be matched if any one of its adversary pairs is matched first, which should be avoided.
For any score function $\mathtt{Score}(,)$, we say $[i,j]$ has no $\beta$-close adversary pairs for some $\beta>0$, if it satisfies $\mathtt{Score}(i,j)>(1+\beta)\mathtt{Score}(i',j')$ for all adversary pairs $[i',j']$ of $[i,j]$ simultaneously. Let $C$ be the candidate set.
%The details of checking strong candidate pairs is shown in Procedure 1. %~\ref{proc:CSC}.

%The reasons behind that are obvious:
%(1) since the candidate pairs are generated gradually, an incorrect pair in the candidate set may have lower score than its corresponding true matches, which have not been added to candidate set;
%(2) the identification of an uncertain pair will be assisted by the matching of its neighboring pairs.
Assume $[i,j]$ is a correct pair. As we are generating and matching candidate pairs iteratively, the following \emph{bad cases} may happen:

(1) $[i,j']\in C$, $[i,j]\notin C$, although $\mathtt{Score}(i,j)>\mathtt{Score}(i,j')$; %and hereby $[i,j]$ is wrongly matched;

(2) $[i,j]\in C, [i,j']\in C$, but currently $\mathtt{Score}(i,j')$ is
slightly higher than $\mathtt{Score}(i,j)$. %and $[i,j]$ is wrongly matched.

To avoid wrong decisions, we will postpone the matching of $uncertain$ pairs. We call a pair $[i,j]$ is \emph{not uncertain}, referred to as a \emph{strong candidate pair}, if
(1) $\mathtt{Score}(i,j)\ge \gamma$ where $\gamma$ is a predefined score threshold; and
(2) $[i,j]$ has no $\beta$-close adversary pairs. If a pair is not a strong candidate, it is uncertain. Using this strategy, we may avoid the bad cases mentioned above, because the wrong match $[i,j']$ is likely an uncertain pair in both cases. The effectiveness of the postponing strategy will be analyzed in Section~\ref{4analysis1}.


%because
%(1) In the first case, we may include $[i,i]$ into $C$ afterwards and match pair $[i,i]$ correctly;
%(2) In the second case, we may add $[j,j]$ to $C$ later with $\mathtt{Score}(j,j)>\mathtt{Score}(i,j)$, thus $[j,j]$ and $[i,i]$ can be correctly matched sequentially.

%Motivated by this, we only match pair $[i,j]$ which is $not$ $uncertain$, referred as to a \emph{strong candidate pair}, if $[i,j]$ satisfies the following conditions:

%Note that an $uncertain$ pair may be transformed into a strong candidate later when the factor $\beta$ is decreased, or when its adversary pair is pruned as the node $i'$ ($j'$) involved is preferentially matched to other node.




%[!t]
\begin{algorithm}[!tb]
\caption{Personalized PageRank Graph Matching}\label{alg:PPRGM}
%\begin{algorithmic}[1]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input {$G_1(V_1, E_1), G_2(V_2, E_2)$, seed set $S$ of correct matches, stopping probability $\alpha$, residue threshold $r_{max}$}
    \Output {The set of matched pairs $M$}

    initialize candidate pair set $C\leftarrow\Emptyset$, strong candidate pair set $Q\leftarrow\Emptyset$, $\beta\leftarrow2$;

    \ForEach {seed pair $[s^1_k, s^2_k]$}{
       $R^1_k$ $\leftarrow$ Forward-Push$(G_1, s^1_k, \alpha, r_{max})$;\\
       $R^2_k$ $\leftarrow$ Forward-Push$(G_2, s^2_k, \alpha, r_{max})$;
    }

    insert each seed pair $[s^1_k, s^2_k]$ into $Q$;

    \While{$C\ne \Emptyset$ and $\beta>1+\epsilon$}{
    	\ForEach { strong candidate pair $[i,j]\in C$  w.r.t. $\beta$}{
    		insert $[i,j]$ into $Q$;
    	}
    	\While{$Q \ne \Emptyset$}{
    		find $[i,j]\in Q$ with highest $\mathtt{Score}(i,j)$;\\
    		%\If {$\mathtt{Score}(i,j)<\gamma$}{
    		%	break;
    		%}
    		mark $i, j$ as matched, insert $[i,j]$ into $M$;\\
    		remove all adversary pairs of $[i,j]$ from $C$;\\ %$[i,j']$ and $[i',j]$
            \textbf{Neighbor-Expansion($i, j$)};
    	}	
        update $\beta \leftarrow (\beta+1)/2$;\\
    }
    \Return {M}

\end{algorithm}

\begin{procedure}[!tb]
\caption{2: Neighbor-Expansion($i, j$)}\label{proc:NE}
	\ForEach {neighboring pair $[i_p,j_q]$ of pair $[i,j]$}{
    	\If {$i_p$ or $j_q$ is matched or $[i_p, j_q]\in C$}{
            continue;
        }

    	$\mathtt{Score}(i_p, j_q)\leftarrow \mathtt{PPRScore}(R^1(i_p), R^2(j_q))$;\\
    	insert $[i_p, j_q]$ into set $C$;\\
        \If {$[i_p, j_q]$ is a strong candidate pair w.r.t. $\beta$}{
    		insert $[i_p, j_q]$ into $Q$;
        }
    }
\end{procedure}


\noindent
\textbf{Algorithm.} The PPRGM algorithm is presented in Algorithm~\ref{alg:PPRGM}.
Given two graphs $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$ to be matched and a seed set $S$. %with correct matches.
The algorithm initializes a set $C$ for storing candidate pairs and a set $Q$ for storing strong candidate pairs. The parameter $\beta$ in the definition of strong candidate is initialized to $2$.
Firstly, the algorithm conducts a pair of personalized PageRank computation for each seed pair, and labels the nodes on each graph with a PPR vector (line 2-5).
Then each seed pair is inserted into candidate set $Q$ (line 6).
In the process of matching, the algorithm starts a while-loop, which repeats as long as the candidate set is not empty and the factor $\beta$ is greater than a threshold.
In each round, it checks each candidate pair and inserts it into $Q$ if it is a strong candidate pair w.r.t. $\beta$ (line 8-10).
In the nested while-loop, whenever the set $Q$ is not empty, the algorithm always fetches the pair $[i,j]$ with the highest score (the score is greater than $\gamma$ because $[i,j]$ is a strong candidate pair) as a match, removes %the pairs that will not be matched ($[i,j']$ or $[i',j]$)
all adversary pairs of $[i,j]$ from $C$, and calls the procedure \emph{Neighbor-Expansion} (line 11-19). The \emph{Neighbor-Expansion} (see Procedure 2) inserts the neighboring pairs of $[i,j]$ into $C$ along with their scores, and inserts the strong candidate pairs among them into $Q$.
When there are no available elements in $Q$, the algorithm relaxes the requirement for strong candidate pairs by decreasing the $\beta$ (line 20), and repeats the outer-loop.
Finally, the algorithm terminates when the candidate set is empty or when $\beta$ is below a threshold.



\subsection{Extended PPRGM}\label{4expand}
In the above basic version of PPRGM, the score of any pair is computed based on the PPR values w.r.t. the initial seed set only. However, it is natural to consider the early matched pairs as new evidence to match other unmatched pairs as in the PGM framework; utilizing more evidence is helpful to eliminate the bad case (2) above.
On the other hand, the above PPRGM only adds the neighboring pairs of already matched pairs to the candidate set. To avoid the bad case (1) mentioned above, we will expand more aggressively by including a local neighborhood of a matched pair.

%\noindent
%\textbf{Motivation.}
%Though the graph labelling based on Personalized PageRank vector is effective in graph matching, it has limitations. The PPRGM framework tends to match pairs with the high $\mathtt{PPRScore}$ first. The effectiveness of evaluating the pairs based on PPR vectors decays while the algorithm is dealing with the pairs with low $\mathtt{PPRScore}$.
%Note that a correct match $[i,j]$ can have a low $\mathtt{PPRScore}$  as a result of the structural difference across two graphs. In this case, pair $[i,j]$ is more likely to have adversary pairs with higher $\mathtt{PPRScore}$, thus may not be correctly matched.
%To amend this, we turn to the pairs that have been matched before $[i,j]$, which have higher credibility ($\mathtt{PPRScore}$) and may suffer less from the unaligned structure. These matched pairs can provide guidance in eliminating the effect of structural difference that lies on the paths from the seeds to them.

%A straightforward idea is to align the two PPR vectors of each matched pair by editing two graphs (deleting the edges and nodes). If the two graphs are isomorphic after being edited, then the corresponding nodes have the identical PPR vectors. For example, assume $N(i_1)=\{i_2,i_3\}$ for $i_{1,2,3}\in V_1$ and $N(j_1)=\{j_2\}$ for $j_{1,2}\in V_2$, once $[i_1,j_1]$ and $[i_2, j_2]$ are matched, we remove $(j_1,j_3)\in E_2$ to align the structures in two graphs, and update the PPR vectors of nodes in $V_2$ with an efficient dynamic PPR approximation method~\cite{zhang2016approximate}.
%However, the graph editing method above is not robust to the wrong matches, because it trusts each matched pair and edits graphs accordingly, which fully determines the evaluation of unmatched pairs.
%Besides, a large number of graph edits and dynamic PPR approximation incurred lead to a high time cost.

%Instead of adopting the graph edit method, we use a percolation and local labelling method to exploit the matched pairs in this paper. Note that the influence of early matches on the unmatched pairs can be regarded as a bias, w.r.t. the effect of global labelling applied by the seeds. The proposed method achieves a balance between both kinds of effect (from the  seeds and from the early matches), and it is more efficient than the graph edit method because it has each match affect the pairs within a local range only.

%We use a percolation and local labelling method to exploit the matched pairs in this paper. Note that the influence of early matches on the unmatched pairs can be regarded as a bias, w.r.t. the effect of global labelling applied by the seeds. The proposed method achieves a balance between both kinds of effect (from the  seeds and from the early matches). %, and it is more efficient than the graph edit method because it has each match affect the pairs within a local range only.



\begin{algorithm}[!tb]
\caption{Extended PPRGM}\label{alg:ESPPRGM}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input {$G_1(V_1, E_1), G_2(V_2, E_2)$, seed set $S$ of correct matches, stopping probability $\alpha$, residue threshold $r_{max}$}
    \Output {The set of matched pairs $M$}

%\Procedure{PPRGM}{$ $}
    %initialize set of matched pairs $M=\Emptyset$, set of matched vertices $VM_1=\Emptyset$ and $VM_2=\Emptyset$,
    %, ratio for checking strong candidate $\beta=2$, and score threshold $\gamma$;
    initialize candidate pair set $C\leftarrow\Emptyset$, strong candidate pair set $Q\leftarrow\Emptyset$, expanding seed set $A\leftarrow\Emptyset$, and $\beta\leftarrow2$;

    \ForEach {seed pair $[s^1_k, s^2_k]$}{
       $R^1$ $\leftarrow$ Forward-Push$(G_1, s^1_k, \alpha, r_{max})$;\\
       $R^2$ $\leftarrow$ Forward-Push$(G_2, s^2_k, \alpha, r_{max})$;
    }

    insert each seed pair $[s^1_k, s^2_k]$ into $Q$;

    \While{$C\ne \Emptyset$ and $\beta>1+\epsilon$}{
        \ForEach { strong candidate pair $[i,j]\in C$  w.r.t. $\beta$}{
    		insert $[i,j]$ into $Q$;
    	}
    	\While{$Q \ne \Emptyset$}{
    		find $[i,j]\in Q$ with highest $\mathtt{Score}(i,j)$;\\
    		%\If {$\mathtt{Score}(i,j)<\gamma$}{
    		%	break;
    		%}
    		mark $i, j$ as matched, insert $[i,j]$ into $M$;\\
    		remove all $[i,j']$ and $[i',j]$ w.r.t. $i$ and $j$ from $C$;\\
            insert $[i,j]$ into $A$;
    	}
        \eIf {$A\ne\Emptyset$}{
            \ForEach {pair $[i,j]\in A$}{
        		\textbf{First-Order-Expansion($i, j$)};
        	}
            $A\leftarrow\Emptyset$;
        }
        {
        	update $\beta \leftarrow (\beta+1)/2$;\\
        }
    }
    \Return {M}
\end{algorithm}


\noindent
\textbf{Extended PPRGM.}
%The PPRGM framework with percolation is introduced then.
In the extended PPRGM, each pair $[i,j]$ that is added to the matching set is considered as a new and unused seed pair. We may start a Forward-Push from $[i,j]$ to compute the PPR values of other nodes w.r.t. the new seed, then add a new label to the PPR labeling of each node. However, to save the computation time, the Forward-Push from new seeds will stop much earlier. We distinguish two cases.
%the new seeds from the initial ones by stopping .
In the first case, we only allow the Forward-Push from new seeds to infects its neighboring pairs, which is referred to as First-Order-Expansion (FOE); in the second case, we allow the Forward-Push to infect pairs within a small local range by setting a relatively large residue threshold, which is referred to as Higher-Order-Expansion (HOE). %determined by the $r_{max}$ in Forward-Push process.
%For each infected pair $[i_p, j_q]$, the PPR values of node $i_p$ and $j_q$ from the Forward-Push method are assigned to them as the new local labels.
In both cases, each infected pair $[i_p, j_q]$ in the Forward-Push process is then included to the candidate set, and two local labels computed in FOE or HOE are assigned to node $i_p$ and $j_q$ respectively.
Meanwhile, an increment $inc_{i,j}(i_p,j_q)$ computed from the new labels (according to the score function) is added to the score of $[i_p,j_q]$. %which is computed based on the newly assigned PPR values (local labels) using the Equation (\ref{pprscore1}).
To avoid the ambiguity, we then use $\mathtt{PPRScore}$ specifically for the score measuring the global labels (w.r.t. initial seeds).
Thus the overall score of each candidate pair $[i_p,j_q]$ is computed by
\begin{equation}\label{totalscore}
\mathtt{Score}(i_p,j_q) = \mathtt{PPRScore}(i_p,j_q) + \sum_{[i,j]~\textrm{infects}~[i_p,j_q]} \mathtt{inc}_{i,j}(i_p,j_q).
\end{equation}

The extended PPRGM framework is presented in Algorithm~\ref{alg:ESPPRGM}. %We are introducing its difference from the Algorithm~\ref{alg:PPRGM}.
%Compared to the PPRGM algorithm in Algorithm~\ref{alg:PPRGM},
A set $A$ is used to store the newly matched pairs. When a pair is matched, it is added to both $M$ and $A$. After a round of matching (line 11-16), if the set $A$ is not empty, the algorithm does FOE (or HOE) for each pair in $A$ and then empties $A$  (line 17-21).
%i.e., there are no matches that have not percolated, then ;
Otherwise, the algorithm relaxes the requirement for strong candidate pairs by decreasing $\beta$ as before (line 23).
%the algorithm starts a round of percolation. Each match $[i,j]\in A$ calls a procedure of expansion (i.e., percolation and local labelling, which will be discussed in details later),
Note that all scores considered in the Algorithm~\ref{alg:ESPPRGM} is computed with Equation (\ref{totalscore}), contributed by both the global labels and local labels.




\begin{procedure}[!tb]
\caption{3: First-Order-Expansion($i, j$)}\label{proc:FOE}
	\ForEach {neighboring pair $[i_p,j_q]$ of pair $[i,j]$}{
    	\If {$i_p$ or $j_q$ is matched}{
            continue;
        }
        label $i_p$ with $\pi^1(i, i_p)\leftarrow\frac{1-\alpha}{|N(i)|}$, $j_p$ with $\pi^2(j, j_p)\leftarrow\frac{1-\alpha}{|N(j)|}$;\\
        compute $\mathtt{inc}(i_p, j_q)$ w.r.t. seed pair $[i,j]$;\\
        \eIf {$[i_p,j_q]\in C$}{
            $\mathtt{Score}(i_p, j_q)\leftarrow \mathtt{Score}(i_p, j_q)+\mathtt{inc}_{i,j}(i_p, j_q)$;
        }
        {
            $\mathtt{Score}(i_p, j_q)\leftarrow \mathtt{PPRScore}(R^1(i_p), R^2(j_q))+$\\$\mathtt{inc}_{i,j}(i_p, j_q)$;\\
            insert $[i_p, j_q]$ into set $C$;\\
        }
        \If {$[i_p, j_q]$ is a strong candidate pair w.r.t. $\beta$}{
    		insert $[i_p, j_q]$ into $Q$;
        }
    	%check whether existing strong candidate pairs w.r.t. $i_p$ or $j_q$ are still qualified;	
    }
\end{procedure}

\begin{procedure}[!tb]
\caption{4: Higher-Order-Expansion($i, j$)}\label{proc:HOE}
    $R^1_i$ $\leftarrow$ Forward-Push$(G_1, i, \alpha, r'_{max})$;\\
    $R^2_j$ $\leftarrow$ Forward-Push$(G_2, j, \alpha, r'_{max})$;

	\ForEach {pair $[i_p,j_q]$ s.t. $i_p\in R^1_i$ and $j_q\in R^2_j$}{
    	\If {$i_p$ or $j_q$ is matched}{
            continue;
        }
        compute $\mathtt{inc}(i_p, j_q)$ based on the PPR values of $[i_p,j_q]$ w.r.t. seed pair $[i,j]$;\\
        \eIf {$[i_p,j_q]\in C$}{
            $\mathtt{Score}(i_p, j_q)=\mathtt{Score}(i_p, j_q)+\mathtt{inc}_{i,j}(i_p, j_q)$;
        }
        {
            $\mathtt{Score}(i_p, j_q)= \mathtt{PPRScore}(R^1(i_p), R^2(j_q))+$\\$\mathtt{inc}_{i,j}(i_p, j_q)$;\\
            insert $[i_p, j_q]$ into set $C$;\\
        }
        \If {$[i_p, j_q]$ is a strong candidate pair w.r.t. $\beta$}{
    		insert $[i_p, j_q]$ into $Q$;
        }
    	%check whether existing strong candidate pairs w.r.t. $i_p$ or $j_q$ are still qualified;	
    }
\end{procedure}


\noindent
\textbf{FOE and HOE.}
%We then propose two strategies of percolation with different percolation range, namely the First-Order-Expansion (FOE) and Higher-Order-Expansion (HOE).%, as shown in Procedure 3 and Procedure 4 respectively.
The First-Order-Expansion (see Procedure 3) percolates and labels each neighboring pair $[i_p, j_q]$ of the match $[i,j]$. The algorithm conducts the Forward-Push method from $i$ and $j$ respectively for only $1$ step. Then the PPR values $\pi(i, i_p)=\frac{1-\alpha}{|N(i)|}$ and $\pi(j, j_p)=\frac{1-\alpha}{|N(j)|}$ are assigned to node $i_p$ and $j_q$ respectively as their local labels (line 5). Meanwhile, an increment $\mathtt{inc}_{i,j}(i_p,j_q)$, which is computed on two newly assigned labels with the score function in Equation (\ref{pprscore1}), is added to $\mathtt{Score}(i_p, j_q)$ (line 6-13). The FOE ensures each $[i_p, j_q]$ is included in the candidate set, and also inserts $[i_p, j_q]$ into $Q$ if it is a qualified strong candidate pair (line 14-16).

The main difference between First-Order-Expansion and the percolation in traditional PGM algorithms is that, the traditional percolation always adds $1$ mark to the score of $[i_p, j_q]$, while in the FOE, the increment added to $\mathtt{Score}(i_p, j_q)$ is
$\frac{\min{(\pi(i, i_p),\pi(j, j_p))}}{\max{(\pi(i, i_p),\pi(j, j_p))}+\sigma}=\min\{\frac{|N(i)|}{|N(j)|+\sigma/(1-\alpha)},\frac{|N(j)|}{|N(i)|+\sigma/(1-\alpha)}\}$.
%The FOE defines the increment in this way such that (1) the evaluation of local labels and global labels can be aligned by the same formulation; (2)
When a match $[i,j]$ has small relative degree difference, it contributes high increment to the scores of its neighboring pairs. In other words, a matching pair with smaller degree difference is considered as stronger evidence for later matching, which is in the same spirit as the matching preference used in EWS~\cite{kazemi2015growing}.
%and when $|N(i)|=|N(j)|$, $\mathtt{inc}_{i,j}(i_p,j_q)$ is maximized ($\approx 1$).

The Higher-Order-Expansion (see Procedure 4) is more aggressive than FOE by considering the pairs within a local range of the match $[i,j]$ (instead of its neighboring pairs only). The algorithm starts Forward-Push procedures on source node $i$ and $j$ respectively using a residue threshold $r'_{max}$ much greater than $r_{max}$ (line 1-2). The Forward-Push method determines both the percolated nodes and their corresponding labels (the PPR values). The HOE also computes an increment $\mathtt{inc}_{i,j}(i_p,j_q)$ for each infected pair using the Equation (\ref{pprscore1}) (line 7).
Then, the HOE includes each infected pair into $C$, adds the increment $\mathtt{inc}_{i,j}(i_p,j_q)$ to the $\mathtt{Score}(i_p, j_q)$, and insert $[i_p, j_q]$ into $Q$ if it is a qualified strong candidate pair (line 8-17).

\noindent
\textbf{Comparison of FOE and HOE.}
When $r'_{max}$ is large enough, the HOE is simply equals to the FOE, i.e., each matched pair percolates to its neighboring pairs only. %We simply assume the $r'_{max}$ in HOE is small in the following comparison thus each matched pair affects more than its neighboring pairs .

The FOE is more efficient than HOE, because it infects less number of nodes in each expansion and includes less candidate pairs overall.
The HOE is likely to have higher recall (more correct matches) than FOE,  because more candidate pairs are considered in HOE.
The final matching score of a pair is the combination of labels from initial seeds (global) and labels from early matches (local).
%Different expansion strategies also result in different biases on either the effect of global labelling, or the effect of local labelling.
In HOE, a matched pair infects many unmatched pairs, thus each unmatched pair is likely to receive many local labels, the overall effect of which may overwhelm the effect of global labels. While in the FOE, the global labelling plays a more important role than the local labelling.
Detailed comparison between FOE and HOE, as well as the effect of various $r'_{max}$ will be presented in the experiment section.



%\noindent
%\textbf{Comparison with ExpandOnce algorithm.}
%It is worth mentioning the ExpandOnce algorithm in~\cite{kazemi2015growing} is a special case of our PPRGM framework with HOE strategy. The ExpandOnce doesn't use the global labelling method, and it has each matched pair $[i,j]$ add $\mathtt{inc}(i_p,j_q)=1$ to the score of pair $[i_p,j_q]$, if $dist(i,i_p)=dist(j,j_q)\le k$ where $k$ is a given constant. Formally, the overall score of each candidate pair defined by the ExpandOnce algorithm is
%\begin{equation}\label{EWSscore}
%\mathtt{Score}(i_p,j_q) = \sum_{[i,j]~\emph{infects}~[i_p,j_q]} 1.
%\end{equation}
%Our HOE method achieves better effectiveness than the ExpandOnce algorithm by introducing both the global labelling and the PPR-based local labelling. It is also noted that Theorem 1 in~\cite{kazemi2015growing} proves the robustness of \emph{noisy seed} method in ExpandOnce algorithm, which can be extended to prove the robustness of our local higher-order labelling strategy as well.
%Moreover, the start-of-the-art algorithm EWS~\cite{kazemi2015growing} is based on the same robustness analysis, but practically performs better than the ExpandOnce.
%The comparison between the EWS algorithm and the proposed FOE and HOE will be presented in the experiment section.

%As a result, the value of $N_m(i,j)$ suffers from the incorrect matches, as the \emph{noisy seed set} in PGM algorithms.
%The affect of incorrect matches on PGM has been analysed in~\cite{kazemi2015growing}. The \emph{noise} in $N_m(i,j)$ has a more minor influence on PPRGM compared to that in PGM:
%(i) the effect of bias is limited, while PGM relies only on the noisy neighboring matches;
%(ii) the framework of PPRGM tends to select the trustiest node pairs at each step, thus overall influence of incorrect matches along the process is diminished.


\subsection{Analysis}\label{4analysis}

%\subsection{An analysis of $\Omega(\sqrt(n))$ seeds and the comparison with IsoRank}
%(1) simple proof: how postponing the adversary pairs works.

%(2) medium proof: how pprscore additionally helps distinguishing compared to EWS.

%(3) hard proof: how ppr works on random graph with edge sampling.
 %   sub: may prove the number of seeds required to label all nodes differently with PPR vectors, on two isomorphic random graphs. Though $\Omega(\log(n))$ has been proved in seeded graph matching.

%An analysis on the effectiveness of the PPRGM algorithm will be provided.

We first introduce the $G(n,p;p_n,p_e)$ random graph model that has been used in~\cite{pedarsani2011privacy, kazemi2015growing}. The $G(n,p;p_n,p_e)$ random graph model generates two corrected graphs as follows: (1) a graph $G(V,E)$ is generated from Erd\"os-Renyi random graph, i.e., in a graph of $n$ nodes, each of ${n}\choose{2}$ possible edges occurs with probability $0<p<1$; (2) $V_1$ and $V_2$ are two independent sample sets of $V$, in which each node $v\in V$ is sampled with probability $p_n$; (3) each edge $(i,j)\in E$ s.t. $i,j\in V_1$ is included in $E_1$ with probability $p_e$, and $E_2$ is generated in the same way. We assume that the average degree $np$ is constant, satisfying that the Erd\"os-Renyi random graph has a unique giant component containing a positive fraction of the vertices
with high probability.
The task of graph matching is to identify the correct matches between $V_1$ and $V_2$.

%%!! we should first analyse how 1/deg works in PGM.

%%In the following part, we are going to show (1) the strategy of postponing the matching of pairs with close adversary pairs (referred as to the postponing strategy) helps improve the precision while not affecting the recall; (2) the nodes on random graph can be distinguished by the PPR vector with a limited number of seeds.

%% Currently we analyse the postponing strategy based on a general percolation framework.
%% It is more complicated to prove it in our framework even with order-1 setting. We should deal with differentiation of 1/degree.
%% If connected, label $\pi$ is expected $1/(npp_e)$; otherwise, label is $0$.

\subsubsection{Effectiveness of Postponing Strategy.} \label{4analysis1}
We propose the postponing strategy in Section~\ref{4main}: the match of a pair having close adversary pairs should be delayed.
It will be shown that the postponing strategy greatly decreases the number of pairs that are wrongly matched.

Recall that the adversary pairs of $[i,j]$ are the set of all pairs in $\{i\}\times V_2$ and $ V_1\times \{j\}$. Any wrong node pair $[i,j]$ always corresponds to two correct adversary pairs $[i_1,j]$ and $[i,j_1]$.
Denote $n_c$ the number of correctly matched pairs in the seed set $S$, and $n_w$ the number of wrongly matched pairs in $S$.
For simplicity, we consider a special case in the analysis:
(1) the order-1 information is considered only, and each seed pair adds $1$ mark to its neighboring pair;% (as in Equation~\ref{EWSscore});
(2) a pair can be matched if it has at least $2$ marks, and its score is greater than that of all its adversary pairs.
% new setting
%(1) the order-1 information is considered only; % i.e., a matched pair $[u,v]$ adds $min\{\frac{deg(u)}{deg(v)}, \frac{deg(v)}{deg(u)}\}$ to each of its neighboring pairs.
%(2) a pair can be matched if it receives score from at least 2 neighboring pairs, and its score is greater than that of all its adversary pairs by a factor $\beta?$. % relevant to maximal degree?

\begin{lemma}\label{lemma1}
In the $G(n,p;p_n,p_e)$ random graph model, assume the above percolation method and matching criteria are adopted, the postponing strategy decreases the probability of a wrong pair being matched
from $(n_c+n_w)^2 p^4p_e^4$ to $(n_c+n_w)^2 p^4 p_e^4 - n_c^2 p^4 p_e^4 (2p_e^4-p_e^8+ 2 p_n^2 p_e^4 - 2p_n^4 p_e^4)$, and decreases the probability of a correct pair being matched
from $n_c^2 p^2 p_e^4$ to $n_c^2 p^2 p_e^4 (1-np^2)$.
\end{lemma}

The proof of Lemma~\ref{lemma1} is included in appendix. Obviously, the postponing strategy greatly decreases the number of pairs that are wrongly matched.
Assume $p_n=1$ (say $V_{1,2}=V$) and $n_w=0$ (no wrong matches in the seed set), then the probability of a wrong pair $[i,j]$ being matched in the next iteration is $p^4p_e^4 n_c^2(1-p_e^4)^2$, which is decreased nearly by $10$ times when the edge sampling probability $p_e=0.9$, compared to a probability of $p^4 p_e^4 n_c^2$ without the postponing strategy. In two isomorphic graphs, as $p_n=1$ and $p_e=1$, then no wrong pairs can be matched if all initial seeds are correct. This will also be verified in the experiments as our algorithm achieves a precision of $1$ in matching two isomorphic graphs.
Because $np\to c_1>1$, $\frac{1}{p^2}\gg n$, thus $n_c^2 p^2 p_e^4 (1-np^2)$ is very close to $n_c^2 p^2 p_e^4$. By replacing the matching probability (for correct pairs and wrong pairs) in Theorem 1~\cite{kazemi2015growing} with the new probabilities derived above, we can conclude that the postponing strategy increases the matching precision greatly while not affecting the overall recall by much.

% the ratio of the number of correct matches over the number of wrong matches in each iteration is $\frac{np^2s^4c^2}{n^2p^4s^4(c+w)^2}$, thus postponing strategy will not affect the overall recall.

\subsubsection{Global Labelling on Random Graph.} \label{4analysis2}
In Erd\"os-Renyi random graph, assume $np\ge c_1>1$ where $c_1$ is a constant, then w.h.p. the graph will have a unique giant component containing a positive fraction of the vertices. In the following analysis, we consider the matching on vertices in this giant component only. %as it is rather meaningless and difficult to do matching on the small components (each with no more than $O(\log(n))$ nodes).

Firstly, we define a labelling method based on the shortest path distances, which is a simplified version of PPR labelling. Let $d(s,i)$ be the shortest path distance from node $s$ to node $i$, and $D_{i}=\{d(s_1,i), d(s_2,i), d(s_3,i), \cdots\}$ be the shortest path distance vector of $i$. Then we can show that the nodes in random graph can be distinguished by shortest path distance vector with only a limited number of seeds.

\begin{lemma}\label{lemma2}
In Erd\"os-Renyi random graph, assume $c$ is a large constant, when $\log(n^3)/\log(\frac{cnp}{cnp-1})$ seeds are provided, then $\forall i,j\in V$, $D(i)\ne D(j)$ with probability $1-\frac{1}{n}$.
\end{lemma}

The proof of Lemma~\ref{lemma2} is included in appendix. When $cnp\to c_2>2$ (where $c_2$ is a constant), then a seed set of $|S|\ge O(\log(n))$ will be enough to distinguish each node in Erd\"os-Renyi random graph with a shortest path distance vector.

% Build the connection between the PPR labelling and shortest path distance labelling.
Note the PPR labelling is much complicated than the labelling method above: (1) the decaying in PPR considers the degree of the each node on the random walk path; (2) the PPR value also demonstrates a local structural information, as shown in Section~\ref{4analysis3}; (3) the PPR considers multiple random walk paths from the seed to each node, rather than the shortest paths only. It should be stressed that the PPR based labeling practically has greater power in distinguishing the nodes. %while we use the above simplified version in analysis to avoid much dependency.
% how to PPR.


\subsubsection{Properties of PPR-based Labelling.} \label{4analysis3}
It will be shown the PPR vector of each node illustrates its region information and local structural information.
The PPR value $\pi(s_k, i)$ of node $i$ can be decomposed into two parts:
(i) the probability that a decaying random walk terminates at node $i$ the first time it arrives at $i$, denoted by \textbf{$\pi_1(s_k, i)$};
(ii) and the probability that a decaying random walk terminates at node $i$ after its arriving node $i$ for the first time, denoted by \textbf{$\pi_2(s_k, i)$}.

Following the analysis in Section~\ref{2PPR}, we denote $LS(i) = [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i$ the probability that a decaying random walk which starts from $i$ returns node $i$ after step $1,2,3 \cdots$, then
\begin{equation}\label{LS}
\pi_2(s_k, i) = \pi_1(s_k, i) \times LS(i).
\end{equation}
Thus the PPR value $\pi(s_k, i)$ can be presented by
\begin{equation}\label{PPR3-math}
\begin{split}
\pi(s_k, i) = \pi_1(s_k, i) +\pi_2(s_k, i) & = \pi_1(s_k, i) + \pi_1(s_k, i)\cdot LS(i) \\
                                            & = \pi_1(s_k, i) \cdot(1+LS(i)).
\end{split}
\end{equation}


Note that  $\pi_1(s_k, i)/\alpha$ represents the summed probability that a decaying random walk from $s_k$ hits node $i$ for the first time at iteration $0, 1, 2\cdots$.
An observation is, with a sufficient number of source nodes, the region information of node $i$ can be represented by all hitting probabilities. This can be explained by the proof in~\ref{4analysis2} if we replace the hitting probability with the shortest path distance (a simplified measurement).
When two correlated graphs are considered, we have the following observation: given a number of correct seed matches as the source nodes on two aligned graphs, then with high probability $i\in V_1$ and $j\in V_2$ are on the aligned region across two graphs if and only if they have very similar hitting probability vectors.
Moreover, the region indication ability of the hitting probability vector also has strong robustness to the incorrect seeds.
%Assume then in expectation any pair of two nodes [i,j] %receive simi-
%lar PPR values from this wrong seed. Therefore, a random
%wrong seed merely shifts the score of all pairs by a same
%constant (in expectation), which doesn¡¯t affect the relative
%order of all scores.

%The correctness of which can be partially shown
%Moreover, in a case where the method is provided with a fraction of wrong seeds which are independently sampled, the similarity of two vectors from a coore% (which is $\{\frac{\pi_1(s^1_1, i)}{\alpha}, \frac{\pi_1(s^1_2, i)}{\alpha}, \frac{\pi_1(s^1_3, i)}{\alpha}, \cdots\}$ for $i$).
%, i.e., $\frac{\pi_1(s^1_k, i)}{\alpha}$ and $\frac{\pi_1(s^2_k, j)}{\alpha}$ should be relatively close w.r.t. a certain number of seed pair $[s^1_k, s^2_k]$.

Note that $LS(i)$ is independent of the source node, but relies on $i$ and its local structural information only.
%graph $G$. $LS(i)$ demonstrates the local structural information of each node, and
Thus the nodes with similar local structures tends to have close $LS(i)$ value.
For instance, consider the probability that a random walk arrives at $i$ at the first two iterations, we denote it by $LS^{(2)}(i)$. Since there is no self loop in graph, a random walk from $i$ cannot return to $i$ after $1$ step. Then we have
\begin{equation}
\begin{split}
LS^{(2)}(i) & = [(1-\alpha)^{2}\cdot P^{2}\cdot e_i]_i  \\
            & = (1-\alpha)^{2}\cdot \frac{1}{|N(i)|} \sum_{(i,j)\in E}\frac{1}{|N(j)|}
\end{split}
\end{equation}
%where $|N(j)|$ is the degree of node $j$.
Thus $LS^{(2)}(i)$ represents the average reciprocal of degree of all neighbors of node $i$ normalized by $(1-\alpha)^{2}$, which indicates the second-order local structural information.
Accordingly, the arriving probability of further iterations $LS^{(r)}(i)$ ($r>2$) embodies the higher-order local structural information of node $i$, the impact of which, however, is decayed by the factor $1-\alpha$ over iterations.


\subsubsection{Stopping Probability $\alpha$ in PPR.} \label{4analysis4}
The stopping probability of random walk in PageRank often varies in different applications. A discussion has been presented in~\cite{gleich2010inner}.
Most works on web search~\cite{kamvar2003extrapolation, najork2007hits} adopt a high stopping probability (e.g. $\alpha=0.95$ or $0.9$), and thus the power method can converge fast.
\cite{avrachenkov2007distribution} selects small stopping probability ($\alpha = 0.5$), as it prevents the Pure-Out nodes (which have links from the strongly connect components but not back) from having very large PageRank values.
We also set a small $\alpha$ (empirically $1-\frac{\sqrt{2}}{2}\approx 0.3$) in this paper, but for a different reason.

In graph labelling, the choice of $\alpha$ corresponds to the biases on either the region information ($\pi_1(s_k, i)$) or the local structural information ($LS(i)$).
With a large $\alpha$, the PPR values of nodes are highly distinguished on the hitting probability of the random walk, i.e., the nodes near the source node tend to have large PPR values; and the algorithm conducts more Forward-Push iterations on these nodes with high PPR values. %But in this case, the algorithm is sensitive to the unaligned structures in two network graphs.
On the other hand, the PPR values are more determined by the nodes' local structure if a small $\alpha$ is used. We empirically set $\alpha=0.3$ to balance two kinds of effect on PPR values and make the labeling robust to cross-network unaligned structures.


% shortest path with decaying factor + (distance=1,2,3,... + multiple paths + 1/deg) = PPR
% but hard to say: different shortest distance -> different PPR.
% intuitively, cannot be distinguished by shortest distance vector -> cannot be distinguished by PPR vector
% 1. discard the setting of 1/deg: set decaying factor = 1/2np, the summed value still converges to c<1
% a random decaying factor w.r.t. a vector of all distances?  multiple distances or multiple paths may lead to dependency.

% what if $np\to \log(n)$

%\textbf{Part3.}
%Recall that the ExpandOnce algorithm has been shown as a special case of our PPRGM framework with HOE in Section~\ref{4expand}. The outstanding matching ability of ExpandOnce algorithm as well as its robustness has been proved in Theorem 1 of~\cite{kazemi2015growing}. Here we take the PPR labelling method as an additional strategy based on ExpandOnce, and show how it additionally increases the matching precision.

%For simplicity,
%have to re-read part 1 first.

%Given random seed $s$ and node $i$, the PPR value of $i$ follows a distribution $\mathcal{D}$. When the random graph is constructed, i.e., each edge is sampled with probability $p$, the PPR value of $i$ follows another distribution $\mathcal{D}_i$ derived from $\mathcal{D}$ w.r.t. edge sampling. $\mathcal{D}_i$ and $\mathcal{D}_j$ have dependency as the computation shares the same set of edges. Prove $v_1$, $v_2$ from $\mathcal{D}_i$ has higher score w.r.t. the score function than that of $v_1$, and $v_3$ from $\mathcal{D}_j$.

% try to prove:
%with a certain probability, cannot be distinguished, e.g., same PPR vector. with subtle probability score(i,i')<score(j,i'), may be solved by the postponing strategy.
%with a certain probability, score(i,i')\gg score(j,i'), can be distinguished.










%add or not
%\subsection{Merge seeds}
%\textbf{Not sure if need this part.}
%Whenever a pair is inserted into the candidate set, the algorithm calls the function in equation (\ref{pprscore2}) to compute $\mathtt{PPRScore}$, with $O(|S|)$ complexity. We propose a strategy to speed up the computation by merging the seeds, more precisely, merging the PPR values of each node w.r.t. to the initial seed set.
%
%Intuitively, we always merge two seeds that are most relevant, i.e.,  seed $p$ and $q$ has highest PPR value w.r.t. each other, against any other pair of seeds.
%For each seed in the graph, we compute a personalized PageRank with it as the source node. Then we sort all nodes labelled by this PPR in a descending order of PPR value and have a PPR sequence w.r.t. this seed.
%Given any two seeds $p$ and $q$ in a graph, we obtain two sequences. XXX We find two longest consecutive sub-sequence that are highly similar, i.e., two seeds have the similar effect in labelling this subsequence.  When all nodes before this sub-sequence are matched, then two seeds should be merged.
%XXX.
%%add or not
%\subsection{Flexibility of PPRGM}
%
%\textbf{Not sure if need this part.}
%%\subsubsection{PPRGM on dynamic graph}
%In this section, we will show the flexibility of PPRGM with two cases.
%
%\subsubsection{PPRGM on real graph}
%\textbf{Not sure if need this part.}
%\textbf{have not proved in experiments.}
%
%In the literature of graph matching, the analysis always focus on a special way of constructing the aligned graphs: given an original graph $G(V,E)$, firstly the algorithm samples each node $i\in V$ with a probability of $pn$ and obtains $V' \subset V$, then the algorithm samples each edge $(i,j)$ s.t. $i\in V'$ and $j\in V'$ with probability of $pe$ and obtains $E'\subset E$, thus $G'(V', E')$ is a subgraph of $G$. Each graph to be matched is constructed in this way.
%However, in the real world applications, the overlap between the graphs is not always uniformly distributed. For example, in the social network, a relationship between two users who share multiple common friends is more likely to exist in aligned networks, i.e., the probability of a edge $(i,j)$ existing in the subgraph is proportional to the number of common neighbors shared by $i$ and $j$.
%
%Our PPRGM framework can deal with this skewed graph generation model with a slight modification, i.e., PPRGM adopts a biased random walk while doing labelling with the personalized PageRank. The reason behind this is that we tend to trust the nodes that share more common neighbors with the matched nodes. XXX . While none of the former works can be easily transferred to deal with this graph model.
%
%
%\subsubsection{PPRGM on weighted graph}
%\textbf{Not sure if need this part.}
%analysis for weighted graph.
%Two isomorphic graph with different edge weight.
%PPR denote the LS difference.
%EWS cannot easily extend to because integer
%graph matching


==> Former_1introduction.tex <==
\section{Introduction}\label{sec1}
In many applications such as protein-network alignment, social network de-anonymization, and pattern recognition, an ubiquitous task is to match two networks from different domains by building a bijection between the two vertex sets.
The input graphs to be matched are often unlabeled, and thus the algorithm needs to construct the matching relying solely on the structural information, which is a generalization of the classic graph isomorphism problem.
%The graph matching in the absence of node or edge attributes is more challenging, and the approaches based on structures can be further integrated with label analysis and work on the labeled graphs.
% It is also feasible to transform the labelled graphs into heterogeneous graphs, and apply the structure-based graph matching approach on them.
%Motivated by this, this paper studies on the graph matching problem on the unlabeled graphs.

More formally, we are given two graphs, $G_1(V_1, E_1)$ and $G_2(V_2, E_2)$, where the two node sets $V_1$ and $V_2$ presumably %(partially)
corresponds to the same set of entities.
For instance, $G_1$ and $G_2$ here could be the user networks of Facebook and Twitter respectively.
The graph matching problem aims to identify all pairs of vertices $[i,j]\in V_1 \times V_2$ such that $i$ and $j$ correspond to the same entity. In general $V_1$ and $V_2$ may only have a partial overlap.
%The graph matching is a generalization of the graph isomorphism problem.

In this paper, we further assume that the algorithm is provided with a small set of ``pre-matched" node pairs in the beginning; this assumption is also adopted in a line of work~\cite{yartseva2013performance, korula2014efficient, kazemi2015growing, zhou2016cross, shirani2017seeded}. We call this the \emph{seeded graph matching} problem.

%an assumption is made that additional side information is provided in the form of seed matches, i.e., a set of correct matches are identified as the prior knowledge.
Such an assumption is reasonable in many practical scenarios.
For example, two social networks are constructed based on Instagram and Facebook respectively: each node represents a user, and the network contains an edge $(i,j)$ if a user $i$ is followed by another user $j$. A graph matching task is to identify pairs of accounts on two networks that belong to the same individual. It is noted that many users on Instagram may connect to their Facebook accounts; such linking information can be collected and used as seed matches.

The seed matches provide valuable information for identifying other matching pairs.  For example, if $i\in V_1$ has a neighbor which is already matched to a neighbor of $j\in V_2$, then $[i,j]$ is more likely to be a valid pair. This simple idea lies at the heart of a popular class of algorithms, namely percolation graph matching.
%a node pair near a seed match has the chance to be a true match; and more potential matches are risen when we consider the newly matched pairs as $seeds$. This greatly simplifies the graph matching problem as the number of candidate matches that should be considered is significantly reduced.


%
\noindent
\textbf{Percolation Graph Matching.} Percolation-based frameworks are widely used for seeded graph matching, referred to as Percolation Graph Matching (PGM)~\cite{narayanan2009anonymizing}. For a pair $[i,j]$, where $i\in V_1,j\in V_2$,  we say $[i',j']$ is its neighboring pair if $(i,i')\in E_1$ and $(j,j')\in E_2$.
% the case has not helped?
So one can imagine there is large graph consists of $|V_1|\cdot|V_2|$ nodes corresponding to all possible pairs; two nodes are adjacent if they are neighboring pairs.
PGM maintains a set of matched pairs which consists of the seed pairs in the beginning, then adds new matches iteratively: (1) in each round, the \emph{unused} matched pairs percolate (spread marks) to neighboring pairs; (2) the pairs that received marks, namely \emph{candidate pairs}, are then examined by certain criteria and matched if they are qualified; (3) the algorithm terminates when all matched pairs have percolated and no further candidate pair qualifies.
Whether to match a pair $[i,j]$ (where $i\in V_1,j\in V_2$), existing PGM algorithms mainly concern the number (denoted as $r$) of its neighboring pairs that have already been matched in previous rounds (which is simply the %number of
marks $[i,j]$ received). If the $r$ is above a given threshold $k$, the pair is added to the matched set~\cite{yartseva2013performance}. When there are multiple qualified candidates, additional rules are used for tie breaking, e.g.,~\cite{korula2014efficient} prefer the nodes of high degrees,~\cite{zhou2016cross} matches the node pairs with the maximal $r$, and~\cite{kazemi2015growing} always selects the node pair with minimal degree difference. 


The performance of the PGM framework is highly sensitive to the size of seed set and the threshold $k$. Insufficient number of seeds often leads to early termination of percolation.
One can reduce the threshold $k$ to make the algorithm percolate easily, but this tends to match wrong pairs.
To prevent early stopping, a new strategy, namely ExpandWhenStuck (EWS), is proposed in~\cite{kazemi2015growing}. When the percolation stops, EWS then collects all candidate pairs, which are pairs that receive at least $1$ mark but haven't meet the matching criteria, to form a \emph{noisy seed set}, and allows this set of pairs to percolate. After this noisy expansion, the algorithm continues the normal PGM process.
The candidate pairs added to noisy seed set once will not be used for percolation again.
This approach effectively prevents early-stop, and EWS significantly outperforms previous PGM algorithms when the number of seeds is very small.

\noindent
\textbf{Limitations of existing PGM algorithms.}
One major limitation of existing PGM algorithms is that they fail to break \emph{Local Symmetry}.
It is easy to check all PGM algorithms mentioned above~\cite{yartseva2013performance, korula2014efficient, zhou2016cross, kazemi2015growing} fail to match the two graphs in Figure~\ref{fig:fig1} with probability $1/2$.
We take EWS~\cite{kazemi2015growing} as an example, which matches node pairs with at least $2$ matched neighboring pairs ($r\ge 2$).
%and utilizes the degree centrality by matching the node pair with minimal degree difference ($||N(i)|-|N(j)||$) first. %, i.e., the pair $[i,j]$ with the minimal $||N(i)|-|N(j)||$.
%In Figure~\ref{fig:fig1}, we are matching two graphs (separated by the dashed line) designed to be isomorphic, thus the ground truth is clear: with seed pairs $[s_1, s_3]$ and $[s_2, s_4]$ provided, $[u_1,v_1]$ and $[u_2,v_2]$ are the correct matches because $\triangle_{u_1i_1i_2}$ and $\triangle_{v_1j_1j_2}$ are aligned, and $\wedge_{i_3u_2i_4}$ and $\wedge_{j_3v_2j_4}$ are aligned.
The EWS algorithm first percolates from two seed pairs and obtains $4$ candidate pairs $[u_1,v_1]$, $[u_1,v_2]$, $[u_2,v_1]$ and $[u_2,v_2]$. Each candidate pair has a score $r=2$ satisfying the matching criteria. Meanwhile, all $4$ candidate pairs have the same degree difference $0$. In this case, the EWS randomly chooses a pair to be matched first, and thus will fail to find the correct hidden matching with probability $1/2$.


Moreover, an early mistake may propagate and lead to cascade of errors.
%Another concern for the PGM algorithms is the cascading mismatching. The percolation mechanism determines the high dependency of matching results, since whether a pair can be correctly matched relies on the matching results of its neighboring pairs directly. Note that the effect of early matches can be regarded as a strong bias on the later matching w.r.t. the effect of initial seed pairs.
In the example of Figure~\ref{fig:fig1}, once EWS matches $[u_1,v_2]$ and $[u_2,v_1]$, the upper left part will more likely be matched to the lower right part. Intuitively, we should postpone this decision making and explore further to seek a symmetry breaker. %but,
%in our example, this leads to early stopping, as no other pair is qualified for percolation.

% The key is, even if the EWS allows repeated percolation whenever symmetry exists, it suffers from the dilemma of 1-order Weisfeiler Lehman coloring, i.e., the similarity is always decided by the first structure difference the percolation meets.

\begin{figure}[!t]
\begin{centering}
\includegraphics [width=3.2in]{fig/fig1.eps}
%\includegraphics[trim=2 0 38 0,clip,width=\figsize]{fig/fig1.eps}
%\label{fig:fig1}
\vspace*{-1mm}
\caption{Graph matching on two isomorphic graphs.}
\label{fig:fig1}
\vspace*{-5mm}
\end{centering}
\end{figure}


%they may argue on the following method. But if we provide the this part, they may ask for a comparison in the experiments

%It is worth mentioning that an additional strategy of postponing the matching of \emph{close adversary pairs}, which has never been proposed though, can help the EWS algorithms match correctly in the case of Figure~\ref{fig:fig1}, i.e., after the first-round percolation, $[u_1,v_1]$ and $[u_1,v_2]$ are two adversary pairs relevant to node $u_1$ with the same scores $r=2$, and the algorithm should postpone the matching of $u_1$ until the tie is broken (in the third-round percolation).
%% corresponding to a weisfeiler-lehman graph labelling method? It does iterative percolation until it firstly finds the asymmetric structure.
%However, this strategy is still sensitive to the structure difference and fails some cases.
%% simple and direct case?
%For example, in Figure~\ref{fig:fig2}, we assume $[u_1,v_1]$ and $[u_2,v_2]$ are two correct matches considering the minimal graph edit distance. But the EWS algorithm with the postponing strategy wrongly matches $[u_1,v_2]$ by the effect of edges $(i_1,i_2)$ and $(j_1,j_2)$. This is because this approach does iterative percolation and is strongly affected by the first asymmetric structure detected. This approach doesn't solve the cascading mismatching either. Moreover, the additional matching criteria leads to a even larger candidate pair set than that of EWS algorithm.% though the latter is already infeasible on large graphs.

\noindent
\textbf{Our approach.}
To resolve this issue, we adopt a different perspective on the percolation process: we model this using \emph{Random Walk}. Let us consider the seed pair $[s_1,s_3]$ in Figure~\ref{fig:fig1}. A one step of percolation in PGM can be modeled as follows. Starting from $s_1$ and $s_3$, we take a $1$-step random walk in $G_1$ and $G_2$ respectively. Let $p_u$ be the probability that the $1$-step random walk reaches $u$, and thus $p_{u_1}=p_{u_2}=p_{v_1}=p_{v_2}=0.5$. To measure the score between a pair $[u,v]$, we use $\frac{\min(p_{u},p_v)}{\max(p_u,p_v)}$. This generates $4$ candidate pairs all with score $1$, which is exactly the same result as a percolation from $[s_1,s_3]$.

By switching to this perspective, we then extend the framework by allowing the random walk to take more steps. This explores higher-order structural information, which is necessary to break local symmetries.
We define the region that can be reached by a $t$-step random walk as the \emph{Order-$t$} information.\footnote{In EWS, when percolation stops, the algorithm will also percolate from candidate pairs with score $1$, which essentially uses order-$2$ information.} In our framework, order-$t$ information is compactly encoded by the probability distribution $p^{(t)}$, where $p^{(t)}_u$ is the probability that the random walk reaches $u$ after $t$ steps. Intuitively, lower-order information is more important in deciding whether to match a pair, and thus will be assigned a higher priority. Therefore, we encode the structural information of a node $u$ (w.r.t. some seed $s$) by $\pi^t(s,u)=\sum_{i=1}^t \beta^t p^{(t)}_u$, where $0< \beta<1$ is some weighing parameter. It can be show that $\pi^{\infty}(s,u)$ is exactly the well-known \emph{Personalized PageRank} (PPR) of $u$ w.r.t. source $s$. To measure the score of a pair $[u,v]$ w.r.t. a seed pair $[s,s']$, we use $\frac{\min(\pi^t(s,u),\pi^t(s',v))}{\max(\pi^t(s,u),\pi^t(s',v))}$, so PGM is a special case ($t=1$) of our framework.
%In this paper, we propose a new graph matching algorithm using the personalized PageRank (PPR), namely personalized PageRank graph matching (PPRGM). The algorithm integrates a PPR based graph labelling approach with the traditional PGM framework, and achieves better effectiveness than existing PGM methods.

\noindent
\textbf{PPRGM framework.}
Here we briefly describe our novel PPRGM framework for seeded graph matching. In each iteration, PPRGM first computes the (truncated) PPR values of each node w.r.t. seeds and matched pairs. The PPR values of each node in $G_{1,2}$ is called the PPR vector, which can be considered as its \emph{numerical features} or \emph{labels}.
%Then the algorithm follows the percolating way to iteratively expand the candidate pair set and do checking. We raise new percolation and local PPR-based labelling strategy, which is more effective than the traditional percolation method.
We then carefully design a score function based on two PPR vectors to measure the matching score of each pair. It is inefficient to compute the scores of all $|V_1|\cdot|V_2|$ pairs, so we will only consider a set of candidate pairs which are generated in a similar way as in PGM. The algorithm then matches candidate pairs with high scores and goes to the next iteration.
%which measures both the similarity of their global labels (the PPR vectors assigned by the seeds), and the similarity of their local labels (obtained from the early matches). The measurement of two kinds of similarities are aligned by the same formulation.
%Besides, several reasonable rules are made to match the pairs of high credibility first, the effectiveness of which is further analysed in a random graph model.

%Given a set of seeds, we take each seed node as the source node and conduct a personalized PageRank approximation with a fixed stopping probability of random walk. For each node in the graph, its PPR values w.r.t. all seed nodes make up a PPR vector, corresponding to the seed sequence.
%Note that the PPR-based labelling is introduced in seeded graph matching for the first time. It will be shown in Section~\ref{3PPR} that the PPR vector of each node illustrates both its region information and its local structure information. It is worth mentioning that, on a pair of isomorphic graphs, any two nodes corresponding to a true match always have the identical PPR vectors.

\noindent
\textbf{Advantages of PPRGM framework.}
% should merge two paragraphs
%The existing PGM algorithms' incapability of dealing with various complex graph matching cases mainly results from the lack of using the higher-order structure information.
%Nevertheless, the existing PGM framework cannot be easily extended to use the higher-order structure information in matching. Firstly, there is no trivial way to measure the structure difference from the 1-hop neighbors to the distant structures by percolation. Another concern is the high computational cost resulting from the higher-order structure comparison for each potential match, aggravated by the increasing number of candidate pairs that should be considered.
 %the dramatically increased size of candidate pair set, aggravated by the  for each candidate pair.
%The state-of-the-art EWS algorithm~\cite{kazemi2015growing} actually exploits the higher-order information in a lazy way by using the noisy seed set: for the candidate pairs unqualified for a match ($r<2$), the algorithm iteratively adds $1$ mark to all neighboring pairs of noisy seed pairs, thus the candidate pairs with the similar \emph{dense} local structure are matched first. However, its ability of using higher-order structure information is sensitive to the value of $r$ (the number of matched neighboring pairs for each candidate pair): with a small $r$ (like $r=2$ or $r=1$), the node pairs satisfies the criteria easily, EWS seldom considers the higher-order structure and easily matches wrong pairs; and with a large $r$ (like $r=5$), EWS often produces a large candidate set with high time complexity and large space usage, but leads to a small recall. Besides, the way of EWS's comparing structure difference (pass $1$ mark always) is too sensitive to the structure difference.
% higher-order structure information; labelling from the seeds thus less dependency; robustness to the wrong seeds; find the high quality matches first;
By exploring the higher-order structural information, PPRGM can easily break local symmetries, which leads to significant increase in matching precision.
%As shown above, there are situations where the 1-hop structure often fails in distinguishing the nodes' difference, while can be solved with the structure information of a larger range.
%It will be shown that the PPR value embodies the local higher-order structure information of each node in a way.
In Figure~\ref{fig:fig1}, a random walk that starts from $s_1$ and $s_3$ will automatically detect the edge $(i_1,i_2)$ and $(j_1,j_2)$ in $3$ steps, and this information will be incorporated into the PPR values of $u_1$ and $v_1$.
%assume the stopping probability of random walk is $\frac{1}{2}$, then $\pi(s_1, u_2)$, the PPR value of $u_2$ w.r.t. source node $s_1$, is smaller than $\pi(s_3, v_1)$, the PPR value of $v_1$ w.r.t. source node $s_3$; while $\pi(s_1, u_1)=\pi(s_3, v_1)$.
%then $u_1$ and $v_1$ have the same PPR values w.r.t. two seed pairs, while the PPR value of $u_2$ w.r.t. source node $s_1$ ($s_2$) is smaller than the PPR value of $v_1$ w.r.t. source node $s_3$ ($s_4$),
Thus the algorithm matches the pair $[u_1, v_1]$ who have closer PPR values rather than $[u_2,v_1]$. In our experimental studies, PPRGM demonstrates significant improvements in both precision and recall. One interesting phenomenon in our experiments is that, when the two graphs are indeed isomorphic, the precision of PPRGM is always $1$, while the recall is very close to $1$; the nodes left unmatched are mostly symmetric nodes, e.g. $i_1$ and $i_2$ in Figure~\ref{fig:fig1}. However, under the same setting, the precision is much lower on the EWS algorithm.

%Note that the PPR vector of global labelling provides an unbiased guidance in marking a node pair, because its computation is independent from the matching process. Though our algorithm introduces the bias on the early matched node pairs during the percolation (similar to the PGM algorithms), such a bias doesn't dominate the examination of a node pair. That is to say, in PPRGM, whether a pair can be correctly matched relies on both the PPR labels from the seeds and the matching result of the early matches. As a result, the cascading mismatching is relieved.
When the number of seeds is very small, PPRGM needs not to do a noisy expansion as in EWS. In our experiments, $4$-$8$ seeds is often sufficient to achieve high precision and recall. Moreover, PPRGM uses all matched pairs as evidence to decide whether to match a new pair, which is highly robust against early wrong matches. This is particularly important when the initial seed pairs provided may contain lots of incorrect matches.
%All existing PGM algorithms are based on local iterative percolation and are lack of the ability of dealing with wrong seeds.
%However, our PPRGM framework has strong robustness against the wrong seeds.
%This is because the personalized PageRank vector globally demonstrates the region information of a node. Moreover, each correct match is aligned by all correct seeds; while the wrong seeds describe the region similarity of a random node pair in the wrong but different ways, thus a wrong match of nodes from different regions can be supported by few wrong seeds.
It is observed in our experiments, %with an enough number of correct seeds provided,
even when the fraction of incorrect seeds is up to $0.8$, the performance of PPRGM declines only slightly in most cases.


One might suspect the time complexity of PPRGM is higher than PGM algorithms, as we need to compute PPR values from unused matched pairs in each iteration. However, PPRGM makes more progress in each iteration, and thus the total number of iterations is smaller, which compensates the higher cost in each iteration.
A significant evidence is the PPRGM considers much fewer candidate pairs than EWS.

In general, the time consumption of PPRGM is more than an order of magnitude lower than EWS in our experiments.
%The proposed PPRGM achieves its efficiency by embedding each node's higher-order structure information into its PPR labels, and evaluating a node pair based on the labels of each node. While the traditional pair-based percolation method may incur an extremely large candidate set with high computational cost.

%Last but not least, PPRGM tends to output the matches of high credibility first, benefiting from the global PPR-based labelling. Such a property is favored by applications in the real world. For example, in online advertising, the budget is considered and the model targets at a portion of matching results of high quality to maximize the profit.

\noindent
\textbf{Contributions.} We summarize our contributions as follows. (1) We propose to use PPR values as a graph labeling method to solve the seeded graph matching problem, and further propose a scoring function based on the PPR-labeling to effectively determine whether to match a pair.
%represents the region information and local structure information of nodes, and a corresponding score function on two PPR vectors is defined.
(2) We propose a powerful graph matching framework PPRGM, by integrating a PPR based graph labeling method with the traditional percolation framework, which improves the matching precision significantly even using a small number of seed pairs. The new approach is also scalable and strongly robust against incorrect seed pairs. (3) We conduct extensive experiments on various large-scale real-world graphs, which demonstrates that our new algorithm outperforms the start-of-the-art PGM algorithm w.r.t. accuracy, robustness and efficiency.

\noindent
\textbf{Outline.} Section \uppercase\expandafter{\romannumeral2} introduces notations and the related work. %Section \uppercase\expandafter{\romannumeral3} introduces personalized PageRank in graph labelling.
Section \uppercase\expandafter{\romannumeral3} proposes our PPRGM framework with unmatched advantages over the start-of-the-art, and effective strategies for improving matching precision. Section \uppercase\expandafter{\romannumeral4} evaluates all introduced algorithms using extensive experiments. Finally we conclude the paper in Section \uppercase\expandafter{\romannumeral5}.

% Time complexity analysis:
%Besides, as PPRGM efficiently encodes the higher-order information of nodes (in each graph) and then compares the nodes across the graphs, the overall time complexity of Forward-Push is $O(|V_1||E_1|+|V_2||E_2|)$ in the worst case (or $c(|E_1|+|E_2|)$ for a const $c$ in practice), which overwhelms the $|E_1||E_2|$, the worst-case time complexity of Percolation in EWS.

\noindent
\textbf{Time complexity analysis.}
In the following time analysis, we assume both graphs in matching contain $O(|V|)$ nodes and $O(|E|)$ edges for simplicity.
Our algorithm mainly conducts two jobs: Forward-Push and pair measurement.
The Forward-Push method is presented in Algorithm~\ref{alg:FP}, with $r_{max}$ determining the termination of pushing forward.
~\cite{andersen2006local} proves a Forward-Push process takes $O(1/r_{max})$ time. In our algorithm, only the seeds and the matched nodes start the Forward-Push. Assume $r_{max}$ and $r'_{max}$ are the parameters used for Forward-Push on initial seeds and matched nodes respectively, then all Forward-Push processes take totally $O(\frac{|S|}{r_{max}}+\frac{|V|}{r'_{max}})$ time\footnote{ If each matched node is only allowed to percolate its neighbors, then all Forward-Push processes take $O(\frac{|S|}{r_{max}}+|E|)$ time.}.
Then we consider the pair measurement cost.
Note that $O(\frac{1}{r_{max}})$ nodes obtain PPR values in a Forward-Push process with parameter $r_{max}$. Thus each node receives on average $O(\frac{|S|}{r_{max}|V|}+\frac{1}{r'_{max}})$ labels in total. Given a pair $[i,j]$ where node $i$ has $m$ labels and node $j$ has $n$ labels, the time complexity of measuring $[i,j]$ is $\min\{m,n\}$.
Denote $C$ the set of candidate pairs that are considered by our algorithm. Then a node on average is measured with $\frac{|C|}{|V|}$ nodes from the aligned graph.
Thus, the pair measurement across two graphs takes $O(\frac{|S|\cdot |C|}{r_{max}|V|}+\frac{|C|}{r'_{max}})$ time.
We also claim $|C|$ is bounded by $O(\frac{|V|}{r'^2_{max}})$, because the number of matched pairs is bounded by $O(|V|)$ and the Forward-Push from a matched pair $[i,j]$ leads to $O(\frac{1}{r'^2_{max}})$ candidate pairs (the Cartesian product of two sets of nodes that are labelled by $i$ and $j$ respectively)
\footnote{The candidate pairs sets produced by different matched pairs are actually greatly overlapped, thus in practice the total number of candidate pairs is much smaller than $\frac{|V_1|}{r'^2_{max}}$. The measurement of the number of candidate pairs will be presented in the experiment section.}.
In conclusion, the overall time complexity of our algorithm is approximately $O(\frac{|S|}{r_{max}} + \frac{|V|}{r'_{max}} + \frac{|S|}{r_{max}r'^2_{max}} + \frac{|V|}{r'^3_{max}})=O(\frac{|S|}{r_{max}r'^2_{max}} + \frac{|V|}{r'^3_{max}})$ (dominated by the cost of pair measurement).

We then provide the time analysis of EWS algorithm.
Denote $C'$ the set of candidate pairs that are considered by EWS algorithm. Because EWS measures a candidate pair simply by its mark, the overall time of pair measurement is $O(|C'|)$. Because each candidate pair $[i,j]$ receives at most $|N(i)||N(j)|$ marks, the total number of percolation is bounded by $O(\frac{|C'||E|^2}{|V|^2})$. We then bound $|C'|$.
Denote $|E^{(2)}|$ the number of non-zero entries in the matrix $A^2$, where $A$ is the adjacency matrix representing graph $G$. Then each node on average has $\frac{|E^{(2)}|}{|V|}$ $2$-hop neighbors.
Thus, each matched pair produces $O(\frac{|E^{(2)}|^2}{|V|^2} + \frac{|E|^2}{|V|^2})$ candidate pairs. Because there are at most $|V|$ matched pairs, $|C'|$ is bounded by $O(\frac{|E^{(2)}|^2+|E|^2}{|V|})$.
In conclusion, the time complexity of EWS algorithm is approximately $O(\frac{|E^{(2)}|^2|E|^2+|E|^4}{|V|^3})$ (dominated by the cost of percolation).


==> Table_with_0.8_0.8.tex <==

\begin{table*}[!tb]
  \centering
  %\footnotesize
  \small
  \caption{\bf{Precision and Recall on Datasets}}
  \label{table:pr_results1}
  \renewcommand{\arraystretch}{1}
  \resizebox{\columnwidth*2+0.3in}{!}{%
  \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
    \noalign{\hrule height 1pt}
    % dataset % method % 1 p % 1r % 2p % 2r % 3p % 3r
    \multirow{2}{*}{Datasets} & \multirow{2}{*}{Alg.} &
        \multicolumn{3}{c|}{$p_n$=$1.0$, $p_e$=$1.0$} & \multicolumn{3}{c|}{$p_n$=$1.0$, $p_e$=$0.9$} & \multicolumn{3}{c|}{$p_n$=$1.0$, $p_e$=$0.8$} &
        \multicolumn{3}{c|}{$p_n$=$0.9$, $p_e$=$0.9$} & \multicolumn{3}{c|}{$p_n$=$0.9$, $p_e$=$0.8$} & \multicolumn{3}{c|}{$p_n$=$0.8$, $p_e$=$0.9$} &
        \multicolumn{3}{c}{$p_n$=$0.8$, $p_e$=$0.8$} \\
        \cline{3-23}
        & & \Recall & \Precison & \FSCORE & \Recall & \Precison & \FSCORE & \Recall & \Precison & \FSCORE & \Recall & \Precison & \FSCORE & \Recall & \Precison & \FSCORE & \Recall & \Precison & \FSCORE & \Recall & \Precison & \FSCORE\\
    \hline
    \hline
    \multirow{6}{*}{\textbf{Twitter}}
        & HOE & \textbf{0.980} & \textbf{1.000} & \textbf{0.990} & \textbf{0.931} & 0.962 & \textbf{0.946} & \textbf{0.854} & 0.889 & \textbf{0.871} & \textbf{0.870} & 0.842 & \textbf{0.856} & \textbf{0.762} & 0.745 & \textbf{0.753} & \textbf{0.799} & 0.716 & \textbf{0.755} & \textbf{0.673} & 0.604 & 0.637  \\
        & NE & 0.965 & \textbf{1.000} & 0.982 & 0.906 & \textbf{0.965} & 0.935 & 0.823 & \textbf{0.896} & 0.858 & 0.840 & \textbf{0.853} & 0.846 & 0.733 & \textbf{0.766} & 0.749 & 0.766 & \textbf{0.736} & 0.751 & 0.644 & \textbf{0.636} & \textbf{0.640} \\
        & EWS & 0.966 & 0.968 & 0.967 & 0.900 & 0.912 & 0.906 & 0.763 & 0.793 & 0.778 & 0.815 & 0.772 & 0.793 & 0.526 & 0.539 & 0.532 & 0.630 & 0.568 & 0.598 & 0.390 & 0.372 & 0.381 \\
        & GSANA & 0.901 & 0.915 & 0.908 & 0.144 & 0.271 & 0.188 & 0.118 & 0.236 & 0.157 & 0.118 & 0.223 & 0.154 & 0.096 & 0.207 & 0.131 & 0.109 & 0.187 & 0.138 & 0.092 & 0.182 & 0.122  \\
        & AE & 0.911 & 0.912 & 0.912 & 0.338 & 0.352 & 0.345 & 0.145 & 0.157 & 0.150 & 0.123 & 0.122 & 0.123 & 0.057 & 0.058 & 0.058 & 0.052 & 0.048 & 0.050 & 0.033 & 0.030 & 0.032 \\
        & FRUI & 0.873 & 0.890 & 0.882 & 0.276 & 0.323 & 0.298 & 0.306 & 0.340 & 0.322 & 0.354 & 0.361 & 0.358 & 0.032 & 0.036 & 0.034 & 0.133 & 0.128 & 0.130 & 0.002 & 0.002 & 0.002  \\
    \hline
    \multirow{6}{*}{\textbf{Dblp}}
        & HOE & \textbf{0.970} & \textbf{1.000} & \textbf{0.985} & \textbf{0.652} & 0.712 & \textbf{0.681} & \textbf{0.535} & 0.596 & \textbf{0.564} & \textbf{0.542} & 0.585 & \textbf{0.563} & \textbf{0.422} & 0.463 & \textbf{0.441} & \textbf{0.413} & 0.432 & \textbf{0.422} & \textbf{0.202} & 0.227 & \textbf{0.214} \\
        & NE & 0.767 & \textbf{1.000} & 0.868 & 0.482 & \textbf{0.737} & 0.583 & 0.371 & \textbf{0.635} & 0.468 & 0.382 & \textbf{0.628} & 0.475 & 0.278 & \textbf{0.501} & 0.357 & 0.274 & \textbf{0.491} & 0.352 & 0.160 & \textbf{0.302} & 0.209  \\
        & EWS & 0.618 & 0.679 & 0.648 & 0.491 & 0.589 & 0.536 & 0.358 & 0.478 & 0.410 & 0.390 & 0.476 & 0.429 & 0.264 & 0.355 & 0.303 & 0.279 & 0.337 & 0.305 & 0.118 & 0.159 & 0.136  \\
        & GSANA & 0.875 & 0.934 & 0.903 & 0.018 & 0.166 & 0.032 & 0.010 & 0.128 & 0.019 & 0.010 & 0.115 & 0.018 & 0.009 & 0.111 & 0.016 & 0.007 & 0.098 & 0.014 & 0.008 & 0.098 & 0.014  \\
        & AE & 0.749 & 0.750 & 0.749 & 0.303 & 0.358 & 0.329 & 0.095 & 0.128 & 0.109 & 0.102 & 0.128 & 0.114 & 0.032 & 0.043 & 0.037 & 0.031 & 0.037 & 0.034 & 0.012 & 0.015 & 0.013  \\
        & FRUI & 0.234 & 0.349 & 0.281 & 0.001 & 0.001 & 0.001 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000  \\
    \hline
    \multirow{6}{*}{\textbf{Amazon}}
        & HOE & \textbf{0.981} & \textbf{1.000} & \textbf{0.990} & \textbf{0.716} & \textbf{0.755} & \textbf{0.735} & \textbf{0.508} & \textbf{0.556} & \textbf{0.531} & \textbf{0.538} & \textbf{0.569} & \textbf{0.553} & \textbf{0.348} & \textbf{0.392} & \textbf{0.369} & \textbf{0.334} & \textbf{0.373} & \textbf{0.353} & \textbf{0.122} & \textbf{0.170} & \textbf{0.142}  \\
        & NE & 0.785 & \textbf{1.000} & 0.880 & 0.454 & 0.754 & 0.567 & 0.130 & 0.328 & 0.186 & 0.106 & 0.289 & 0.155 & 0.013 & 0.044 & 0.019 & 0.008 & 0.029 & 0.013 & 0.001 & 0.004 & 0.002  \\
        & EWS & 0.671 & 0.774 & 0.719 & 0.401 & 0.571 & 0.471 & 0.071 & 0.160 & 0.098 & 0.075 & 0.157 & 0.101 & 0.003 & 0.009 & 0.005 & 0.002 & 0.006 & 0.003 & 0.001 & 0.003 & 0.002  \\
        & GSANA & 0.958 & 0.973 & 0.966 & 0.010 & 0.206 & 0.020 & 0.006 & 0.183 & 0.011 & 0.006 & 0.176 & 0.011 & 0.005 & 0.162 & 0.009 & 0.004 & 0.157 & 0.008 & 0.004 & 0.158 & 0.007 \\
        & AE & 0.898 & 0.899 & 0.898 & 0.353 & 0.409 & 0.379 & 0.075 & 0.106 & 0.088 & 0.075 & 0.099 & 0.085 & 0.016 & 0.024 & 0.019 & 0.014 & 0.019 & 0.016 & 0.003 & 0.005 & 0.004  \\
        & FRUI & 0.141 & 0.212 & 0.169 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline
    \multirow{3}{*}{\textbf{Youtube}}
        & HOE & \textbf{0.908} & \textbf{1.000} & \textbf{0.952} & \textbf{0.811} & 0.937 & \textbf{0.869} & \textbf{0.714} & 0.866 & \textbf{0.783} & \textbf{0.730} & 0.833 & \textbf{0.778} & \textbf{0.643} & 0.751 & \textbf{0.693} & \textbf{0.652} & 0.721 & \textbf{0.685} & \textbf{0.559} & 0.634 & \textbf{0.594}  \\
        & NE & 0.868 & \textbf{1.000} & 0.929 & 0.750 & \textbf{0.963} & 0.843 & 0.629 & \textbf{0.938} & 0.753 & 0.660 & \textbf{0.899} & 0.761 & 0.563 & \textbf{0.855} & 0.679 & 0.574 & \textbf{0.832} & 0.679 & 0.478 & \textbf{0.783} & \textbf{0.594}  \\
       % & AE & &   &   &   &   &   &   &   &   &   &   & \\
        & FRUI & 0.266 & 0.441 & 0.332 & 0.101 & 0.189 & 0.132 & 0.000 & 0.000 & 0.000 & 0.040 & 0.068 & 0.050 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline
    \multirow{3}{*}{\textbf{WikiTalk}}
        & HOE & \textbf{0.773} & \textbf{1.000} & \textbf{0.872} & 0.730 & 0.968 & 0.832 & \textbf{0.682} & 0.917 & 0.782 & \textbf{0.703} & 0.899 & 0.789 & \textbf{0.650} & 0.870 & \textbf{0.744} & \textbf{0.658} & 0.845 & 0.740 & \textbf{0.604} & 0.775 & 0.679  \\
        & NE & 0.772 & \textbf{1.000} & 0.872 & \textbf{0.732} & \textbf{0.975} & \textbf{0.836} & 0.680 & \textbf{0.937} & \textbf{0.788} & 0.702 & \textbf{0.920} & \textbf{0.796} & 0.641 & \textbf{0.876} & 0.740 & 0.657 & \textbf{0.860} & \textbf{0.745} & 0.596 & \textbf{0.800} & \textbf{0.683}  \\
        & FRUI & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000  \\
    \noalign{\hrule height 1pt}
  \end{tabular}
  }
\end{table*}
\vspace{0.1cm}


==> Table_without_F1-score.tex <==
\begin{table*}[!tb]
  \centering
  %\footnotesize
  \small
  \caption{\bf{Precision and Recall on Datasets}}
  \label{table:pr_results1}
  \renewcommand{\arraystretch}{1}
  \resizebox{\columnwidth*2+0.3in}{!}{%
  \begin{tabular}{l|c|cc|cc|cc|cc|cc|cc|cc}
    \noalign{\hrule height 1pt}
    % dataset % method % 1 p % 1r % 2p % 2r % 3p % 3r
    \multirow{2}{*}{Datasets} & \multirow{2}{*}{Alg.} &
        \multicolumn{2}{c|}{$p_n$=$1.0$, $p_e$=$1.0$} & \multicolumn{2}{c|}{$p_n$=$1.0$, $p_e$=$0.9$} & \multicolumn{2}{c|}{$p_n$=$1.0$, $p_e$=$0.8$} &
        \multicolumn{2}{c|}{$p_n$=$0.9$, $p_e$=$0.9$} & \multicolumn{2}{c|}{$p_n$=$0.9$, $p_e$=$0.8$} & \multicolumn{2}{c|}{$p_n$=$0.8$, $p_e$=$0.9$} &
        \multicolumn{2}{c}{$p_n$=$0.8$, $p_e$=$0.8$} \\
        \cline{3-16}
        & & \Recall & \Precison & \Recall & \Precison & \Recall & \Precison & \Recall & \Precison & \Recall & \Precison & \Recall & \Precison & \Recall & \Precison  \\
    \hline
    \hline
    %\multirow{6}{*}{\textbf{Epinions}}
%        & HOE   & 0.948 & \textbf{1.000} & \textbf{0.890} & 0.956 & \textbf{0.838} & 0.903 & \textbf{0.844} & 0.863 & \textbf{0.791} & 0.804 & \textbf{0.791} & 0.776 & \textbf{0.736} & 0.706 \\
%        & NE   & 0.923 & \textbf{1.000} & 0.862 & \textbf{0.970} & 0.804 & \textbf{0.931} & 0.807 & \textbf{0.890} & 0.747 & \textbf{0.850} & 0.737 & \textbf{0.838} & 0.685 & \textbf{0.765}  \\
%        & EWS   & 0.635 & 0.968 & 0.630 & 0.949 & 0.614 & 0.926 & 0.590 & 0.876 & 0.533 & 0.808 & 0.530 & 0.759 & 0.419 & 0.625  \\
%        & GSANA & 0.766 & 0.837 & 0.113 & 0.249 & 0.079 & 0.199 & 0.216 & 0.303 & 0.110 & 0.204 & 0.090 & 0.156 & 0.073 & 0.163  \\
%        & AE   & 0.846 & 0.892 & 0.723 & 0.774 & 0.330 & 0.381 & 0.324 & 0.342 & 0.168 & 0.177 & 0.196 & 0.184 & 0.005 & 0.004  \\
%        & FRUI  & \textbf{0.958} & 0.959 & 0.341 & 0.374 & 0.123 & 0.139 & 0.114 & 0.118 & 0.055 & 0.056 & 0.045 & 0.041 & 0.031 & 0.028  \\
%    \hline
    \multirow{6}{*}{\textbf{Twitter}}
        & HOE & \textbf{0.980} & \textbf{1.000} & \textbf{0.931} & 0.962 & \textbf{0.854} & 0.889 & \textbf{0.870} & 0.842 & \textbf{0.762} & 0.745 & \textbf{0.799} & 0.716 & \textbf{0.673} & \textbf{0.604} \\
        & NE & 0.965 & \textbf{1.000} & 0.906 & \textbf{0.965} & 0.823 & \textbf{0.896} & 0.840 & \textbf{0.853} & 0.733 & \textbf{0.766} & 0.766 & \textbf{0.736} & 0.644 & 0.636 \\
        & EWS & 0.966 & 0.968 & 0.900 & 0.912 & 0.763 & 0.793 & 0.815 & 0.772 & 0.526 & 0.539 & 0.630 & 0.568 & 0.390 & 0.372 \\
        & GSANA & 0.901 & 0.915 & 0.144 & 0.271 & 0.118 & 0.236 & 0.118 & 0.223 & 0.096 & 0.207 & 0.109 & 0.187 & 0.092 & 0.182 \\
        & AE & 0.911 & 0.912 & 0.338 & 0.352 & 0.145 & 0.157 & 0.123 & 0.122 & 0.057 & 0.058 & 0.052 & 0.048 & 0.033 & 0.030 \\
        & FRUI & 0.873 & 0.890 & 0.276 & 0.323 & 0.306 & 0.340 & 0.354 & 0.361 & 0.032 & 0.036 & 0.133 & 0.128 & 0.002 & 0.002 \\
    \hline
    \multirow{6}{*}{\textbf{Dblp}}
        & HOE & \textbf{0.970} & \textbf{1.000} & \textbf{0.652} & 0.712 & \textbf{0.535} & 0.596 & \textbf{0.542} & 0.585 & \textbf{0.422} & 0.463 & \textbf{0.413} & 0.432 & \textbf{0.202} & 0.227 \\
        & NE & 0.767 & \textbf{1.000} & 0.482 & \textbf{0.737} & 0.371 & \textbf{0.635} & 0.382 & \textbf{0.628} & 0.278 & \textbf{0.501} & 0.274 & \textbf{0.491} & 0.160 & \textbf{0.302} \\
        & EWS & 0.618 & 0.679 & 0.491 & 0.589 & 0.358 & 0.478 & 0.390 & 0.476 & 0.264 & 0.355 & 0.279 & 0.337 & 0.118 & 0.159 \\
        & GSANA & 0.875 & 0.934 & 0.018 & 0.166 & 0.010 & 0.128 & 0.010 & 0.115 & 0.009 & 0.111 & 0.007 & 0.098 & 0.008 & 0.098 \\
        & AE & 0.749 & 0.750 & 0.303 & 0.358 & 0.095 & 0.128 & 0.102 & 0.128 & 0.032 & 0.043 & 0.031 & 0.037 & 0.012 & 0.015 \\
        & FRUI & 0.234 & 0.349 & 0.001 & 0.001 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline
    \multirow{6}{*}{\textbf{Amazon}}
        & HOE & \textbf{0.981} & \textbf{1.000} & \textbf{0.716} & \textbf{0.755} & \textbf{0.508} & \textbf{0.556} & \textbf{0.538} & \textbf{0.569} & \textbf{0.348} & \textbf{0.392} & \textbf{0.334} & \textbf{0.373} & \textbf{0.122} & \textbf{0.170} \\
        & NE & 0.785 & \textbf{1.000} & 0.454 & 0.754 & 0.130 & 0.328 & 0.106 & 0.289 & 0.013 & 0.044 & 0.008 & 0.029 & 0.001 & 0.004 \\
        & EWS & 0.671 & 0.774 & 0.401 & 0.571 & 0.071 & 0.160 & 0.075 & 0.157 & 0.003 & 0.009 & 0.002 & 0.006 & 0.001 & 0.003 \\
        & GSANA & 0.958 & 0.973 & 0.010 & 0.206 & 0.006 & 0.183 & 0.006 & 0.176 & 0.005 & 0.162 & 0.004 & 0.157 & 0.004 & 0.158 \\
        & AE & 0.898 & 0.899 & 0.353 & 0.409 & 0.075 & 0.106 & 0.075 & 0.099 & 0.016 & 0.024 & 0.014 & 0.019 & 0.003 & 0.005 \\
        & FRUI & 0.141 & 0.212 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline
    \multirow{3}{*}{\textbf{Youtube}}
        & HOE & \textbf{0.908} & \textbf{1.000} & \textbf{0.811} & 0.937 & \textbf{0.714} & 0.866 & \textbf{0.732} & 0.833 & \textbf{0.643} & 0.751 & \textbf{0.652} & 0.721 & \textbf{0.559} & 0.634 \\
        & NE & 0.868 & \textbf{1.000} & 0.750 & \textbf{0.963} & 0.629 & \textbf{0.938} & 0.662 & \textbf{0.899} & 0.564 & \textbf{0.855} & 0.574 & \textbf{0.832} & 0.478 & \textbf{0.783} \\
       % & AE & &   &   &   &   &   &   &   &   &   &   & \\
        & FRUI & 0.266 & 0.441 & 0.101 & 0.189 & 0.000 & 0.000 & 0.040 & 0.068 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \hline
    \multirow{3}{*}{\textbf{WikiTalk}}
        & HOE & \textbf{0.773} & \textbf{1.000} & \textbf{0.730} & 0.968 & \textbf{0.682} & 0.917 & \textbf{0.703} & 0.899 & \textbf{0.650} & 0.870 & \textbf{0.658} & 0.845 & \textbf{0.604} & 0.775 \\
        & NE & 0.772 & \textbf{1.000} & \textbf{0.730} & \textbf{0.976} & 0.680 & \textbf{0.937} & 0.702 & \textbf{0.920} & 0.641 & \textbf{0.876} & 0.657 & \textbf{0.860} & 0.596 & \textbf{0.800} \\
        & FRUI & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    \noalign{\hrule height 1pt}
  \end{tabular}
  }
\end{table*}
\vspace{0.1cm}





\begin{table}[!tb]
\small
\begin{center}
\vspace*{-2mm}\caption{\label{table:pr_results2}\bf{Precision and Recall on Datasets}}
\renewcommand{\arraystretch}{1}
\resizebox{\columnwidth-0.2in}{!}{%
\begin{tabular}{c|cc|cc|cc}
    \noalign{\hrule height 1pt}
    \multirow{2}{*}{Alg.} & \multicolumn{2}{c|}{P0 vs. P1} & \multicolumn{2}{c|}{P0 vs. P2} & \multicolumn{2}{c}{P0 vs. P3} \\
    \cline{2-7}
    & \Recall & \Precison & \Recall & \Precison & \Recall & \Precison  \\
    \hline
    \hline
    \multicolumn{6}{l}{\textbf{Superuser}}\\
    \hline
    HOE & \textbf{0.863} & 0.966 & \textbf{0.820} & 0.911 & \textbf{0.776} & 0.847 \\
    NE & 0.855 & \textbf{0.982} & 0.809 & \textbf{0.952} & 0.766 & \textbf{0.912} \\
    EWS & 0.609 & 0.673 & 0.452 & 0.570 & 0.353 & 0.466 \\
    GSANA & 0.277 & 0.518 & 0.105 & 0.278 & 0.084 & 0.221 \\
    AE & 0.084 & 0.097 & 0.013 & 0.014 & 0.008 & 0.008 \\
    FRUI & 0.345 & 0.531 & 0.226 & 0.350 & 0.141 & 0.228 \\
    \hline
    \multicolumn{6}{l}{\textbf{AskUbuntu}}\\
    \hline
    HOE & \textbf{0.842} & 0.950 & \textbf{0.768} & 0.865 & \textbf{0.678} & 0.771 \\
    NE & 0.820 & \textbf{0.977} & 0.737 & \textbf{0.932} & 0.636 & \textbf{0.888} \\
    EWS & 0.574 & 0.643 & 0.414 & 0.527 & 0.139 & 0.227 \\
    GSANA & 0.115 & 0.331 & 0.073 & 0.222 & 0.054 & 0.186 \\
    AE & 0.103 & 0.115 & 0.014 & 0.015 & 0.005 & 0.005 \\
    FRUI & 0.523 & 0.635 & 0.081 & 0.147 & 0.042 & 0.070 \\
    \noalign{\hrule height  1pt}
\end{tabular}
}
\vspace*{-6mm}
\end{center}
\end{table}

==> delete_part.tex <==

%We will show that (1) In two isomorphic network graphs with all seed matches correct, the exact PPR vectors of two aligned nodes are identical, and two aligned nodes should be correctly matched .
%(2) The PPR vector of each node represents its region information and local structure information.
%(3) The graph labeling based on PPR vector has unmatched advantages over the traditional weisfeiler-lehman graph labeling method on graph matching problem.
%(4) PPRGM is relevant to but more efficient and more flexible than the IsoRank algorithm~\cite{singh2008global}, which is designed for the non-seed network alignment.
%XXX(3) PPRGM does not expand the seed set, which reduces the bias in judging the potential matches, thus PPRGM has the stable performance in the complicated phenomena.
% still not sure if we are going to expand the seed set. Intuitively it should be better. Trust the high score match. But no obvious better result yet.
%(5) Each wrong match in the initial seed set has limited affect on the performance of PPRGM. NEED Experiments?

\begin{lemma}~\label{isomophic}
Given two isomorphic network graphs with all seed matches correct, the exact PPR vectors of two aligned nodes are identical.
\end{lemma}
%\begin{proof}
%Assume $V_1$ and $V_2$ are ordered in the same way as $S_1$ and $S_2$ respectively s.t. each pair of nodes at the same position in two sequences are aligned. Then the adjacency matrix $A_1$ on $G_1$ with respect to $S_1$ and $A_2$ on $G_2$ with respect to $S_2$ are identical, i.e., $A_1=A_2$ and also $P_1= P_2$. Then $e_{s^1_k}=e_{s^2_k}$ since $[s^1_k, s^2_k]$ is a correct match, and thus $\pi(s^1_k, i) = \pi(s^2_k, i)$ based on Equation~(\ref{PPR-math}).
%Given all correct seed matches, we have $R^1(i)=R^2(j)$ for the aligned pair $[i,j]$.
%\end{proof}

explain detailed LS
%we define a transition matrix $\bar{P}$ on $G$ that does not stop by node $i$ by
%\[
%    \bar{P}_{ji'}=
%\begin{cases}
%    0 & \text{if } i' = i,\\
%    P_{ji'}  & \text{otherwise.}
%\end{cases}
%\]
%The probability of the random walk from $s_k$ arriving at node $i$ for the first time at step $t$ is
%\begin{equation}\label{R1-math}
%    rf_{i}^{(t)} =
%\begin{cases}
%    [(1-\alpha)^{t} \cdot \bar{P}^{t-1} \cdot P \cdot e_{s_k}]_i & \text{if } t>0,\\
%    [e_{s_k}]_i  & \text{t=0.}
%\end{cases}
%\end{equation}
%Thus we have
%\begin{equation}\label{PPR1-math}
%\pi_1(s_k, i) = \alpha\cdot\sum_{t=0}^{\infty}rf^{(t)}_{i}. %= [(I_{|V|} + \sum_{t=1}^{\infty}(1-\alpha)^{t} \cdot \bar{P}^{t-1} \cdot P) \cdot (\alpha e_{s_k})]_i.
%\end{equation}
%
%Following the definition of $rf_{i}^{(t)}$, the probability of a random walk, that arrives at $i$ for the first time at the $t^{th}$ iteration, arriving at node $i$ afterwards is defined by
%\begin{equation}\label{R2-math}
%    rl_{i}^{(t)} = rf_{i}^{(t)}\cdot [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i
%\end{equation}
%where $e_i \in \real^{|V|\times1}$ has $1$ at the $i^{th}$ position and $0$s at all other positions. Then we have
%\begin{equation}\label{PPR2-math}
%\begin{split}
%\pi_2(s_k, i) & = \alpha\cdot\sum_{t=0}^{\infty}rl_{i}^{(t)} = \alpha\cdot\sum_{t=0}^{\infty}(rf_{i}^{(t)}\cdot [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i) \\
%            & = (\alpha\cdot\sum_{t=0}^{\infty}rf_{i}^{(t)})\cdot [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i \\
%            & = \pi_1(s_k, i)\cdot [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i.
%\end{split}
%\end{equation}
%Let $LS(i) = [\sum_{q=1}^{\infty}(1-\alpha)^{q}\cdot P^{q}\cdot e_i]_i$. Note that $LS(i)$ is independent of the source node $s_k$, but only depends on node $i$ and graph $G$.
%Thus the PPR value $\pi(s_k, i)$ can be presented by
%\begin{equation}\label{PPR3-math}
%\begin{split}
%\pi(s_k, i) = \pi_1(s_k, i) + \pi_2(s_k, i) & = \pi_1(s_k, i) + \pi_1(s_k, i)\cdot LS(i) \\
%                                            & = \pi_1(s_k, i) \cdot(1+LS(i)).
%\end{split}
%\end{equation}

%\textbf{Comment: Just recall in randomized shortest path betweenness problem, a similar definition to $\pi_1(s_k, i)$, representing the probability of absorbing random walk, also can be computed by $\frac{z_{st}}{z_{tt}}$}.
%
%According to Equation~(\ref{R1-math})(\ref{PPR1-math}), $\frac{\pi_1(s_k, i)}{\alpha}$ represents the summed probability of a random walk from $s_k$, with a decaying factor $1-\alpha$, hitting node $i$ for the first time at iteration $0, 1, 2\cdots$.
%This summed hitting probability measures a \emph{random walk distance} from the source node to node $i$.
%The closer node $i$ is to the source node with respect to \emph{random walk distance}, the greater $\frac{\pi_1(s_k, i)}{\alpha}$ is.
%~
%Consider a source node as a pivot, then each node in graph is encoded with its \emph{random walk distance} with respect to the pivot. Note that a single \emph{random walk distance} does not necessarily illustrate the region of node, since the random walk proceeds to all its neighbors (each as a \emph{direction}) at each step.
%~
%With a sufficient number of source nodes as pivots, apparently, the region information can be encoded in a way by all hitting probabilities.
%For two graphs $G_1$ and $G_2$ to be matched, given a number of correct seed matches as the source nodes on two graphs respectively, then with a certain probability $i\in V_1$ and $j\in V_2$ are on the aligned region over two graphs if and only if they have similar hitting probability vector, i.e., $\frac{\pi^1_1(s^1_k, i)}{\alpha}$ and $\frac{\pi^2_1(s^2_k, j)}{\alpha}$ are relatively close with respect to a certain number of seed pair $[s^1_k, s^2_k]$.
%



\subsection{Compared with Weisfeiler-Lehman labelling}
%The Weisfeiler-Lehman graph labelling method has drawn great attention recently~\cite{shervashidze2011weisfeiler, morris2017global, zhang2017weisfeiler}.
%The k-dimensional Weisfeiler-Lehman algorithm scales exponentially in $k$ on both time complexity and storage, and thus is not favored in most cases.
%~\cite{zhang2017weisfeiler} proposed a Palette-WL, a variation of 1-dimensional WL that is fast and order-preserving.
%However, we can shown that the PPR based graph labelling method has unmatched advantages over Palette-WL method on graph matching problem.
%XXXX
% linear PPR, consistency, than non-linear WL.




\subsubsection{Decomposition of LS}
%
%\textbf{Note: $LS(i)$ may be upper bounded and lower bounded with a simple second order information, the approximate ratio can be evaluated for each node independently, thus it can be decomposed! compute it tomorrow, otherwise we can write sth about the selection of $\alpha$, to bound $LS(i)<1$, $\alpha$ is near $0.3$!!
%\\
%if we can approximately decompose $\pi_1(s_k, i)$ from $\pi$, then a vector based on distance. $Norm\_2$ with respect to Euclidean is not good. Near in one dimensional should have high score, but far has less penalty.}
%
%\textbf{This can be used as an improvement. And the former algorithm is the baseline. IT'S VERY DATABASE..}
%
%\textbf{The question is, if it is necessary to decompose $LS+1$ and $\pi_1$.}
%
%We continue to analyse the value of $LS(i)$. Since a random walk from $i$ takes at least two steps to arrive at $i$, thus $LS(i)$ is upper bounded by $(1-\alpha)^2+(1-\alpha)^4+(1-\alpha)^6+...=\frac{(1-\alpha)^2}{2\alpha-\alpha^2}$ (in the case where all neighbors of $i$ only links to $i$).
%Note that it always satisfies $LS(i)<=1$ (\textbf{why good?}) when $\alpha>=(1-\frac{\sqrt{2}}{2})\approx 0.3$, which happens to be an ideal parameter in our experiments.
%~
%Then we will show how to approximate the value of $LS(i)$ based on the second-order local structure only. Recall the definition of $LS^{(2)}$, we represent $LS^{(3)}$ similarly by
%
%\begin{equation}
%\begin{split}
%LS^{(3)} & = (1-\alpha)^{3}\cdot \frac{1}{|N(i)|} \sum_{\bigtriangleup_{ijk}\in G}\frac{1}{|N(j)||N(k)|}
%\end{split}
%\end{equation}
%For simplification, we assume $T_2= \frac{1}{|N(i)|} \sum_{(i,j)\in E}\frac{1}{|N(j)|}$, and $T_3 = \frac{1}{|N(i)|} \sum_{\bigtriangleup_{ijk}\in G}\frac{1}{|N(j)||N(k)|}$, thus $LS^{(2)}=(1-\alpha)^{2}\cdot T_2$, and $LS^{(3)}=(1-\alpha)^{3}\cdot T_3$.
%
%Apparently, the upper bound of $LS^{(4)}$, say $LS^{(4)}_{ub}= \frac{1-T_2-T_3}{2}*(1-\alpha)^4 + (LS^{(2)})^2$. Then, we have the following equation
%\begin{equation}
%\begin{split}
%    LS^{(t)}_{ub} = LS^{(t-2)}_{ub}*LS^{(2)} + LS^{(t-3)}_{ub}*LS^{(3)} \\
%                  + LS^{(t-4)}_{ub}*LS^{(4)}_{ub}, \ \forall t\ge 5.
%\end{split}
%\end{equation}
%\textbf{Problem:} How to compute the converge of $LS_{ub}=\sum_{t=2}^{\infty} LS_{ub}^{(t)}.$
%%Accordingly, the lower bound of $LS^{(4)}$, say $LS^{(4)}_{lb}=  (1-\alpha)^{4}\cdot \frac{1}{|N(i)|} \sum_{\bigtriangleup_{ijk}\in G}\frac{1}{|N(j)|^2|N(k)|}$.
%
%Next, we define a transition matrix $P_{ub}$ by
%\begin{equation}
%\begin{split}
%P_{ub}=
%\begin{bmatrix}
%    0 & T_2 & 0 & 0   \\
%    (1-\alpha)^2 & 0 & \frac{T_3}{T_2} & 0  \\
%    (1-\alpha)^3 & 0 & 0 & \frac{1-T_2-T_3}{2\cdot T_3} \\
%    (1-\alpha)^4 & 0 & 0 & 0
%\end{bmatrix}
%\end{split}
%\end{equation}
%where $[P^t_{ub}]_{11}=LS^{(t)}_{ub}$. Then $LS_{ub}$ can be presented by
%\begin{equation}
%\begin{split}
%& LS_{ub}  = [\sum_{t=1}^{\infty}P^t_{ub}]_{11} = [(I_4-P_{ub})^{-1}-I_4]_{11} \\
%&         = (1-(1-\alpha)^2 T_2 - (1-\alpha)^3 T_3 - (1-\alpha)^4 \frac{1-T_2-T_3}{2})^{-1}-1.
%\end{split}
%\end{equation}
%
%Similarity, a lower bound of $LS^{(4)}$, say $LS^{(4)}_{lb}= (LS^{(2)})^2 + \frac{1}{|N(i)|} \sum_{\bigtriangleup_{ijk}\in G}\frac{1}{|N(j)|^2|N(k)|}\cdot (1-\alpha)^4$. Note here we enumerate only triangles in the graph but not the quadrangle. Let $T_4 = \frac{1}{|N(i)|} \sum_{\bigtriangleup_{ijk}\in G}\frac{1}{|N(j)|^2|N(k)|}$, and a transition matrix $P_{lb}$ is defined by
%\begin{equation}
%\begin{split}
%P_{lb}=
%\begin{bmatrix}
%    0 & T_2 & 0 & 0   \\
%    (1-\alpha)^2 & 0 & \frac{T_3}{T_2} & 0  \\
%    (1-\alpha)^3 & 0 & 0 & \frac{T_4}{T_3} \\
%    (1-\alpha)^4 & 0 & 0 & 0
%\end{bmatrix}
%\end{split}
%\end{equation}
%where $[P^t_{lb}]_{11}=LS^{(t)}_{lb}$. Then $LS_{lb}$ can be presented by
%\begin{equation}
%\begin{split}
%& LS_{lb} = [\sum_{t=1}^{\infty}P^t_{lb}]_{11} = [(I_4-P_{lb})^{-1}-I_4]_{11} \\
%& = (1-(1-\alpha)^2 T_2 - (1-\alpha)^3 T_3 - (1-\alpha)^4 T_4)^{-1}-1.
%\end{split}
%\end{equation}
%Thus, we finally approximate $LS(i)$ using the first-order and second-order local structure information only, with the time complexity of $O(|E|^{\frac{3}{2}})$ (bound by the cost triangle enumeration) by
%\begin{equation}
%\begin{split}
%LS_{lb}(i) \le LS(i) \le LS_{ub}.
%\end{split}
%\end{equation}
%Let $1+\epsilon_i = \frac{LS_{ub}(i)+1}{LS_{lb}(i)+1}$, then we can have an $(1+\frac{\epsilon_i}{2})$-relative approximation to $LS(i)+1$ by setting
%\[
%\widetilde{LS}(i)+1 = \sqrt{(LS_{ub}(i)+1)(LS_{lb}(i)+1)}.
%\]
%We can prove that $\forall i$, it satisfies $1+\epsilon_i < \frac{1}{1-\frac{(1-\alpha)^4}{2}}$. By setting $\alpha=1-\frac{\sqrt{2}}{2}$, we have $1+\frac{\epsilon_i}{2} < \frac{15}{14}$, which proves the effectiveness of the approximation method.

%
%\textbf{Discussion: Why we set $\alpha=1-\frac{\sqrt{2}}{2}$? Still unconvincing.} With a larger $\alpha$, we can have better relative approximation with respect to both $LS(i)+1$ and $\pi_1$, while the domain of $LS(i)+1$ is very small (on $\alpha=1-\frac{\sqrt{2}}{2}$, $LS(i)+1 \in [1,2)$), and $\pi_1$ can be too distinguishable (or say, \emph{hard}, as weisfeiler-lehman method).
%
%\textbf{In the experiments, all $LS$ concentrates on around $0.06-0.09$, instead of spreading between $(1,2)$. The effect of decomposition is limited.}
%
%\textbf{Interestingly, $LS(i)$, even PPR actually is not directly related to the first-order information \emph{degree}, i.e., assume each neighbor of node $i$ has the same local structure, then $PPR(i)$ remains same.
%Perhaps we can add a degree feature.}
%
%\textbf{Surprisingly, despite of the poor performance of $LS$ approximation distribution, the overall prediction result on facebook dataset only is improved, but on others not. May try other methods of $LS$ approximation, like forward push with relative high stopping threshold, or use the matrix inversion, which takes $O(n^3)$, as the cost of exact PPR computation, impractical though.}



%Seems each source seed $s$ randomly divides the node set into fractions of $\frac{1}{np}$ and $1-\frac{1}{np}$, then needs $O(\log_{\frac{np}{np-1}}{n})$ seeds. Assume $O(np)=o(1)$, then $O(\log(n))$ seeds.
%Given seed $s$, node $i$ and $j$ on graph $G_1$, denote $dist(s,i)$ ($dist(s,j)$) the shortest path distance from $s$ to $i$ ($j$), then we claim $dist(s,i)\ne dist(s,j)$ with probability greater than $1-\frac{1}{np}$.
%The above is wrong: should be the probability on one possible world. thus all seeds have dependency.
%new: two seeds to a node, overlap or not; a seed to two nodes, overlap or not.


%simply denoted by $Pr(\sum_r{I_r(i,j)})$ where $I_r(i,j)={|Y^r_i \cap Y^r_j|}/n$. We are going to prove $1-Pr(\sum_r{I_r(i,j)})= O(\frac{1}{np})$.

% how to model |Y^r_i|? it's more complicated than markov binomial distributions
% can $Pr(s\in Y^2_i)$ be regarded as an independent bernoulli trial? not sure if the following is correct.
%A random node $s\in Y^1_i$ with probability $p$.
%Then $Pr(s\in Y^2_i)=(1-p)\sum^{\infty}_{k=1}{{{n}\choose{k}} p^k(1-p)^{n-k}(1-(1-p)^k)}\approx(1-p)np^2$, denoted by $p_2$.
%And we also have $Pr(s\in Y^{\le 2}_i)=p+np^2-np^3$, denoted by $p_{\le 2}$. %\approx=p+np^2

% Pr(s\in Y^2_i) and Pr(s\in Y^3_i) have dependency, and the following induction is wrong.
%Since $Pr(s\in Y^{3}_i)=Pr(s\not\in Y^{\le 2}_i)Pr(s\in Y^3_i \given s\not\in Y^{\le 2}_i)$, the correlation has not been solved by any existing work, according to a recent slide \footnote{\url{https://www.uni-oldenburg.de/fileadmin/user_upload/physik/ag/compphys/download/talks/eytan_katzav2015.pdf}}. The correlation is ignored in paper Distance distribution in random graphs and application to networks exploration, when the simulation is the focus.

%wrong. Then $Pr(s\in Y^{3}_i)=(1-p_{\le 2})\sum^{\infty}_{k=1}{n\choose k}p_{2}^k(1-p_{2})^{n-k}(1-(1-p)^k)=(1-p_{\le 2})np_2p\approx (1-p-np^2)n^2p^3$.

%wrong. Note we always have $P(s\in Y^{r}_i)=(1-p_{\le r})\sum^{\infty}_{k=1}{n\choose k}p_{r}^k(1-p_{r})^{n-k}(1-(1-p)^k)=(1-p_{\le r})np_r p$ = $(1-\sum_{k=0}^{r-2}{n^k p^{k+1}})n^{r-1}p^r$ for $r\ge 2$.

%wrong. As we have $np\to c>1$, thus $\frac{1}{p}\gg \log(n)$, and $1\gg p\log_{np}(n)$. As a result, the dependency between $Y^r_i\cap Y^r_j$ and $Y^{r+1}_i\cap Y^{r+1}_j$ for all $r\in \mathbb{Z}^+$, which aggregates to approximately $p\log_{np}(n)$, is negligible in approximating $Pr(\sum_r{I_r(i,j)})$.
% don't know how to solve the dependency otherwise.

% if assume $np \to w\log(n)$, where $w\to \infty$, then cannot distinguish with shortest path.
% if assume $np \to c >1$, then cannot bound diameter $d$ simply by a fixed value.
% $np\to c\log(n)$?sss
%If $np\ge 4$ (the case where $np<4$ should be better), assume $|Y^r_i|=t$, then w.h.p. $\frac{t}{2np} \le |Y^{r-1}_i|\le \frac{2t}{np}$, $ \le |Y^{\le r}_i| \le $
% If $n\to \infty$, then the expected number of isolated nodes

